Differentially Private Data Release over Multiple Tables

We study synthetic data release for answering multiple linear queries over a set of database tables in a differentially private way. Two special cases have been considered in the literature: how to release a synthetic dataset for answering multiple linear queries over a single table, and how to release the answer for a single counting (join size) query over a set of database tables. Compared to the single-table case, the join operator makes query answering challenging, since the sensitivity (i.e., by how much an individual data record can affect the answer) could be heavily amplified by complex join relationships. We present an algorithm for the general problem, and prove a lower bound illustrating that our general algorithm achieves parameterized optimality (up to logarithmic factors) on some simple queries (e.g., two-table join queries) in the most commonly-used privacy parameter regimes. For the case of hierarchical joins, we present a data partition procedure that exploits the concept of {\em uniformized sensitivities} to further improve the utility.

==> backup-laplace/conclusion.tex <==
\section{Conclusions and Discussion}

In this work, we proposed algorithms for answering linear queries of multi-table joins.  Our work opens up several interesting questions that we list below.

\paragraph{Non-Hierarchical Setting.} 
First and perhaps the most immediate question is if   uniformization can benefit the non-hierarchical case. We note that the uniformization technique from \Cref{sec:hierarchical} itself is applicable but may not lead to uniformized residual sensitivity on non-hierarchical queries, even on the simplest non-hierarchical join $R_1(A,B)\Join R_2(B,C) \Join R_3(C,D)$. %However, this does not rule out the possibility of other ways to improve Theorem~\ref{the:ub-multi-table} on non-hierarchical joins. Let us use this length-3 path join to illustrate the idea. 
We can simply partition values in $\dom(B)$ into buckets, each of which is indexed by two integers such that $B^{ij} = \{b \in \dom(B): \degg_1(B,b) \in (\gamma_{i-1},\gamma_i], \degg_2(B,b) \in (\gamma_{j-1}, \gamma_j]\}.$
%\begin{align*}
%    B^{ij} = \{b \in \dom(B): & \degg_1(B,b) \in %(\max\{0,\lambda\cdot 2^{i-1}\},\lambda \cdot 2^i], \\ 
%    & \degg_2(B,b) \in (\max\{0,\lambda\cdot 2^{j-1}\},\lambda \cdot 2^j]\}.
%\end{align*}
Similar partition idea applies to values in $\dom(C)$. Note that each pair  $\left(B^{ij}, C^{kh}\right)$ of buckets corresponding to $\sigma=(i,j,k,h)$ defines a sub-instance $\I^\sigma$. But, residual sensitivity within each sub-instance is not guaranteed to be uniformized. In determining the residual sensitivity in (\ref{eq:residual}), we observe that $T_{23} \le \lambda^2 \cdot 2^{j+h}$ and $T_{12} \le \lambda^2 \cdot 2^{i+k}$; however, $\degg_2(B,b)$ and $\degg_2(C,c)$ are defined over the whole instance $\I$, instead of the specific instance $\I^\sigma$. %the join size of following residual queries can be upper bounded by $\sigma$:
%\begin{align*}
%    T_{23} & \le \max_{b \in \dom(B)} \degg_{2}(B,b) \cdot \max_{c \in \dom(C)} \degg_3(C,c) \le 2^{j+h} \\ 
%    T_{12} & \le \max_{c \in \dom(C)} \degg_{2}(C,c) \cdot \max_{b \in \dom(B)} \degg_1(B,b) \le 2^{i+k},
    %T_{13} & \le \max_{b \in \dom(B)} \degg_{1}(B,b) \cdot \max_{c\in \dom(C)} \degg_3(C,c) \le 2^{i+h}
%\end{align*}
%where $\degg_2(B,b)$ and $\degg_2(C,c)$ are defined over the whole instance $\I$, instead of the specific instance $\I^\sigma$. 
This coarse-grained partition can be extended to arbitrary acyclic query (see Appendix~\ref{appendix:uniformization}), but does not necessarily lead to uniformized residual sensitivity inside each sub-instance. We leave this as an interesting future work.

\paragraph{Query-Specific Optimality.} 
Throughout this work, we consider \emph{worst-case} set $\Q$ of queries parameterized by its size. Although this is a reasonable starting point, it is also plausible to hope for an algorithm that is nearly optimal for \emph{all} query set $\Q$. In the single table case, this has been achieved in~\cite{HardtT10,BhaskaraDKT12,NikolovT016}. However, the situation is rather complicated in multi-table setting since we have to take the local sensitivity into account, whereas, in the single table case, the query family already tells us everything about the possible change by moving to a neighboring dataset. This also seems like an interesting open question for future research.

\paragraph{Instance-Specific Optimality.}
Similarly, we have considered worst-case instances. One might instead prefer to achieve finer-grained instance-optimal errors. For the single table case, \cite{asi2020instance} observed that an instance-optimal DP algorithm is not achievable, since a trivial algorithm can return the same answer(s) for all input instances, which could work perfectly on one specific instance but miserably on all remaining instances. To overcome this, a notion of ``neighborhood optimality'' has been proposed~\cite{dong2021nearly, asi2020instance} where we consider not only a single instance but also its neighbors at some constant distance. We note, however, that this would not work for our setting when there are a large number of queries. Specifically, if we again consider an algorithm that always returns the true answer for this instance, then its error with respect to the entire neighborhood set is still quite small--at most the distance times the maximum local sensitivity in the set. This is independent of the table size $n$, whereas our lower bounds show that the dependency on $n$ is inevitable. As such, the question of how to define and prove instance-optimal errors remains open for the multi-query case.

%Instead, it has been proved that smooth sensitivity (as well as residual sensitivity) already achieves $(O(1), O(1))$-{\em neighborhood optimality} for answering this single counting query $\countsize(\cdot)$; we refer interested readers to \cite{dong2021nearly, asi2020instance} for more details. Here, we also believe that it would be inherently impossible to close the gap, but this will be left as an open question. On the other hand, this gap is tight up to logarithmic factors on some simple join queries, for example, the two-table join.
 
%\paragraph{Discussion.} Comparing with Theorem~\ref{the:lb-two-table-2}, a more fine-grained parameterized notion of optimality has been achieved in Theorem~\ref{the:up-2table-uniformize}. A natural question is: Can we push this idea to the extreme, such that each parameterized class only contains a single instance, to obtain {\em instance-optimality}? As observed by \cite{asi2020instance}, this is not possible. We then leave the question of obtaining a neighborhood-optimal algorithm for releasing synthetic dataset as future work. 

==> backup-laplace/hierarchical.tex <==
\subsection{Uniformize Hierarchical Query} 
\label{sec:hierarchical}

Beyond two-table query, we surprisingly find that this uniformization technique can be further extended to the class of {\em hierarchical queries}. A join query $\H = \{\x, \{\x_1, \x_2, \cdots, \x_m\}\}$ is {\em hierarchical}, if for any pair of attributes $x,y$, either $E_x \subseteq E_y$, or $E_y \subseteq E_x$, or $E_x \cap E_y = \emptyset$, where $E_x = \{i: x \in \x_i\}$ is the set of relations containing attribute $x$. One can always organize the attributes of a hierarchical join into a tree such that every relation corresponds to a root-to-node path (see Figure~\ref{fig:hierarchical}). 

Thanks to the nice structures of hierarchical joins, it is feasible to play with the magic of uniformization. Recall that the essence of uniformization is to partition instance into a set of sub-instances, so that we can get an upper bound on the residual sensitivity as tight as possible, as implied by the error expression in Theorem~\ref{the:ub-multi-table}. In (\ref{eq:residual}), the residual sensitivity is built on the join sizes of a set of residual queries, but these statistics are too far away from being the partition criteria. Instead of using residual sensitivity directly, we first rewrite the join size of an residual query and get an upper bound for it in terms of degrees. 
%The residual sensitivity for counting the join size of an input instance $\I$ displays a rather complicated form, by taking all neighboring instances within distance $k$ from $\I$ into consideration, for any $k \ge 0$. Instead, we adopt a constant upper bound of residual sensitivity known as residual sensitivity in the literature, 
%The residual sensitivity to be used involves statistics of the input instance $\I$ itself, which makes the uniformization feasible.

\subsubsection{{\bf An Upper Bound on Residual Query Size}} 

To derive an upper bound on $T_E$'s for $E \subseteq [m]$, we target a broader class of {\em $\bar{q}$-hierarchical queries}\footnote{This is different from {\em q-hierarchical queries} in \cite{berkholz2017answering}, where $\y$ serves as the set of output attributes, although they have the same property characterization on $\y$.} by generalizing the aggregate attributes in (\ref{eq:TE}) to any subset of attributes that sit on the ``top'' of $\mathcal{T}$. It is not hard to see that $T_E = T_{E,\partial E}$ for boundary attributes $\partial E$.

\begin{definition}
\label{def:bar-q}
    For a hierarchical join $\H = (\x, \{\x_1, \x_2, \cdots, \x_m\})$ and instance $\I$, a $\bar{q}$-hierarchical query on $E \subseteq [m]$ and $\y \subseteq (\cup_{i\in E}\x_i)$ is defined as
    $\displaystyle{T_{E,\y}(\I) = \max_{t \in \dom(\y)} \big|(\Join_{i \in E} R_i) \ltimes t \big|}$, 
    where $\y$ satisfies the property: for any $x_1, x_2 \in \x$, if $E_{x_1} \subseteq E_{x_2}$ and $x_1 \in \y$, then $x_2 \in \y$.
\end{definition}

In the remaining, we focus on deriving an upper bound for $\bar{q}$-hierarchical queries $T_{E,\y}(\I)$, which boils down to a product chain of {\em degree functions}.
For example, $\degg^\I_{34}(AB, ab)$ in Figure~\ref{fig:hierarchical} indicates the number of tuples in $\pi_{ABE} (R_3 \Join R_4)$ that $ab$ appears.

\begin{definition}[Degree Function]
\label{def:degree-function}
    For a hierarchical join $\H = (\x, \{\x_1, \x_2, \cdots, \x_m\})$ and an instance $\I$, the degree function $\degg^\I_E(\y,\vec{y})$ for a subset of relations $E \subseteq [m]$, a subset of attributes $\y \subseteq (\cap_{i \in [E]} \x_i)$ and %\pasin{Why is $\Vec{y}$ here denoted as a vector?} 
    a tuple $\Vec{y} \in \dom(\y)$ is defined as\footnote{When the context is clear, we drop the superscript $\I$ from 
$\degg^\I_E(\cdot,\cdot)$. Moreover, when $|E| =1$, say $E = \{i\}$, we just write $\degg_i(\cdot,\cdot)$ as short for $\degg_E(\cdot,\cdot)$.}:
    \begin{equation}
        \label{eq:degree-function}
        \degg^\I_E(\y,\Vec{y}) = \bigg|\left\{t \in \pi_{\cap_{i \in [E]} \x_i}\Join_{i \in E} R_i: \pi_\y t = \Vec{y} \right\}\bigg|
    \end{equation}
    %i.e.,  the number of tuples that $\Vec{y}$ appears over attributes $\y$ in the projection of the residual query \badih{previous sentence unclear?} result onto their common attributes. \badih{Per discussion with Xiao, might be better to given an example of what this means based on one of the figures?}
\end{definition}


%Equivalently, $\y$ in Definition~\ref{def:bar-q} forms a connected subtree of $\mathcal{T}$, including $r$. Moreover, $T_E = T_{E,\partial E}$ since $\partial E$ also satisfies the constraint in Definition~\ref{def:bar-q}. In the remaining, we focus on deriving an upper bound for $\bar{q}$-hierarchical queries using degree functions.

\noindent
\textbf{Base Case.} When $|E|=1$, say $E = \{i\}$, $T_{E,\y}$ degenerates to the degree of tuples over attributes $\y$ in $R_i$ (as $\y \subseteq \x_i$): 
\begin{displaymath}
T_{E,\y}(\I) = \max_{t \in \dom(\y)}\big|R_i \ltimes t\big| = \left\{ \begin{array}{ll}
    1 & \textrm{if $\y = \x_i$}\\
    \displaystyle{\max_{t \in \dom(\y)} \degg_i(\y, \pi_{\y} t)} & \textrm{otherwise}
\end{array} \right.
\end{displaymath}

\noindent
\textbf{General Case.} Denote $\bar{H}_E$ as the residual query of $\Join_{i\in E} R_i$ by removing attributes in $\y$. We distinguish the following two cases:
\begin{itemize}[leftmargin=*]
    \item {$\bar{H}_E$ is disconnected.} Let $\mathcal{C}_E$ be the set of connected component of $\bar{H}_E$. We can then decompose $\Join_{i\in E} R_i$ into a set of sub-queries, after pushing the semi-join inside each connected component:
    \begin{align*}
        T_{E,\y}(\I) = & \max_{t \in \dom(\y)} \prod_{E' \in \mathcal{C}_E} \big|\left(\Join_{i \in E'} R_i\right) \ltimes t\big| \\
        \le & \prod_{E' \in \mathcal{C}_E} \max_{t \in \dom(\y)} \big|\left(\Join_{i \in E'} R_i\right) \ltimes t\big| = \prod_{E' \in \mathcal{C}_E} T_{E', \y \cap (\cup_{i\in E'} \x_i)}(\I)
    \end{align*}
    The correctness follows that $\y \cap (\cup_{i\in E'} \x_i) \subseteq \cup_{i \in E'} \x_i$ and $\y \cap (\cup_{i\in E'} \x_i)$ satisfies the property in Defition~\ref{def:degree-function}.
    \item {$\bar{H}_E$ is connected.} In this case, we must have $\y \subsetneq (\cap_{i \in E} \x_i)$.
    \begin{align*}
        T_{E,\y}(\I) \le & \max_{t \in \dom(\y)} \degg_{E}(\y, t) \cdot \max_{t' \in \dom(\cap_{i \in E} \x_i): \pi_{\y} t' = t} \big|(\Join_{i \in E} R_i) \ltimes t'\big| \\
        \le& \max_{t \in \dom(\y)}\degg_{E}(\y, t) \cdot \max_{t' \in \dom(\cap_{i \in E} \x_i)} \big|(\Join_{i \in E} R_i) \ltimes t'\big| \\
        =& \max_{t \in \dom(\y)} \degg_{E}(\y, t) \cdot T_{E, \cap_{i \in E} \x_i}(\I)
    \end{align*}
    The correctness follows that $(\cap_{i \in E} \x_i) \subseteq (\cup_{i\in E} \x_i)$ and $\cap_{i \in E} \x_i$ satisfies the property in Definition~\ref{def:degree-function}.
\end{itemize}

It is not hard to see that $T_{E,\y}$ is eventually upper bounded by a product chain of degree functions (see Example~\ref{exp:hierarchical}). Careful inspection reveals that degree functions participate in $T_{E,\partial E}$ are not arbitrary; instead, they display very special structures captured by Lemma~\ref{lem:hierarchical-degree-function}, which is critical to our partition procedure. %An example is given in Figure~\ref{fig:hierarchical}. %We note that these special degree functions used by $T_{E, \partial E}$, which is the foundation for our partition algorithm. An example is given in Figure~\ref{fig:hierarchical}. 

%\begin{lemma}
%\label{lem:hierarchical-degree-function}
%    Every degree function $\degg_{E'}(\y', \cdot)$ participating in an upper bound for $T_{E, \partial E}$, must satisfy the following properties:
%    \begin{itemize}[leftmargin=*]
%        \item $\y' = \{x \in \x: \exists i \in E', j \notin E', x \in \x_i \cap \x_j\}$;
%        \item $\y' \subsetneq (\cap_{i\in E'}\x_i)$;
%        \item there exists no $j \notin E'$ such that $(\cap_{i \in E'} \x_i) \subseteq \x_j$.
%       \item If $x$ is the node such that $\cap_{i \in E'} \x_i = \textsf{path}(r,x)$, let $x' \in \textsf{path}(r,x)$ be the lowest ancestor of $x$ with more than one child. Then, $E' = E_x$ and $\y' = \textsf{path}(r,x')$.    
%    \end{itemize}
%\end{lemma}

\begin{lemma}
\label{lem:hierarchical-degree-function}
    Every degree function $\degg_{E'}(\y', \cdot)$ participating in the upper bound of $T_{E, \partial E}$ corresponds to a distinct attribute $x \in \x$ such that $E' = E_x$ and $\y'$ corresponds to the set of attributes lying on the path from the root $r$ to $x$'s parent in $\mathcal{T}$. %, where $x'$ is the parent of $x$ in $\mathcal{T}$, $r$ is the root of $\mathcal{T}$, and $\textsf{path}(r,x')$ is the set of attributes lying on the path from $r$ to $x$.
\end{lemma}

\begin{figure}
    \centering
    \includegraphics[scale=0.47]{img/attribute-tree.pdf}
    \caption{Attribute tree for hierarchical join: $R_1(A,B,D) \Join R_2(A,B,F) \Join R_3(A,B,G,K) \Join R_4(A,B,G,L) \Join R_5(A,C)$, and an example of $H_E$ for $E = \{3,4,5\}$, with boundary attributes $\partial E = \{A,B\}$. After removing $\partial E$, $E$ is decomposed into $\{\{3,4\}, 5\}$.}
    \label{fig:hierarchical}
    \end{figure}
    
    \begin{example}
    An upper bound derived for $T_E$ in Figure~\ref{fig:hierarchical}:
    \begin{align*}
        T_{345} =& \max_{(a,b) \in A \times B} |R_3 \Join R_4 \Join R_5 \ltimes (a,b)| \\
        =& \max_{a \in A} |R_5 \ltimes (a)| \times \max_{(a,b) \in A\times B} |R_3 \Join R_4 \ltimes (a,b)|\\
        =& \max_{a \in A} |R_5 \ltimes (a)| \times \max_{(a,b) \in A\times B} |\pi_{ABG} R_3 \Join R_4| \\
        \times & \max_{(a,b,g) \in A \times B \times G} |R_3 \ltimes (a,b,g)| \times  \max_{(a,b,g) \in A \times B \times G} |R_4 \ltimes (a,b,g)| \\
        =& \max_{a \in A} \degg_5(A,a) \times \max_{(a,b,g) \in A\times B \times G} \degg_3(ABG,abg) \\
        \times& \max_{(a,b,g) \in A \times B \times G} \degg_4(ABG,abg) \times \max_{(a,b) \in A\times B} \degg_{34}(AB,ab)
    \end{align*}
    \label{exp:hierarchical}
    \end{example}

%\begin{figure}
%    \begin{minipage}{1\linewidth}
%    \centering
%    \includegraphics[scale=0.47]{img/pdfresizer.com-pdf-crop.pdf}
%    \caption{Right upper is the attribute tree for hierarchical join: $R_1(A,B,D) \Join R_2(A,B,F) \Join R_3(A,B,G,K) \Join R_4(A,B,G,L) \Join R_5(A,C)$, and  an example of $H_E$ for $E = \{3,4,5\}$, with boundary attributes $\partial E = \{A,B\}$. After removing $\partial E$, $E$ is decomposed into $\{\{3,4\}, 5\}$. The left is an upper bound derived for $T_E$.}
 %   \label{fig:hierarchical}
 %   \end{minipage} %\quad 
    %\begin{minipage}{0.2\linewidth}
   % \centering
    %%\vspace{-1em}
    %\includegraphics[scale=0.5]{img/hard-three-table.pdf}
    %\caption{A hard instance of line-3 join query for uniformization.}
   % \label{fig:line-3}
   % \end{minipage}
%\end{figure}


\subsubsection{Partition with Degree Characterization}

From the upper bound on $T_{E,\partial E}(\I)$, we now define the degree characterization for hierarchical joins, similar as the two-table join. Our target is to partition the input instance into a set of sub-instances (which may not be tuple-disjoint), such that each sub-instance is captured by a distinct degree characterization, and the join results over all sub-instances form a partition of the final join result. 

\begin{definition}[Degree Characterization]
\label{def:degree-characterization}
    For a hierarchical join $\H =(\x, \{\x_1,\x_2,\cdots,\x_m\})$, a degree characterization is defined as $\sigma: 2^{[m]}\times 2^{\x} \to \mathbb{Z}^* \cup \{\bot\}$ such that for any $E \subseteq [m]$ and $\y \subseteq \x$, $\sigma(E, \y) \neq \bot$ if and only if there exists an attribute $x \in \x$ such that $E = E_x$ and $\y$ is the set of ancestors of $x$ in $\mathcal{T}$.
\end{definition}

As described in Algorithm~\ref{alg:uniformize-hierarchical}, the high-level idea is to partition the input instance by attributes in a bottom-up way on $\mathcal{T}$, where $\mathcal{T}$ is the attribute tree of the input hierarchical query $\mathcal{H}$, and invoke Algorithm~\ref{alg:partition-hierarchical} as a primitive on every sub-instance obtained so far.

As described in Algorithm~\ref{alg:partition-hierarchical}, {\sc PartitionByAttr} takes an input an attribute $x$ and an instance $\I'$ such that
\begin{itemize}[leftmargin=*]
    \item for every attribute $x'$ as a descendant of $x$ in $\mathcal{T}$, $\degg^{\I'}_{E_{x'}}(\y', \vec{y})$ is uniformized for every $\vec{y} \in \dom(\y')$, where $\y'$ is the set of ancestors of $x'$ in $\mathcal{T}$.
\end{itemize}
and outputs a set of sub-instances $\mathbb{I}'$ of $\I'$, such that 
\begin{itemize}[leftmargin=*]
    \item $\bigcupplus_{\I'' \in \mathbb{I}'} \left(\Join_{i \in [m]} R^{\I''}_i\right) = \left(\Join_{i \in [m]} R^{\I'}_i\right)$, i.e., the join results of sub-instances in $\mathbb{I}'$ form a partition of join result of $\I'$;
    \item for every sub-instance $\I'' \in \mathbb{I}'$, $\degg^{\I''}_{E_x}(\y, \vec{y})$ is roughly the same for every $\vec{y} \in \dom(\y)$, where $\y$ is the set of ancestors of $x$ in $\mathcal{T}$.
\end{itemize}
Similar to the two-table case, for every $\vec{y} \in \dom(\y)$, we compute a noisy version of its degree $\degg^{\I'}_{E_x}(\y,\Vec{y})$ and put it into the bucket indexed by its logarithmic value. For each $j \in E_x$, we obtain a tuple-disjoint partition of $R^{\I'}_j$ based on $\y$, such that each $i \in \lceil \log \left(\frac{n}{\lambda}+1\right) \rceil$ defines a sub-instance involving a sub-relation $R^{\I'}_{j,i}$ for each $j \in E_x$ as well as all remaining relations $R^{\I'}_j$ with $j \notin E_x$. At last, we return the union of all sub-instances. 

\begin{algorithm}[t]
\caption{{\sc Partition-Hierarchical}$(\I)$}
\label{alg:uniformize-hierarchical}

$\mathbb{I} \gets \{\I\}$\;
$\mathcal{T} \gets$ the attribute tree of $\left(\x, \{\x_1, \x_2, \cdots, \x_m\}\right)$\;
\While{there is an non-visited node in $\mathcal{T}$}{
    $x \gets$ any leaf or any node whose children are all visited\;
    \ForEach{$\I' \in \mathbb{I}$}{
        $\mathbb{I} \gets \mathbb{I} \cup \textsc{PartitionByAttr}(\I', x)$\;
    }
    Mark $x$ as ``visited''\;
}
\Return $\mathbb{I}$\;
\end{algorithm}

\begin{algorithm}[t]
\caption{{\sc PartitionByAttr}$(\I', x)$}
\label{alg:partition-hierarchical}

$\y \gets \{y \in \x: E_x \subsetneq E_y\}$\;
%$\ell \gets \lceil \log (\frac{n}{\lambda} + 1) \rceil$\;
%$\y^i \gets \emptyset$ for $i \in [\ell]$\;
\ForEach{$\Vec{y} \in \dom(\y)$}{
    $\deg^{\I'}_{E_x}(\y, \Vec{y}) = \degg^{\I'}_{E_x}(\y, \Vec{y}) + \textsf{STGeom}_{\epsilon, \delta, 1}(x)$\;
    $i \gets \max\left\{1, \left\lceil \log \frac{1}{\lambda} \cdot \deg^{\I'}_{E_x}(\y,\Vec{y}) \right\rceil\right\}$\;
    \lIf{$\y^i$ does not exist}{$\y^i \gets \left\{\Vec{y}\right\}$}
    \lElse{$\y^i \gets \y^i \cup \left\{\Vec{y}\right\}$}
}
\ForEach{$i$ with $\y^i \neq \emptyset$}{
    \ForEach{$j \in E_x$}{
    $R^{\I'}_{j,i} = \left\{R^{\I'}_j(t): t\in \D_j, \pi_\y t \in \y^i, R^{\I'}_j(t) >0\right\}$}
}

\Return $\bigcup_{i: \y^i \neq \emptyset} \left\{\{R^{\I'}_{j,i}: j \in E_x\} \cup \{R^{\I'}_{j}: j \notin E_x\} \right\}$\;
\end{algorithm}

\begin{lemma}
\label{lem:partition-hierarchical}
    For input instance $\I$, let $\mathbb{I}$ be the set of sub-instances returned by Algorithm~\ref{alg:partition-hierarchical}. $\mathbb{I}$ satisfies the following properties:
    \begin{itemize}[leftmargin=*]
        \item $\bigcupplus_{\I' \in \mathbb{I}} \left(\Join_{i \in [m]} R^{\I'}_i\right) = \left(\Join_{i \in [m]} R^{\I}_i\right)$, i.e., the join results of all sub-instances in $\mathbb{I}$ form a partition of the join result of $\I$;
        \item Each input tuple appears in $O\left(\log^c n\right)$ sub-instances of  $\mathbb{I}$, where $c$ is a constant depending on query size;
        \item Each sub-instance $\I^\sigma \in \mathbb{I}$ corresponds to a distinct degree characterization $\sigma$ such that for any $E \in [m]$ and $\y \subseteq \x_E$ with $\sigma(E,\y)\neq \bot$:
        %\begin{equation}
        %    \label{eq:degree-sigma}
        %    \deg^{\I^\sigma}_E(\y, \vec{y}) \in \left(\max\left\{0,\lambda \cdot 2^{\sigma(E,\y)-1}\right\}, \lambda \cdot 2^{\sigma(E,\y)}\right]
        %\end{equation}
        \begin{equation}
            \label{eq:degree-sigma}
            \deg^{\I^\sigma}_E(\y, \vec{y}) \in \left(\gamma_{i-1} \cdot 2^{\sigma(E,\y)-1}, \gamma_{i} \cdot 2^{\sigma(E,\y)\right]
        \end{equation}
        holds for any $\vec{y} \in \dom(\y)$ if  $\deg^{\I^\sigma}_E(\y,\vec{y}) >0$.
    \end{itemize}
\end{lemma}


\begin{lemma}
\label{lem:partition-hierarchical-DP}
    Algorithm~\ref{alg:uniformization-framework} on hierarchical joins is $(O(\log^c n) \cdot \epsilon, O(\log^c n) \cdot \delta)$-DP%, where $c$ is the query-dependent constant.
    , where $c$ is a constant depending only on the tree.
    \pasin{I fixed this: I think $c$ is tree-dependent but *not* query (i.e. $\Q$)-dependent.}
\end{lemma}

The logarithmic factor in Lemma~\ref{lem:partition-hierarchical-DP} arise since each input tuple participates in $O(\log^c n)$ sub-instances, implied by Lemma~\ref{lem:partition-hierarchical}.
Next, given a degree characterization $\sigma$, how to derive the residual sensitivity of instances consistent with $\sigma$? Actually, this is already resolved by just rewriting the upper bound derived for $T_{E}$, denoted as $T^\sigma_{E}$. Similar to the two-table case, we also define the {\em uniform partition} of an input instance $\I$ over a hierarchical join query $\Q$ using true degrees as $\{\I^\sigma: \sigma \textrm{ is a degree characterization of } \I\}$. As shown in Appendix~\ref{appendix:uniformization}, the error complexity achieved by the partition based on noisy degrees can be bounded by the uniform one.

\begin{theorem}
\label{the:ub-hierarhical-uniformize}
    For any hierarchical join $\H = (\x, \{\x_1, \x_2,\cdots,\x_m\})$ and an instance $\I$, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that is $(\epsilon, \delta)$-DP, and with probability at least $1- 1/\textsf{poly}(|\Q|)$ produces $\F$ such that all queries in $\Q$ can be answered within error:
    \[\alpha = O\left( (\sum_{\sigma}  \sqrt{\OUT^{\sigma} \cdot SS^\beta_\countsize\left(\I^\sigma\right) \cdot \lambda} + SS^\beta_\countsize\left(\I^\sigma\right) \cdot \lambda) \cdot \fup \right)  \]
    where $\sigma$ is over all degree characterizations of $\I$, $\I^\sigma$ is the sub-instance characterized by $\sigma$,  $\OUT^\sigma$ is the join size of $\I^\sigma$, and $\beta = \frac{\epsilon}{2 \ln (2/\delta)}$.
\end{theorem}

Let $\overrightarrow{\OUT} = \left\{\OUT^\sigma \in \mathbb{Z}: \sigma \textrm{ is a degree characterization of } \I\right\}$ as the output size distribution over the uniform degree partition. 
An instance $\I$ conforms to $\overrightarrow{\OUT}$ if $|J^\sigma| = \OUT^\sigma$, for every degree characterization $\sigma$, where $J^\sigma$ is the join result of sub-instance $\I^\sigma$. Extending the lower bound argument of Theorem~\ref{the:lb-instance-optimality-2table}, we obtain the following parameterized lower bound for hierarchical queries.

\begin{theorem}
\label{the:lb-hierarhical-uniformize}
    %Given arbitrary parameters $\OUT \geq \Delta > 0$,
    Given a hierarchical join $\H = (\x, \{\x_1, \x_2, \cdots, \x_m\})$ and an arbitrary parameters $\overrightarrow{\OUT}$, 
    %let $\mathbb{I}(\overrightarrow{\OUT})$ be the set of instances that conform to $\overrightarrow{\OUT}$. There exists a set of queries $\Q$ on which any $(\epsilon, \delta)$-DP algorithm that takes as input an instance from $\mathbb{I}(\overrightarrow{\OUT})$ and outputs an approximate answer to each query in $\Q$ within error $\alpha$ must require
    for every sufficiently small $\eps, \alpha>0$, $n_D \ge (1/\alpha)^{\Omega(1)}$ and $n_Q \leq (1/\alpha)^{O(1)}$, there exists a family of queries $\Q$ of size $n_Q$ on domain $\D$ of size $n_D$ such that any $(\epsilon, o(1/n))$-differentially private algorithm that takes as input a multi-table database over $\H$ of input size at most $n$ while conforming to $\overrightarrow{\OUT}$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ must satisfy 
    \[\alpha \ge \tOmega\left(\max_{\sigma} \sqrt{\OUT^{\sigma}}\cdot \sqrt{LS^\sigma_\countsize} \cdot \flo\right) \]
    where $\sigma$ is over all degree characterizations and $\displaystyle{LS^\sigma_\countsize = \max_{i \in [m]} T^\sigma_{[m]-i}}$ is the local sensitivity of $\countsize(\cdot)$ under $\sigma$.
\end{theorem}

%\input{three-table}




==> backup-laplace/intro.tex <==
\section{Introduction}
\label{sec:intro}

 Synthetic data release is a very useful objective in private data analysis. Differential privacy (DP) \cite{dwork2006calibrating,dwork2006our} has emerged as a compelling model that enables us to formally study the tradeoff between utility of released information and the privacy of individuals. In the literature, there has been a large body of work that studies synthetic data release over a single table, for example, the private multiplicative weight algorithm~\cite{hardt2012simple}, the histogram-based algorithm~\cite{vadhan2017complexity}, the matrix mechanism~\cite{li2010optimizing}, the Bayesian network algorithm \cite{zhang2017privbayes}; as well as other works focusing on geometric range queries~\cite{li2011efficient, li2012adaptive, dwork2010differential, bun2015differentially, chan2011private, dwork2015pure, cormode2012differentially, huang2021approximate}, and datacubes~\cite{ding2011differentially}. 

Data analysis over multiple private tables connected via join operators has been the subject of significant interest within the area of modern database systems. In particular, the challenging question of releasing the join size over a set of private tables has been studied in several recent works including the sensitivity-based framework~\cite{johnson2018towards, dong2021residual,dong2021nearly}, the truncation-based mechanism~\cite{kotsogiannis2019privatesql, dong2022r2t, tao2020computing}, as well as in works on one-to-one joins~\cite{mcsherry2009privacy,proserpio2014calibrating}, and on graph databases~\cite{blocki2013differentially, chen2013recursive}. In practice, multiple queries (as opposed to a single one) are typically issued for data analysis, for example, a large class of linear queries on top of join results with different weights on input tuples, as a generalization of the counting join size query. One might consider answering each query independently but the utility would be very low due to the limited privacy budget, implied by the DP composition rule~\cite{dwork2006calibrating, dwork2006our}. Hence the question that we tackle in this paper is: how can we release synthetic data for accurately answering a large class of linear queries over multiple tables in a differentially private way?
% In this paper, we take the first step in answering this question with theoretical guarantees.

\subsection{Problem Definition}

 \paragraph{Multi-way Join and Linear Queries.} A (natural) join query can be represented as a hypergraph $\mathcal{H} = (\x, \{\x_1, \x_2, \cdots, \x_m\})$~\cite{abiteboul1995foundations}, where $\x$ is the set of vertices or attributes and each $\x_i \subseteq \x$ is a hyperedge or relation. Let $\dom(x)$ be the domain of attribute $x$. Define $\displaystyle{\D = \dom(\x) = \prod_{x \in \x} \dom(x)}$, and $\displaystyle{\D_i = \dom(\x_i) = \prod_{x \in \x_i} \dom(x)}$ for any $i \in [m]$. Given an input instance $\I = \left(R^\I_1, R^\I_2, \cdots, R^\I_m\right)$, each table $R^\I_i: \D_i \to \mathbb{Z}^{\geq 0}$ %\pasin{Is it standard for the range to be $0, 1$? Or do we people generally consider the range to be $\Z$ as well?} Resolved.
 is defined as a function from domain $\D_i$ to a non-negative integer, indicating the frequency of each tuple. This is more general than the setting where each tuple appears at most once in each relation, since it can capture annotated relations~\cite{green2007provenance} with non-negative values. The \emph{input size} of $\I$ is defined as the sum of frequencies of data records, i.e., $\displaystyle{n = \sum_{i \in [m]} \sum_{t \in \D_i} R^\I_i(t)}$. When the context is clear, we just drop the superscript $\I$ from $R^\I_j$, and often use $R_j = \{t\in \D_j: R_j(t) >0\}$ to denote the set of tuples with non-zero frequency.\pasin{This notion $R_j$ is pretty confusing to me. Do we really need it?}
 
 For each $i \in [m]$, we have a family $\Q_i$ of linear queries defined over $\D_i$ such that for $q \in \Q_i$, $q: \D_i \to [-1,+1]$. The family of linear queries defined over $\I$ is $\Q  = \times_{i \in [m]}\Q_i$. For each linear query $q = (q_1, q_2, \cdots, q_m) \in \Q$, the result is defined as
 \[ q(\I) = \sum_{\vec{t}= (t_1, t_2, \cdots, t_m) \in \times_{i \in [m]}\D_i} \rho\left(\vec{t}\right) \prod_{i \in [m]} q_i(t_i) \cdot R_i(t_i) \]
 where $\rho: \times_{i \in [m]}\D_i \to \{0,1\}$ is the natural join function, such that for each combination $\vec{t} \in \times_{i \in [m]}\D_i$,  $\rho(\vec{t}) = 1$ if and only if $\pi_{\x_i \cap \x_j} t_i = \pi_{\x_i \cap \x_j} t_j$ for each pair of $i,j \in [m]$. Here, $\pi$ is the standard projection operator, such that $\pi_x t$ indicates the value(s) that tuple $t$ displays on attribute(s) $x$.
 
 Our goal is to release a function $\F: \times_{i \in [m]}\D_i \to \mathbb{N}$ such that all queries in $\Q$ can be answered over $\F$ as accurately as possible, i.e., minimizing the $\ell_\infty$-error $\displaystyle{\alpha = \max_{q \in \Q} |q(\I) - q(\F)|}$, where  
 \begin{align*}
    q(\F) &= \sum_{(t_1, t_2, \cdots, t_m) \in \times_{i \in [m]}\D_i}  \F(t_1, t_2, \cdots, t_m) \prod_{i\in [m]} q_i(t_i). 
 \end{align*}
 % \pasin{I intentionally removed the following paragraph because it is far from clear that the error has to depend e.g. on $n(\I)$. For example, in the single-table case, the error when we take $n \to \infty$, depends only on the query set (and privacy parameters of course).}
 %We study the data complexity~\cite{vardi1982complexity} of this problem, i.e., assume that the query size, namely $m$, is a constant. Hence, the error only depends on the input-dependent quantities, such as input size $n(\I)$.
 
%  \badih{Need to specify which of these two models we study in the paper? E.g., in Definition~\ref{def:neighboring} below?}
 \paragraph{DP Setting.} Two DP settings have been studied in the relational model, depending on whether foreign key constraints are
 considered or not. The one considering foreign key constraints assumes the existence of a primary private table, and deleting a tuple in the primary private relation will delete all other tuples referencing it; see~\cite{kotsogiannis2019privatesql, tao2020computing, dong2022r2t}. In this work, we adopt the other notion, which does not consider foreign key constrains, but defines instances to be neighboring if one can be converted into the other by adding/removing a single tuple; this is the same as the notion studied in previous works~\cite{johnson2018towards, kifer2011no, narayan2012djoin, proserpio2014calibrating}.
%  \badih{Cite some papers, in particuarl, some that don't consider foreign key constraints.}
 %As all instances have the same input size, we simply assume that $n$ is public.
 %More formally, our neighboring notion is as follows
 \footnote{Our definition corresponds to the \emph{add/remove} variant of DP where a record is added/removed from a single database $R_i$. Another possible definition is based on \emph{substitution} DP. Add/remove DP implies substitution DP with only a factor of two increase in the privacy parameters; therefore, all of our results also apply to substitution DP.}%:
 
 \begin{definition}[Neighboring Instance]\label{def:neighboring-addremove}
     A pair of instances $\I = (R_1, \cdots, R_m)$ and $\I' = (R'_1, \cdots, R'_m)$ are {\em neighboring} if there exist some $i \in [m]$ and $t^* \in \D_i$ such that:
    \begin{itemize}[leftmargin=*]
        \item for any $j \in [m] - \{i\}$, $R_j(t) = R'_j(t)$ for every $t \in \D_j$;
        \item $R_i(t) = R'_i(t)$ for every $t \in \D_i - \{t^*\}$ and $|R_i(t^*) - R'_i(t^*)| = 1$.
    \end{itemize}
 \end{definition}

%We note that the above definition corresponds to the \emph{add/remove} variant of DP where a record is added/removed from a single database $R_i$. Another possible definition is based on the \emph{substitution} variant of DP; we remark that add/remove DP implies substitution DP with only a factor of two increase in the privacy parameters; therefore, all of our results here also apply to the substitution variant of DP.

\begin{definition}[Differential Privacy~\cite{dwork2006calibrating,dwork2006our}]
    For $\epsilon,\delta>0$, a randomized algorithm $\mathcal{A}$ is \emph{$(\epsilon, \delta)$-differentially private} (denoted by $(\epsilon, \delta)$-DP) if for any pair $\I$, $\I'$ of neighboring instances and any subset $\mathcal{S}$ of outputs,
   $\Pr(\mathcal{A}(\I) \in \mathcal{S}) \le e^\epsilon \cdot \Pr(\mathcal{A}(\I') \in \mathcal{S}) + \delta$.
   %, which is also denoted by $\mathcal{A}(\I) \sim_{(\epsilon, \delta)} \mathcal{A}(\I')$.
\end{definition}

\paragraph{Notation.}
For simplicity of presentation, we henceforth assume throughout that $0 < \eps \leq O(1)$ and $0 \leq \delta \leq 1/2$. Furthermore, all lower bounds below hold against an algorithm that achieves the stated error $\alpha$ \emph{with probability $1 - \beta$ for some sufficiently small constant $\beta > 0$}; we will omit mentioning this probabilistic part for brevity.
%
For notational ease, we define the following quantities:
\[
\flo(\mathbb{D}, \Q, \epsilon) = \sqrt{\frac{1}{\epsilon} \cdot \log |\Q| \cdot
\sqrt{\log |\D|}}, \mbox{ and }
\]
\[
\fup(\mathbb{D}, \Q, \epsilon, \delta) = \flo(\mathbb{D}, \Q, \epsilon) \cdot \sqrt{\log 1/\delta}.
\]
%\[
%\fup(\mathbb{D}, \Q, \epsilon, \delta) = \left(\frac{1}{\epsilon} \cdot \log |\Q| \cdot \log \frac{1}{\delta} \cdot \log^{\frac{1}{2}} |\D|\right)^\frac{1}{2}
%\]
%Note that these two quantities are only a factor of $\log^{1/2}(1/\delta)$ apart.
When $\D, \Q, \eps, \delta$ are clear from context, we will omit them.  Let $\lambda = \frac{1}{\epsilon} \log \frac{1}{\delta}$, which is a commonly-used parameter in this paper.

\subsection{Prior Work}

We first review the problem of releasing synthetic data for a single table, and mention two important results in the literature. In the single table case, nearly tight upper and lower bounds are known, as stated below.

\begin{theorem}[\cite{hardt2012simple}]
\label{the:single-table}
    For a single table $R$ of at most $n$ records, a family $\Q$ of linear queries, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that is $(\epsilon, \delta)$-DP, and with probability at least $1- 1/\mathrm{poly}(|\Q|)$ produces $\F$ such that all queries in $\Q$ can be answered within error $\displaystyle{\alpha =O\left(\sqrt{n} \cdot \fup\right)}$ using $\F$.
\end{theorem}

%We next generalize it to the settings that neighboring instances have distances as $\Delta$ for $\Delta > 1$. The corollary below follows Theorem~\ref{the:single-table}, whose proof is deferred to Appendix~\ref{appendix:single-table}.

%\begin{corollary}
%\label{cor:single-table-sensitivity}
%    For a single table $R$ of $n$ records with sensitivity $\Delta$, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that preserves $(\epsilon, \delta)$-DP, and with probability at least $1- 1/\textsf{poly}(|Q|)$ produces $\F$ such that all queries in $\Q$ can be answered within error $\displaystyle{\alpha =O\left(\left(n \cdot \Delta\right)^{\frac{1}{2}} \cdot \left(\frac{1}{\epsilon} \cdot \log |\Q| \cdot \log \frac{1}{\delta} \cdot \log^{\frac{1}{2}} |\D|\right)^\frac{1}{2}\right)}$.
%\end{corollary}

%We define $f(\mathbb{D}, \Q, \epsilon, \delta) = \left(\frac{1}{\epsilon} \cdot \log |\Q| \cdot \log \frac{1}{\delta} \cdot \log^{\frac{1}{2}} |\D|\right)^\frac{1}{2}$.
%In the remaining of this paper, we usually hide this factor within the notation\pasin{I'm not sure I understand this notion $O_f(\cdot)$. In the TCS convention, this would mean that we fix $f$ to be a constant but clearly this cannot be true because e.g. if we fix $f$ to be constant then $n$ is bounded and all the other terms are already $O_f(1)$. Maybe I'm not understanding the usage here correctly?} $O_f(\cdot)$, since both $\log |\Q|$ and $\log^{\frac{1}{2}} |\D|$ are enlarged by a factor of $m$, the number of tables, which is considered as a constant. 
%\badih{What's the smallest error that can be achieved for single-table synthetic data generation?} Resolved.

\begin{theorem}[\cite{bun2018fingerprinting}]
\label{the:lb-single-table}
    For every sufficiently small $\eps, \alpha>0$, $n_D \ge (1/\alpha)^{\Omega(1)}$ and $n_Q \leq (1/\alpha)^{O(1)}$, there exists a family $\Q$ of queries of size $n_Q$ on a domain $\D$ of size $n_D$ such that any $(\epsilon, o(1/n))$-DP algorithm that takes as input a database of size at most $n$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ must satisfy $\displaystyle{\alpha \geq \tOmega\left(\sqrt{n} \cdot \flo\right)}$.
    %requires that 
    %$\displaystyle{n \ge \widetilde{\Omega}\left(\frac{\sqrt{d} \log |\Q|}{\epsilon \cdot (\frac{\alpha}{n})^2}\right)}$.%\pasin{Note: this needs to be some sort of probabilistic statement?}
\end{theorem}

Another related problem that has been widely studied by the database community is how to release the answer of join size queries over multiple tables with DP, denoted as $\countsize(\cdot)$:
\[\countsize(\I) =  \sum_{\vec{t} = (t_1, t_2, \dots, t_m) \in \times_{i \in [m]}\D_i} \rho\left(\vec{t}\right) \prod_{i \in [m]} R_i(t_i),\]
which can be captured by a special linear query $q = (q_1, q_2, \dots, q_m)$ such that $q_i: \D_i \to \{+1\}$ for $i \in [m]$. 

\ravi{The following para needs rephrasing}\xiao{Just rewrite this part, and please check!}

A popular approach of answering the counting join size query is based on
the sensitivity framework, which first computes $\countsize(\I)$, then computes the sensitivity of the query (measuring the difference between the query answers on
neighboring database instances), and releases a noise-masked query answer, where the noise is
drawn from some %zero-mean 
distribution calibrated appropriately according to the sensitivity. It is known that the local sensitivity $LS_\countsize(\cdot)$ cannot be directly used for calibrating noise, as $LS_\countsize(\I), LS_\countsize(\I')$ for a pair of neighboring databases can lead to distinguishability of $\I,\I'$. Global sensitivity (e.g.,~\cite{dwork2006calibrating}) could be used, but the utility is not satisfactory in many instances. Instead, smooth upper bounds on local sensitivity~\cite{nissim2007smooth} have been considered, for example, the {\em smooth sensitivity}, which is the smallest smooth upper bound, the {\em residual sensitivity}~\cite{dong2021residual}, which is a constant-approximation to the smooth sensitivity, and the {\em elastic sensitivity}~\cite{johnson2018towards}, which is further strictly larger than residual sensitivity.

We note that this sensitivity-based framework can be adapted to answering any single linear query, as long as the sensitivity is correctly computed. However, we are not interested in answering each linear query individually, since the privacy budget blows up with the number of queries to be answered,  implied by the DP composition rule~\cite{dwork2006calibrating, dwork2006our}, which would be too costly when the query space is extremely large. Instead, we aim to release a synthetic dataset such that an arbitrary linear query can be freely answered over it while preserving DP. In building our data release algorithm, we also resort to the existing literature on the sensitivities derived for this counting join size query $\countsize(\cdot)$. Although smooth sensitivity enjoys the best utility, we adopt the residual sensitivity in this paper for two reasons: it is much more computationally efficient compared to smooth sensitivity; and more importantly, it is only built on the statistics of the input instance while smooth sensitivity is built on all neighboring instances, which is critical to our optimization technique of uniformizing sensitivities.

%We note that this framework can be adapted to answer any single linear query, as long as the sensitivity Although this framework can be used to answer any single linear query with  the sensitivity computation becomes much more complicated, as a weighted version of $\countsize(\cdot)$. However, we are not interested in answering each linear query individually, since the privacy budget blows up with the number of queries to be answered, which would be too costly when the query space is very large. Our algorithm of releasing a synthetic dataset for answering multiple queries uses the existing results on sensitivity derived for $\countsize(\cdot)$. 
%
%

\subsection{Our Results}
%
\badih{Based on discussion with Xiao, we might need to add more interpretation of the results in this section?} \xiao{I added a few sentences after Theorem 1.6, but not sure if they make sense.}
%
We first present the basic join-as-one approach for releasing a synthetic dataset for multi-table queries, with error a function of the output size of join results and the residual sensitivity of $\countsize(\cdot)$. 

\begin{theorem}
\label{the:ub-multi-table}
     For any join query $\mathcal{H}$, an instance $\I$, a family $\Q$ of linear queries, and $\epsilon > 0$, $\delta > 0$, there exists an $(\epsilon, \delta)$-DP algorithm that with probability at least $1- 1/\textsf{poly}(|\Q|)$ produces $\F$ that can be used to answer all queries in $\Q$ within error:
    \[\alpha = O\left((\sqrt{\OUT \cdot SS^\beta_\countsize(\I) \cdot \lambda} + SS^\beta_\countsize(\I) \cdot \lambda )\cdot \fup \right) \]
    where $\OUT$ is the join size of $\I$ and $SS^\beta_\countsize(\I)$ is the $\beta$-residual sensitivity of the counting join size query $\countsize(\cdot)$ on $\I$ for $\beta = \frac{\epsilon}{2\ln 2/\delta}$ (see Definition~\ref{def:residual}).
\end{theorem}

We next present the parameterized optimality with respect to the output size of join results and local sensitivity of $\countsize(\cdot)$.

\begin{theorem}
\label{the:lb-multi-table}
    Given arbitrary parameters $\OUT \geq \Delta > 0$ and a join query $\mathcal{H}$,
    for every sufficiently small $\eps, \alpha>0$, $n_D \ge (1/\alpha)^{\Omega(1)}$ and $n_Q \leq (1/\alpha)^{O(1)}$, there exists a family $\Q$ of queries of size $n_Q$ on domain $\D$ of size $n_D$ such that any $(\epsilon, o(1/n))$-differentially private algorithm that takes as input a multi-table database over $\mathcal{H}$ of input size at most $n$, join size $\OUT$ and local sensitivity $\Delta$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ must satisfy  \[\alpha \ge \tOmega\left(\sqrt{\OUT \cdot \Delta} \cdot \flo\right).\]
    %Suppose we are given For any join query $\mathcal{H}$, for any parameters $\OUT >0$ and $\Delta > 0$ for $\OUT \ge \Delta$, let $\mathbb{I}(\OUT,\Delta)$ be the class of instances over $\mathcal{H}$ that have join size $\OUT$ and local sensitivity $\Delta$. There exists a set of queries $\Q$ such that any $(\epsilon,\delta)$-DP algorithm that takes as input an instance $\I \in \mathbb{I}(\OUT,\Delta)$ and outputs an approximate answer to each query in $\Q$ within error $\alpha$ must require $\displaystyle{\alpha \ge \Omega\left(\sqrt{\OUT} \cdot \sqrt{\Delta} \cdot \flo + \Delta\right)}$, with probability at least $\exp(-\epsilon) \cdot (1-\delta)$. \badih{In this theorem, $\delta$ is being used to denote both the DP parameter and the failure probability?}\xiao{the probability is inherited from Theorem~\ref{the:lb-two-table-1}.}
\end{theorem}

 It should be noted that for the setting with $\epsilon = \Omega(1)$ and $\delta = O\left(\frac{1}{n^c}\right)$ for some constant $c$, we just have $\lambda = O\left(\log n\right)$. %for some query-dependent constant $c$.\pasin{Isn't $\lambda$ just $O(\log n)$ here?} 
The gap between the upper bound in Theorem~\ref{the:ub-multi-table} and the lower bound in Theorem~\ref{the:lb-multi-table} boils down to the gap between smooth sensitivity and local sensitivity of $\countsize(\cdot)$, which also appears (but in a different formula) in answering such a single query.\pasin{Moved instance-optimality discussion to the conclusion.}


\pasin{Our upper bound above is in terms of smooth sensitivity but lower bound is in terms of local sensitivity. Do we need to state a connection between the two?} \xiao{I added a few sentences here, but not sure if they make sense.}

From the upper bound in terms of residual sensitivity, we exploit the idea of {\em uniformizing sensitivity}\footnote{Similar idea of uniformizing degrees of join values, i.e., how many tuples a join value appears in a relation, has been used in query processing~\cite{joglekar2015s}, but we use it in a more complicated scenario in combination of sensitivity.}\badih{Per discussion with Xiao, since the previous work used ``uniformization'' to refer to a much simpler technique, we might want to consider using a different term to avoid confusion?} to further improve Theorem~\ref{the:ub-multi-table}, by using a more fine-grained characterization of input instances. For the class of hierarchical queries, which has been widely studied in the context of various database problems~\cite{dalvi2007efficient, fink2016dichotomies, berkholz2017answering, hu2022temporal}, we obtain a more fine-grained parameterized upper bound in Theorem~\ref{the:ub-hierarhical-uniformize} and lower bound in Theorem~\ref{the:lb-hierarhical-uniformize}. As the utility formula display a rather complicated form, we defer all details to Section~\ref{sec:uniformization}. 




==> backup-laplace/intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

 Synthetic data release is a very useful objective in private data analysis. Differential privacy \cite{dwork2006calibrating,dwork2006our} has emerged as a compelling model that enables us to formally study the tradeoff between utility of released information and the privacy of individuals. In the literature, there has been a large body of work that studies synthetic data release over a single table, for example, the private multiplicative weight algorithm~\cite{hardt2012simple}, the histogram-based algorithm~\cite{vadhan2017complexity}, the matrix mechanism~\cite{li2010optimizing}, the Bayesian network algorithm\cite{zhang2017privbayes}; and some specialized works for geometric range queries~\cite{li2011efficient, li2012adaptive, dwork2010differential, bun2015differentially, chan2011private, dwork2015pure, cormode2012differentially, huang2021approximate}, and datacubes~\cite{ding2011differentially}. 

Data analysis over multiple private tables connected via join operators has been the subject of significant interest within the area of modern database systems. In particular, the challenging question of releasing the counting join size over a set of private tables has been studied in several recent works including the sensitivity-based framework~\cite{johnson2018towards, dong2021residual,dong2021nearly} and truncation-based mechanism~\cite{kotsogiannis2019privatesql, dong2022r2t, tao2020computing}; and some specialized works for one-to-one join~\cite{mcsherry2009privacy,proserpio2014calibrating}, and graph database~\cite{blocki2013differentially, chen2013recursive}. In practice, multiple queries instead of a single query are typically issued for data analysis, for example, a large class of linear queries on top of join results with different weights on input tuples, as a variant of counting join size query. One might consider answering each query independently but the utility would be very bad due to the limited privacy budget \badih{Do we want to somehow mention here that this would be applying DP composition?}. Hence, how can we release synthetic data for answering such a large class of linear queries over a set of multiple tables in a differentially private way? In this paper, we take the first step in answering this question with theoretical guarantees.

\badih{Do we need to cite previous work on DP SQL queries? Actually, looks like we already added two such citations: the Johnson et al. paper and the Privatesql paper.}

\subsection{Problem Definition}

 \paragraph{Multi-way Join and Linear Queries.} A (natural) join query can be represented as a hypergraph $\mathcal{H} = (\x, \{\x_1, \x_2, \cdots, \x_m\})$~\cite{abiteboul1995foundations}, where $\x$ is the set of vertices or attributes and each $\x_i \subseteq \x$ is a hyperedge or relation. Let $\dom(x)$ be the domain of attribute $x$. Define $\displaystyle{\D = \dom(\x) = \prod_{x \in \x} \dom(x)}$, and $\displaystyle{\D_i = \dom(\x_i) = \prod_{x \in \x_i} \dom(x)}$ for any $i \in [m]$. Given an input instance $\I = \left(R^\I_1, R^\I_2, \cdots, R^\I_m\right)$, each table $R^\I_i: \D_i \to \mathbb{Z}^+$ %\pasin{Is it standard for the range to be $0, 1$? Or do we people generally consider the range to be $\Z$ as well?} Resolved.
 is defined as a function from domain $\D_i$ to a non-negative integer, indicating the frequency of each tuple. This is more general than the setting that each tuple appears at most once in each relation, since it can capture annotated relations with non-negative values. The input size of $\I$ is defined as the sum of frequencies of data records, i.e., $\displaystyle{n = \sum_{i \in [m]} \sum_{t \in \D_i} R^\I_i(t)}$. When the context is clear, we just drop the script $\I$ from $R^\I_j$, and often use $R_j = \{t\in \D_j: R_j(t) >0\}$ to denote the set of tuples with non-zero frequency.\pasin{This notion $R_j$ is pretty confusing to me. Do we really need it?}
 
 For each $i \in [m]$, we have a family of linear queries $\Q_i$ defined over $\D_i$ such that for $q \in \Q_i$, $q: \D_i \to [-1,+1]$. The family of linear queries defined over $\I$ is $\Q  = \times_{i \in [m]}\Q_i$. For each linear query $q = (q_1, q_2, \cdots, q_m) \in \Q$, the result is defined as
 \[ q(\I) = \sum_{\vec{t}= (t_1, t_2, \cdots, t_m) \in \times_{i \in [m]}\D_i} \rho\left(\vec{t}\right) \prod_{i \in [m]} q_i(t_i) \cdot R_i(t_i) \]
 where $\rho: \times_{i \in [m]}\D_i \to \{0,1\}$ is the natural join function, such that for each combination $\vec{t} \in \times_{i \in [m]}\D_i$,  $\rho(\vec{t}) = 1$ if and only if $\pi_{\x_i \cap \x_j} t_i = \pi_{\x_i \cap \x_j} t_j$ for each pair of $i,j \in [m]$, where $\pi$ is the standard projection operator, such that $\pi_x t$ indicates the value(s) that tuple $t$ displays on attribute(s) $x$.
 
 Our target is to release a function $\F: \times_{i \in [m]}\D_i \to \mathbb{N}$ such that all queries in $\Q$ can be answered over $\F$ as accurately as possible, i.e., minimizing the $\ell_\infty$-error $\displaystyle{\alpha = \max_{q \in \Q} |q(\I) - q(\F)|}$, where  
 \begin{align*}
    q(\F) &= \sum_{(t_1, t_2, \cdots, t_m) \in \times_{i \in [m]}\D_i}  \F(t_1, t_2, \cdots, t_m) \prod_{i\in [m]} q_i(t_i). 
 \end{align*}
 % \pasin{I intentionally removed the following paragraph because it is far from clear that the error has to depend e.g. on $n(\I)$. For example, in the single-table case, the error when we take $n \to \infty$, depends only on the query set (and privacy parameters of course).}
 %We study the data complexity~\cite{vardi1982complexity} of this problem, i.e., assume that the query size, namely $m$, is a constant. Hence, the error only depends on the input-dependent quantities, such as input size $n(\I)$.
 
 \paragraph{DP Settings.} Two DP models \badih{Need to specify which of these two models we study in the paper? E.g., in Definition~\ref{def:neighboring} below?} have been studied in the relational model, depending on whether foreign key constraints are
 considered. One considering foreign key constrains assumes the existence of a single primary private table, and deleting a tuple in the primary private relations will delete all other tuples referencing to it; see~\cite{kotsogiannis2019privatesql, tao2020computing, dong2022r2t}. \xiao{We adopt the other one not considering foreign key constrains, which is the same as \cite{johnson2018towards, kifer2011no, narayan2012djoin, proserpio2014calibrating}, that defines the neighboring instances if they can be converted into each other by updating one tuple.} \badih{Cite some papers, in particuarl, some that don't consider foreign key constraints.} As all instances have the same input size, we simply assume that $n$ is public.
 
 \begin{definition}\label{def:neighboring}
     A pair of instances $\I = (R_1, \cdots, R_m)$ and $\I' = (R'_1, \cdots, R'_m)$ are {\em neighboring} if there exists some $i \in [m]$ such that:
    \begin{itemize}[leftmargin=*]
        \item for any $j \in [m] - \{i\}$, $R_j(t) = R'_j(t)$ for every $t \in \D_j$;
        \item there exists $t_1,t_2 \in \D_i$ such that $R_i(t) = R'_i(t)$ for every $t \in \D_i - \{t_1,t_2\}$ with $R_i(t_1) - R'_i(t_1) = 1$ and $R_i(t_2) - R'_i(t_2) = -1$.
    \end{itemize}
 \end{definition}

\begin{definition}[\cite{dwork2006calibrating,dwork2006our}]
    For $\epsilon,\delta>0$, $\mathcal{A}$ is $(\epsilon, \delta)$-differentially private if for any pair of neighboring instances $\I$, $\I'$ and any subset of outputs $\mathcal{S}$,
   $\Pr(\mathcal{A}(\I) \in \mathcal{S}) \le e^\epsilon \cdot \Pr(\mathcal{A}(\I') \in \mathcal{S}) + \delta$,
    which is also denoted by $\mathcal{A}(\I) \sim_{(\epsilon, \delta)} \mathcal{A}(\I')$.
\end{definition}

\subsection{Previous Results on Answering Multiple Queries over a Single Table}

We first review the problem of releasing synthetic data for a single table, and mention two important results in the literature. 
\begin{theorem}[\cite{hardt2012simple}]
\label{the:single-table}
    For a single table $R$ of $n$ records, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that preserves $(\epsilon, \delta)$-DP, and with probability at least $1- 1/\textsf{poly}(|Q|)$ produces $\F$ such that all queries in $\Q$ can be answered within error $\displaystyle{\alpha =O\left(n^{\frac{1}{2}} \cdot \left(\frac{1}{\epsilon} \cdot \log |\Q| \cdot \log \frac{1}{\delta} \cdot \log^{\frac{1}{2}} |\D|\right)^\frac{1}{2}\right)}$.
\end{theorem}

We next generalize it to the settings that neighboring instances have distances as $\Delta$ for $\Delta > 1$. The corollary below follows Theorem~\ref{the:single-table}, whose proof is deferred to Appendix~\ref{appendix:single-table}.

\begin{corollary}
\label{cor:single-table-sensitivity}
    For a single table $R$ of $n$ records with sensitivity $\Delta$, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that preserves $(\epsilon, \delta)$-DP, and with probability at least $1- 1/\textsf{poly}(|Q|)$ produces $\F$ such that all queries in $\Q$ can be answered within error $\displaystyle{\alpha =O\left(\left(n \cdot \Delta\right)^{\frac{1}{2}} \cdot \left(\frac{1}{\epsilon} \cdot \log |\Q| \cdot \log \frac{1}{\delta} \cdot \log^{\frac{1}{2}} |\D|\right)^\frac{1}{2}\right)}$.
\end{corollary}

We define $f(\mathbb{D}, \Q, \epsilon, \delta) = \left(\frac{1}{\epsilon} \cdot \log |\Q| \cdot \log \frac{1}{\delta} \cdot \log^{\frac{1}{2}} |\D|\right)^\frac{1}{2}$. In the remaining of this paper, we usually hide this factor within the notation\pasin{I'm not sure I understand this notion $O_f(\cdot)$. In the TCS convention, this would mean that we fix $f$ to be a constant but clearly this cannot be true because e.g. if we fix $f$ to be constant then $n$ is bounded and all the other terms are already $O_f(1)$. Maybe I'm not understanding the usage here correctly?} $O_f(\cdot)$, since both $\log |\Q|$ and $\log^{\frac{1}{2}} |\D|$ are enlarged by a factor of $m$, the number of tables, which is considered as a constant. 
%\badih{What's the smallest error that can be achieved for single-table synthetic data generation?} Resolved.

\begin{theorem}[\cite{bun2018fingerprinting}]
\label{the:lb-single-table}
    For every sufficiently small $\alpha>0$, $d \ge \log \frac{1}{\alpha}$, there exists a family of queries $\Q$ of size at least $\frac{d}{\alpha^2}$ such that any $(\epsilon, \delta)$-differentially private algorithm that takes as input a database $D \in (\{0,1\}^d)^n$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ requires that 
    $\displaystyle{n \ge \widetilde{\Omega}\left(\frac{\sqrt{d} \log |\Q|}{\epsilon \cdot (\frac{\alpha}{n})^2}\right)}$.\pasin{Note: this needs to be some sort of probabilistic statement?}
\end{theorem}

\subsection{Previous Results on Answering Single Counting Query over Multiple Tables}

Another related problem that has been widely studied by database community is how to release the answer of counting join size query under DP, denoted as $\countsize(\cdot)$:
\[\countsize(\I) =  \sum_{\vec{t} = (t_1, t_2, \cdots, t_m) \in \times_{i \in [m]}\D_i} \rho\left(\vec{t}\right) \prod_{i \in [m]} R_i(t_i),\]
which can be captured by a special linear query $q = (q_1, q_2, \cdots, q_m)$ such that $q_i: \D_i \to \{+1\}$ for $i \in [m]$. 

A popular approach is
the sensitivity framework, which computes $\countsize(\I)$, computes some notions of sensitivity of the query (measuring the difference between the query answers on
neighboring database instances), and then releases a noise-masked query answer, where the noise is
drawn from some %zero-mean 
distribution calibrated appropriately according to the sensitivity. Although this framework can be carried over to answering any single linear query, the computation of sensitivity becomes much more complicated, as a weighted version of $\countsize(\cdot)$. However, we are not interested in answering each linear query individually, since the privacy budget blows up with the number of queries to be answered, which would be too costly when the query space is very large. Our algorithm of releasing a synthetic dataset for answering multiple queries uses the existing results on sensitivity derived for $\countsize(\cdot)$. 
%
%
It is known that the local sensitivity $LS_\countsize(\cdot)$ cannot be directly used for calibrating noise, as $LS_\countsize(\I), LS_\countsize(\I')$ for a pair of neighboring databases can lead to distinguishability of $\I,\I'$ \badih{Not sure if we want to add a citation for this fact?}. Global sensitivity~\cite{} could be used, but the utility is not ideal in many instances. Instead, people have considered smooth upper bounds on local sensitivity~\cite{nissim2007smooth}, for example the {\em smooth sensitivity}, which is the smallest smooth upper bound, and the {\em residual sensitivity}~\cite{dong2021residual}, which is a constant-approximation of smooth sensitivity.
%
Although smooth sensitivity enjoys the best utility, we adopt residual sensitivity in this paper for two reasons: it is much more computationally efficient than smooth sensitivity; and more importantly, it is only built on the statistics of input databases itself while smooth sensitivity built on its all neighboring instances, which is critical in building our optimization algorithm in Section~\ref{sec:hierarchical}. 

\subsection{Our Results}

\badih{Based on discussion with Xiao, we might need to add more interpretation of the results in this section?}

We first present the basic join-as-one approach for releasing a synthetic dataset for multi-table queries, with error a function of the output size of join results and the residual sensitivity. Let $\lambda = \frac{1}{\epsilon} \log \frac{1}{\delta}$, which is a commonly-used parameter in this paper.

\begin{theorem}
\label{the:ub-multi-table}
     For any join query $\mathcal{H}$, an instance $\I$, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that preserves $(\epsilon, \delta)$-DP, and with probability at least $1- \frac{1}{\textsf{poly}(|\Q|)}$ produces $\F$ that all queries in $\Q$ can be answered within error:
    \[\alpha = O_f\left(\sqrt{\OUT} \cdot \sqrt{SS^\beta_\countsize(\I) \cdot \lambda} + SS^\beta_\countsize(\I) \cdot \lambda \right) \]
    where $\OUT$ is the join size of $\I$ and $SS^\beta_\countsize(\I)$ is the $\beta$-residual sensitivity of counting join size $\countsize(\cdot)$ on $\I$ for $\beta = \frac{\epsilon}{2\ln 2/\delta}$.
\end{theorem}

We next show the parameterized optimality with respect to the output size and local sensitivity. It should be noted that taking the choice of  $\epsilon = O(1)$ and $\delta = O\left(\frac{1}{n^c}\right)$ for some constant $c$, we have $\lambda = O\left(\log^c n\right)$ for some query-dependent constant $c$.  The gap between the upper bound in Theorem~\ref{the:ub-multi-table} and the lower bound in Theorem~\ref{the:lb-multi-table} boils down to the inherent gap between local sensitivity and smooth sensitivity, which also exists in answering the single counting join size query. Moreover, this gap is \badih{tight?} up to logarithmic factors \badih{factors?} on the simplest two-table join query.

\begin{theorem}
\label{the:lb-multi-table}
     For any join query $\mathcal{H}$, for any parameters $\OUT >0$ and $\Delta > 0$ for $\OUT \ge \Delta$, let $\mathbb{I}(\OUT,\Delta)$ be the class of instances over $\mathcal{H}$ that have join size $\OUT$ and local sensitivity $\Delta$. There exists a set of queries $\Q$ such that any $(\epsilon,
     \delta)$-DP algorithm that takes as input an instance $\I \in \mathbb{I}(\OUT,\Delta)$ and outputs an approximate answer to each query in $\Q$ within error $\alpha$ must require $\displaystyle{\alpha \ge \Omega\left(\sqrt{\OUT} \cdot \sqrt{\Delta} + \Delta\right)}$, with probability at least $\exp(-\epsilon) \cdot (1-\delta)$. \badih{In this theorem, $\delta$ is being used to denote both the DP parameter and the failure probability?}\xiao{the probability is inherited from Theorem~\ref{the:lb-two-table-1}.}
\end{theorem}

\pasin{Our upper bound above is in terms of smooth sensitivity but lower bound is in terms of local sensitivity. Do we need to state a connection between the two?}
From the error complexity in terms of residual sensitivity, we exploit the technique of {\em uniformizing degrees}\footnote{\xiao{Similar idea have been used in query processing~\cite{joglekar2015s}, but we use it in a more complicated scenario.}} \badih{Per discussion with Xiao, since the previous work used ``uniformization'' to refer to a much simpler technique, we might want to consider using a different term to avoid confusion?} to further improve Theorem~\ref{the:ub-multi-table} and Theorem~\ref{the:lb-multi-table}. For the class of hierarchical queries, which has been widely studied in various contexts of database problems~\cite{dalvi2007efficient, fink2016dichotomies, berkholz2017answering, hu2022temporal}\badih{Should we add a citation to indicate that this class of queries is well-studied in database theory research?}, we obtain a more fine-grained parameterized upper and lower bound in Theorem~\ref{the:ub-hierarhical-uniformize} and Theorem~\ref{the:lb-hierarhical-uniformize}, which are deferred to Section~\ref{sec:uniformization}. 




==> backup-laplace/multi-table-backup.tex <==
\subsection{Multi-table Query}

We next extend the join-as-one approach to multi-table query. The general framework shares the common spirit as Algorithm~\ref{alg:two-table}, but involves a non-trivial usage of residual sensitivity. Before diving into the algorithm, we formally define the residual sensitivity. For a join query $\mathcal{H} = (\x, \{\x_1,\x_2,\cdots,\x_m\})$, the residual query on a subset $E \subseteq [m]$ of relations is $H_E = \Join_{i\in E} R_i$. Its boundary, denoted as $\partial_{E}$, is the set of attributes that belong to relations both in and out of $E$, i.e.,
$\partial E = \{x|x \in \textbf{x}_i \cap \textbf{x}_j, i \in E, j \notin E\}$. For a residual query $H_E$ on instance $\I$, the query result is\footnote{The semi-join result of $R \ltimes t$ is defined as $\left\{t' \in R: R(t')>0, \pi_{\x_i} t' = \pi_{\x_i} t\right\}$.}:
\begin{equation}
\label{eq:TE}
    T_E(\I) = \max_{t \in \dom(\partial E)} |H_E(\I) \ltimes t|
\end{equation}
 which is a join-aggregate queries over attributes in $\partial E$. Now, we can use residual query to define the residual sensitivity.
 
 \begin{definition}[Residual Sensitivity for Counting Query~\cite{dong2021residual, dong2021nearly}] Given $\beta > 0$, the $\beta$-residual sensitivity of counting the output size of multi-way join $\mathcal{H}$ over instance $\I$ is defined as $SS^\beta_\countsize(\I) = \max_{k\ge 0} e^{-\beta k} \min\left\{\hat{LS}^{(k)}_\countsize(\I), GS_\countsize\right\}$, where
    \begin{equation}
    \label{eq:residual}
        \hat{LS}^{(k)}_\countsize(\I) =  \max_{\s \in \mathcal{S}^k} \max_{i \in [m]} \sum_{E' \subseteq [m] -\{i\} }T_{[m]-\{i\}-E'}(\I) \cdot \prod_{j \in E'} \s_j 
     \end{equation}
     \begin{equation*}
         GS_\countsize = \max_{i \in [m]} n^{\rho(\x-\x_i, \{\x_1 -\x_i, \x_2 - \x_i, \cdots, \x_m -\x_i\})} \quad \quad \quad \quad 
     \end{equation*}
    for $\mathcal{S}^k = \left\{\s = (\s_1, \s_2, \cdots, \s_m): \sum_{i=1}^m \s_i = k, \s_i \in \mathbb{Z}, \forall i \in [m]\right\}$, and $\rho(\cdot)$ is the optimal fractional edge covering number\footnote{For a hypergraph $(\x, \{\x_1,\x_2,\cdots,\x_m\})$, a fractional edge covering is a length-$m$ vector $\Vec{x}$ such that $\Vec{x}_i \ge 0$ and $\sum_{i: x \in \x_i} \Vec{x}_i \ge 1$. The number of $\Vec{x}$ is defined as $\sum_{i\in[m]} \Vec{x}_i$. }.
 \end{definition}


Now, we are ready to present our general algorithm using residual sensitivity. As described in Algorithm~\ref{alg:multi-table}, we first compute the join results over $\I$ as $J$, and the $\beta$-residual sensitivity of $\countsize(\cdot)$ over $\I$ as $SS^\beta_\countsize(\I)$. After obtaining $SS^\beta_\countsize(\I)$, adding noise to $|J|$ to
achieve DP is straightforward, for example, the Laplacian or Cauchy mechanism~\cite{nissim2007smooth}.  However, we might end up with a negative value, leading to a invalid initial distribution for single-table algorithm (line 4-5). 
%\pasin{I'm not sure why we're using SS and not LS here. Can you please explain more? Is this because LS can now have large sensitivity?} 
To guarantee the correctness, we derive a strict upper bound on $SS^\beta_\countsize(\I)$, denote as $\widetilde{\Delta}$, which also satisfies $(\epsilon, \delta)$-DP. We use this noisy random variable $\widetilde{\Delta}$ to calibrate the truncated and shifted geometric distribution, draw a random variable from $\textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}$, and add it to the true join size as $\widehat{n}$. Finally, we invoke the single-table algorithm to $J$, with initial distribution parameterized by $\widehat{n}$. This upper bound of $SS^\beta_\countsize(\I)$ is also used in parameterizing the exponential mechanism (line 7), and masking the query answer (line 8). 

\begin{algorithm}[t]
\caption{{\sc JoinMultiTable}$(\I = \{R_1,R_2, \cdots, R_m\})$}
\label{alg:multi-table}

$J = \Join_{i \in [m]} R_i$\;
$\beta \gets \frac{\epsilon}{2\ln 2/\delta}$\;
$\widetilde{\Delta} \gets  \max \left \{SS^\beta_\countsize(\I),  SS^\beta_\countsize(\I) \cdot e^{\frac{\beta}{\epsilon} \cdot \textsf{Lap}_1(x) + \frac{1}{2}} \right\}$\;
$\widehat{n} = |J| + \textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}(x)$\; 
$\F_0 \gets \widehat{n}$ times uniform distribution over $\D$: $\F_0(x) = \frac{\widehat{n}}{|\D|}$\;
\ForEach{$i = 1, 2, \cdots, T$}{
    Sample a query $q_i \in \Q$ using the EM parameterized with $\frac{\epsilon}{2T \cdot \widetilde{\Delta}}$ and score function $s_i(J,q) = |q(\F_{i-1}) - q(J)|$\;
    $m_i \gets q_i(J) + \textsf{STGeom}_{\frac{\epsilon}{2T}, \delta, \widetilde{\Delta}}(x)$\;
    Update for each $x \in \D$: $\F_i(x) \propto \F_{i-1}(x) \times \exp\left(q_i(x) \cdot \left(m_i - q_i(\F_{i-1})\right) \cdot \frac{1}{2 \widehat{n}}\right)$\;
}
\Return $\textsf{Avg} \left(\sum_{i=1}^T \F_i\right)$\;
\end{algorithm}

\begin{lemma}
\label{lem:multi-table-DP}
    Algorithm~\ref{alg:multi-table} preserves $(4\epsilon, 4 \delta)$-DP.
\end{lemma}

%The proof of Lemma~\ref{lem:multi-table-DP} is given in Appendix~\ref{appendix:join-as-one}.

\paragraph{Error analysis} With probability at least $1 - \delta$, $\widetilde{\Delta} = O\left(SS_\countsize(\I)\right)$, and therefore $\widehat{n} = O\left(|J| + SS_\countsize(\I)\cdot \lambda \right)$. Putting everything together, the error that can be achieved is (omitting $\fup$): 
\[O\left(\sqrt{\widehat{n}} \cdot \sqrt{\widetilde{\Delta}} \right) = O\left(\sqrt{|J| \cdot SS_\countsize(\I) \cdot \lambda} + SS_\countsize(\I) \cdot \lambda \right)\]

The upper bound is given in Theorem~\ref{the:ub-multi-table}. Moreover, extending the previous lower bound argument on the two-table query, we can obtain the lower bound on the multi-table query in Theorem~\ref{the:lb-multi-table}. 



==> backup-laplace/mutil-table.tex <==
\subsection{Multi-Table Query}

%We next extend the join-as-one approach to multi-table query by using the same primitive in Algorithm~\ref{alg:pmw}, but involving a non-trivial incorporation of residual sensitivity. 

We next extend the join-as-one approach to multi-table query. First, notice that \Cref{alg:two-table} does not work in multi-table setting because $\LS_{\countsize}(\I)$ may itself have a large local sensitivity, unlike in the two table case where the global sensitivity was one.

%Before diving into the algorithm, we formally define the residual sensitivity in Definition~\ref{def:residual}. 
To handle this, we will need the notion of \emph{the residual sensitivity}.
For a join query $\mathcal{H} = (\x, \{\x_1,\x_2,\dots,\x_m\})$, the \emph{residual query} on a subset $E \subseteq [m]$ of relations is $ \Join_{i\in E} R_i$. Its \emph{boundary}, denoted as $\partial_{E}$, is the set of attributes that belong to relations both in and out of $E$, i.e.,
$\partial E = \{x \mid x \in \textbf{x}_i \cap \textbf{x}_j, i \in E, j \notin E\}$. For a residual query on $E$ over instance $\I$, the query result is\footnote{The semi-join result of $R_i \ltimes t$ is defined as function $R'_i: \D_i \to \mathbb{Z}^+$ such that $R_t(t') = R(t')$ if $\pi_{\x_i} t' = \pi_{\x_i} t$ and $0$ otherwise.}:
\begin{equation}
\label{eq:TE}
    T_E(\I) = \max_{t \in \dom(\partial E)} \big|\Join_{i \in [m]} (R_i \ltimes t)\big|,
\end{equation}
 which is a join-aggregate queries over attributes in $\partial E$. %Now, we can use residual query to define the residual sensitivity.
 
 \begin{definition}[Residual Sensitivity for Counting Query~\cite{dong2021residual, dong2021nearly}] 
 \label{def:residual}
 Given $\beta > 0$, the \emph{$\beta$-residual sensitivity} of counting the join size of multi-way query $\mathcal{H}$ over instance $\I$ is defined as %%$SS^\beta_\countsize(\I) = \max_{k\ge 0} e^{-\beta k} \cdot \min\left\{\hat{LS}^{(k)}_\countsize(\I), GS_\countsize\right\}$, where
 \[SS^\beta_\countsize(\I) = \max_{k\ge 0} e^{-\beta k} \cdot \hat{LS}^{(k)}_\countsize(\I),\] 
 where
    \begin{equation}
    \label{eq:residual}
        \hat{LS}^{(k)}_\countsize(\I) =  \max_{\s \in \mathcal{S}^k} \max_{i \in [m]} \sum_{E' \subseteq [m] -\{i\} }T_{[m]-\{i\}-E'}(\I) \cdot \prod_{j \in E'} \s_j,
     \end{equation}
     %\begin{equation*}
     %    GS_\countsize = \max_{i \in [m]} n^{\rho(\x-\x_i, \{\x_1 -\x_i, \x_2 - \x_i, \dots, \x_m -\x_i\})}, \quad \quad \quad \quad 
     %\end{equation*}
    for $\mathcal{S}^k = \left\{\s = (\s_1, \s_2, \dots, \s_m): \sum_{i=1}^m \s_i = k, \s_i \in \mathbb{Z}, \forall i \in [m]\right\}$. %and $\rho(\cdot)$ is the optimal fractional edge covering number\footnote{For a hypergraph $(\x, \{\x_1,\x_2,\dots,\x_m\})$, a \emph{fractional edge covering} is a length-$m$ vector $\Vec{x}$ such that $\Vec{x}_i \ge 0$ and $\sum_{i: x \in \x_i} \Vec{x}_i \ge 1$. The number of $\Vec{x}$ is defined as $\sum_{i\in[m]} \Vec{x}_i$. }.
 \end{definition}

It is clear that $SS^\beta_\countsize(\I)$ is an upper bound on $\LS_\countsize(\I)$, and therefore it suffices for us to find an upper bound $\tDelta$ for $SS^\beta_\countsize(\I)$ (which is then passed to the single-table algorithm). To compute $\tDelta$, we observe that $\ln(SS^\beta_\countsize(\I))$ has global sensitivity at most $\beta$. Therefore, adding an appropriately calibrated (truncated and shifted) Laplace noise to it provides a DP upper bound. The idea is formalized in \Cref{alg:multi-table}. Its privacy guarantee is immediate:

%Now, we are ready to present our general algorithm using residual sensitivity. As described in Algorithm~\ref{alg:multi-table}, we first compute the $\beta$-residual sensitivity of $\countsize(\cdot)$ over $\I$ as $SS^\beta_\countsize(\I)$. Note that adding noise calibrated by $SS^\beta_\countsize(\I)$ for
%answering the counting join size query $\countsize$ is straightforward to achieve DP~\cite{dong2021residual}, for example, the Laplace or Cauchy mechanism~\cite{nissim2007smooth}.  %However, we might end up with a negative answer, leading to a invalid initial distribution for single-table algorithm (line 4). 
%However, we require the estimate (denoted by $\tDelta$) to be an upper bound on the true value of $SS^\beta_\countsize(\I)$ in order to ensure the privacy for single-table algorithm (line 4).
%Our computation of $\tDelta$ relies on the fact that $SS^\beta_\countsize(\I) \le e^\beta \cdot SS^\beta_\countsize(\I')$, which implies that $\tDelta$ is $(\eps/2, \delta/2)$-DP.
%\pasin{I'm not sure why we're using SS and not LS here. Can you please explain more? Is this because LS can now have large sensitivity?} 
%To guarantee the correctness, we derive a strict upper bound on $SS^\beta_\countsize(\I)$, denote as $\tDelta$, which also satisfies $(\epsilon, \delta)$-DP since $SS^\beta_\countsize(\I) \le e^\beta \cdot SS^\beta_\countsize(\I')$ holds for any pair of neighboring instances $\I,\I'$. 
%Similarly, we add $\textsf{Geom}_{\exp(0.5\epsilon/\tDelta)}(x)$ random noise to $\countsize(\I)$ as $\widehat{n}$, and then invoke the single-table algorithm on $J$ starting with a uniform distribution parameterized by $\widehat{n}$. %We add $\textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}$, and add it to the true join size as $\widehat{n}$. 
%Finally, we invoke the single-table algorithm to $J$, with initial distribution parameterized by $\widehat{n}$. 
%This upper bound of $SS^\beta_\countsize(\I)$ is also used in parameterizing the EM, and masking the query answer. 
%As $\Tilde{\Delta}$ satisfies DP, $\widehat{n}$ is released under DP and the single-table algorithm~\cite{hardt2012simple} satisfies under DP, Algorithm~\ref{alg:multi-table} also satisfies DP, as stated in Lemma~\ref{lem:multi-table-DP}.

\begin{algorithm}[t]
\caption{{\sc JoinMultiTable}$(\I = \{R_1,R_2, \dots, R_m\})$}
\label{alg:multi-table}

%$J = \Join_{i \in [m]} R_i$\;
$\beta \gets \frac{\epsilon}{2\ln 2/\delta}$\;
$SS^\beta_\countsize(\I) \gets \beta$-residual sensitivity of $\countsize(\I)$\;
$\tDelta \gets  \max \left \{SS_\countsize(\I),  SS_\countsize(\I) \cdot e^{\frac{1}{2} + \textsf{Lap}_{\eps/2\beta}} \right\}$\;
\Return $\textsc{PMW}_{\eps/2,\delta/2,\tDelta}(\I)$\; 
\end{algorithm}
\pasin{I changed the notation of Lap the exponent a bit (in Algorithm 3). Might need to be propagated to the proofs} \pasin{I don't think we've define Laplace distribution before Algorithm 3. Might need to do that.}

\begin{lemma}
\label{lem:multi-table-DP}
    Algorithm~\ref{alg:multi-table} is $(\epsilon,  \delta)$-DP.
\end{lemma}

%The proof of Lemma~\ref{lem:multi-table-DP} is given in Appendix~\ref{appendix:join-as-one}.

\paragraph{Error analysis.} With probability at least $1 - \delta$, $|\textsf{Lap}_{\eps/2\beta}| < 1/2$, then $\frac{1}{2} + \textsf{Lap}_{\eps/2\beta}\in [0,1]$ since $\beta = \frac{\epsilon}{2 \ln 2/\delta}$, and therefore $\tDelta \in [SS^\beta_\countsize(\I), SS^\beta_\countsize(\I) \cdot e]$. Hence $\widehat{n} = O\left(\OUT + SS_\countsize(\I)\cdot \lambda \right)$. Putting everything together, the error can be achieved is (omitting $\fup$): 
\[O\left(\sqrt{\widehat{n}} \cdot \sqrt{\tDelta} \right) = O\left(\sqrt{\OUT \cdot SS^\beta_\countsize(\I) \cdot \lambda} + SS^\beta_\countsize(\I) \cdot \lambda \right)\]

The upper bound is given in Theorem~\ref{the:ub-multi-table}. Moreover, extending the previous lower bound argument on the two-table query, we can obtain the lower bound on the multi-table query in Theorem~\ref{the:lb-multi-table}. 



==> backup-laplace/pasin-scratch.tex <==
\section{Pasin's Scratch Pad}

\subsection{Add-Remove DP}

\pasin{This is not a strong suggestion but I think it is a little bit more convenient to use the add-remove DP which anyway also implies substitution DP.}

It will be more convenient to work with the \emph{add-remove} notion of differential privacy, as defined below.

 \begin{definition}\label{def:neighboring-addremove}
     A pair of instances $\I = (R_1, \cdots, R_m)$ and $\I' = (R'_1, \cdots, R'_m)$ are {\em neighboring} if there exists some $i \in [m]$ such that:
    \begin{itemize}[leftmargin=*]
        \item for any $j \in [m] - \{i\}$, $R_j(t) = R'_j(t)$ for every $t \in \D_j$;
        \item there exists $t^* \in \D_i$ such that $R_i(t) = R'_i(t)$ for every $t \in \D_i - \{t^*\}$ with $|R_i(t^*) - R'_i(t^*)| = 1$.
    \end{itemize}
 \end{definition}

We note that the above notion corresponds to the so-called \emph{add-remove} DP where a record is added / removed from a single database $R_i$. Another possible definition is the \emph{substitution} DP; we remark that add-remove DP implies substitution DP with only a factor of two increase in the privacy parameters; therefore, all of our results here also apply to the substitution DP setting.


\subsection{Additional Preliminaries}

\pasin{We probably need the following in our prelims.}

\paragraph{Exponential Mechanism.}
The exponential mechanism (EM)~\cite{McSherryT07} can select a ``good'' candidate from a set $\cC$ of candidates. The goodness here is defined by a scoring function $s(\I, c)$ for input dataset $\I$ and a candidate $c \in \cC$ which should have sensitivity at most one. Then, the EM algorithm is to sample each candidate $c \in \cC$ with probability proportional to $\exp\left(-0.5\eps \cdot s(\I, c)\right)$. When the scoring function has sensitivity at most one, this algorithm is $\eps$-DP.

\subsection{Private Multiplicative Weight Algorithm}

\pasin{The following is my suggestion on how to rephrase the multiplicative weight algorithm. I think it is not a very good idea to repeat this part several times in different algorithm with unclear guarantee. Having something like the following should allow us to avoid repetition and be clear about what exactly we need.}

For an instance $\I = (R_1, \cdots, R_m)$, we write $\joindat{\I}$ as a shorthand for $R_1 \Join \cdots \Join R_m$. Furthermore, for two sets $S, T$, we write $S \setdiff T$ as a shorthand for the symmetric set difference between $S$ and $T$, i.e. $(S \setminus T) \cup (T \setminus S)$. 

%For $k \in \N$, we say that $\I$ and $\I'$ are $k$-neighbors, denoted by $\I\sim_t \I'$, iff there is a sequence $\I_0 = \I, \dots, \I_k = \I'$ such that $\I_{i - 1}, \I_i$ are neighbors for all $i \in [k]$.

A central parameter for our investigation is the (symmetric set) difference between the Join of $\I$ and that of its neighbor $\I'$, i.e. $(\joindat{\I}) \setdiff (\joindat{\I'})$. Its importance stems from the fact that this quantity upper bounds the local sensitivity of any linear queries:

\begin{observation}
For any linear query $q$, we have $|q(\I) - q(\I')| \leq |(\joindat{\I}) \setdiff (\joindat{\I'})|$. Consequently, $\LS_q(\I) \leq \max_{\I' \sim \I} |(\joindat{\I}) \setdiff (\joindat{\I'})|$.
\end{observation}

\pasin{One advantage of removal notion is that $\max_{\I' \sim \I} |(\joindat{\I}) \setdiff (\joindat{\I'})|$ exactly coincides with the LS of $\countsize$ at $\I$.}

A priori, the quantity $\max_{\I' \sim \I} |(\joindat{\I}) \setdiff (\joindat{\I'})|$ can be arbritrarily large. However, as we will see below, we can often estimate it well. Indeed, if we have an upper bound $\tDelta$ on this quantity, then the private multiplicative weight (PMW) algorithm of~\cite{hardt2012simple} from the single table setting can be easily applied to our setting. The algorithm is described in \Cref{alg:pmw} and its guarantees (which follows almost directly from \cite{hardt2012simple}) are stated in \Cref{thm:pmw}.

%Here it takes an additional parameter $\tDelta$ which represents an ``upper bound on the local sensitivity''. 

\begin{algorithm}[t]
\caption{{\sc PMW}$_{\eps, \delta, \tDelta}(\I = \{R_1,R_2, \cdots, R_m\})$}
\label{alg:pmw}
$\widehat{n} = \max\{1, |\joindat{J}| + \textsf{Geom}_{\exp(0.5\epsilon/\tDelta)}(x)\}$\; 
$\F_0 \gets \widehat{n}$ times uniform distribution over $\D$: $\F_0(x) = \frac{\widehat{n}}{|\D|}$\;
$\eps' \leftarrow \frac{\eps}{16 \sqrt{T \cdot \log(1/\delta)}}$\;
\ForEach{$i = 1, 2, \cdots, T$}{
    Sample a query $q_i \in \Q$ using the $\eps'$-DP EM with score function $s_i(\I,q) = \frac{1}{\tDelta}|q(\F_{i-1}) - q(\I)|$\;
    $m_i \gets q_i(\I) + \textsf{Geom}_{\eps', \tDelta}(x)$\;
    Update for each $x \in \D$: $\F_i(x) \propto \F_{i-1}(x) \times \exp\left(q_i(x) \cdot \left(m_i - q_i(\F_{i-1})\right) \cdot \frac{1}{2 \widehat{n}}\right)$\;
}
\Return $\textsf{Avg} \left(\sum_{i=1}^T \F_i\right)$\;
\end{algorithm}


\begin{theorem} \label{thm:pmw}
Let $\I, \I'$ be such that $|(\joindat{\I}) \setdiff (\joindat{\I'})| \leq \tDelta$. Then, \Cref{alg:pmw} satisfies the following:
\begin{itemize}[leftmargin=*]
\item (Privacy) $\PMW(\I) \sim_{(\eps, \delta)} \PMW(\I')$.
\item (Utility) With probability at least $1 - 1/\poly(|\Q|)$, $\PMW(\I)$ produces a dataset such that all queries in $\Q$ can be answered to within error $\displaystyle{\alpha =O\left(\left(n \cdot \tDelta\right)^{\frac{1}{2}} \cdot \fup\right)}$.
\end{itemize}
\end{theorem}





==> backup-laplace/prelim.tex <==
\section{Preliminaries}

For random variables $X, Y$ and scalars $\eps >0, \delta \in [0, 1)$, we write $X \sim_{(\eps, \delta)} Y$ if $\Pr[X \in S] \leq e^\eps \cdot \Pr[Y \in S] + \delta$ and $\Pr[Y \in S] \leq e^\eps \cdot \Pr[X \in S] + \delta$ for all sets $S$ of outcomes.

For convenience, we write $a + \cD$ as a shorthand for $a + X$ where $X$ is a random variable with distribution $\cD$ (denoted by $X \sim \D$).

\paragraph{Laplacian distribution~\cite{}.} \new{to be done.}

\paragraph{Shifted and truncated geometric distribution~\cite{chan2019foundations}.} Let $\textsf{Geom}_\alpha(x) \\= \frac{\alpha-1}{\alpha+1} \cdot \alpha^{-|x|}$. Let $\epsilon > 0$, $\delta \in (0, 1)$, and $\Delta \ge 1$.
Let $n_0$ be the smallest positive integer such that $\displaystyle{\Pr\left[\left|\textsf{Geom}_{\exp(\epsilon/\Delta)}(x) \right| \ge n_0\right] \le \delta}$,
where $n_0 \leq \frac{\Delta}{\epsilon} \log \frac{2}{\delta} + 1$. The \emph{shifted and truncated geometric distribution} $\textsf{STGeom}_{\epsilon, \delta, \Delta}(x)$ has support in $[0, 2\cdot(n_0 + \Delta-1)]$, and is defined as 
$\displaystyle{\min\left\{\max \left\{0, n_0 + \Delta - 1 + \textsf{Geom}_{\exp(\frac{\epsilon}{\Delta})}(x)\right\}, 2(n_0 + \Delta - 1)\right\}}$. It has been proved~\cite{balcer2017differential, chan2019foundations} that for any pair  $u,v$ with $|u -v| \le \Delta$,
\[u + \textsf{STGeom}_{\epsilon, \delta, \Delta} \sim_{(\epsilon, \delta)} v + \textsf{STGeom}_{\epsilon, \delta, \Delta}\]
%and 
\[u + \textsf{Geom}_{\exp(\eps/\Delta)} \sim_{(\epsilon, 0)} v + \textsf{Geom}_{\exp(\eps/\Delta)}\]

\paragraph{Exponential Mechanism.}
The exponential mechanism (EM)~\cite{McSherryT07} can select a ``good'' candidate from a set $\cC$ of candidates. The goodness is defined by a \emph{scoring function} $s(\I, c)$ for input dataset $\I$ and a candidate $c \in \cC$ and is assumed have sensitivity at most one. Then, the EM algorithm is to sample each candidate $c \in \cC$ with probability $\propto \exp\left(-0.5\eps \cdot s(\I, c)\right)$; this algorithm is $(\eps, 0)$-DP.

\paragraph{Local Sensitivity.} Given a function $f$ that takes an input dataset and outputs a vector, its \emph{$(\ell_1-)$local sensitivity} at $\I$ is defined as $s_f(\I) := \max_{\I'} \|f(\I') - f(\I)\|_1$ where the maximum is over all neighbors $\I'$ of $\I$. %The global sensitivity of $f$, denoted by $s_f$, is defined as $\max_{\I} s_f(\I)$.

\paragraph{Join Result as a Function.} For $\I = (R_1,R_2,\cdots, R_m)$, as each input relation is abstracted as a function, we introduce the \emph{join result function} as $J = \Join_{i \in [m]} R_i$, such that $J\left(\vec{t}\right) = \prod_{i \in [m]} R_i\left(\pi_{\x_i} \vec{t}\right)$ for any $\vec{t} \in \D$. Moreover, $\countsize(\I) = |J| = \sum_{\vec{t} \in \D} J\left(\vec{t}\right)$ is denoted as {\em join size} of $\I$, and we might exchangably use them later.

When we mention ``local sensitivity'' without a specific function $f$, it should be assumed that the function is the counting join size query; note that this is equal to $\LS_{\countsize}(\I)$.

\pasin{Should we add definitions of global and smoothed sensitivity here?}

==> backup-laplace/three-table.tex <==


%Note that $2^{i+j}$
%We consider an instance $\I$ for this join query (see Figure~\ref{fig:line-3}). Let $\dom(B) = \{b_1,b_2,\cdots, b_{\sqrt{n}}\}$ and $\dom(C) = \{c_1,c_2,\cdots, c_{\sqrt{n}}\}$. For any $i \in [\sqrt{n}]$, every value $b_i \in \dom(B)$ forms a tuple with $c_j$ for each $j \in \{\sqrt{n}-i+1,\sqrt{n}-i+2, \cdots, \sqrt{n}\}$. On this instance, $T_E$ can be simplified as:
%$\displaystyle{\max\left\{\max_{b \in \dom(B)} \degg_2(B,b), \max_{c \in \dom(C)} \degg_2(C,c)\right\}}$. Uniformizing $\I$ boils down to finding a partition $(R^1_2, R^2_2, \cdots, R^k_2)$ of $R_2$, to minimize the error achieved by Algorithm~\ref{alg:uniformization-framework}. Note that  Algorithm~\ref{alg:multi-table} can achieve an error of $O\left(n^{3/4}\right)$ on this instance. As proved in Appendix~\ref{appendix:uniformization}, every possible partition leads to an error at least $\Omega(n^{3/4})$, thus establishing a gap of uniformization on hierarchical and non-hierarchical join queries.

\newpage


==> backup-laplace/two-table-backup.tex <==
\subsection{Upper Bound on Two-Table Query}
We start with the simplest two-table case. For simplicity, assume $\mathcal{H}$ has $\x = \{A,B,C\}$, $\x_1 = \{A,B\}$ and $\x_2 = \{B,C\}$. Let's define some parameters first. For $i \in [2]$, the degree of join value $b \in \dom(B)$ %\pasin{What is $B$? Is this the set of all attributes?}in $R_i$ is denoted as $\degg_i(B,b)$, the frequencies of data records displaying join value $b$ in $R_i$, i.e., resolved
$\displaystyle{\degg_i(B, b) = \sum_{t \in \D_i:\pi_B t=b} R_i(t)}$. The maximum degree of any join value in $R_i$ is denoted as 
$\displaystyle{\Delta_i = \max_{b \in \dom(B)} \degg_i(B, b)}$. Define $\Delta = \max\{\Delta_1, \Delta_2\}$.
We note that $LS_\countsize(\I) = \Delta$. \badih{Has $LS_\countsize(\I)$ been defined anywhere? Also, is the last sentence a fact or a definition?}


\paragraph{Shifted and truncated geometric distribution~\cite{chan2019foundations}.} Let $\textsf{Geom}_\alpha(x) \\= \frac{\alpha-1}{\alpha+1} \cdot \alpha^{-|x|}$. Let $\epsilon > 0$, $\delta \in (0, 1)$ and $\Delta \ge 1$.
Let $n_0$ be the smallest positive integer such that $\displaystyle{\Pr\left[\left|\textsf{Geom}_{\exp(\frac{\epsilon}{\Delta})}(x) \right| \ge n_0\right] \le \delta}$,
where $n_0 \leq \frac{\Delta}{\epsilon} \log \frac{2}{\delta} + 1$. The shifted and truncated geometric distribution $\textsf{STGeom}_{\epsilon, \delta, \Delta}(x)$ has support in $[0, 2\cdot(n_0 + \Delta-1)]$, and is defined as 
$\displaystyle{\min\left\{\max \left\{0, n_0 + \Delta - 1 + \textsf{Geom}_{\exp(\frac{\epsilon}{\Delta})}(x)\right\}, 2(n_0 + \Delta - 1)\right\}}$. It has been proved~\cite{balcer2017differential, chan2019foundations} \badih{Need to add some citation here.} that for any pair of $u,v$ with $|u -v| \le \Delta$,
\[u + \textsf{STGeom}_{\epsilon, \delta, \Delta}(x) \sim_{(\epsilon, \delta)} v + \textsf{STGeom}_{\epsilon, \delta, \Delta}(x).\]

\paragraph{Join result as a function.} As each input relation is a function, we introduce the natural join result function $J = \Join_{i \in [m]} R_i$, such that $J\left(\vec{t}\right) = \prod_{i \in [m]} R_i\left(\pi_{\x_i} \vec{t}\right)$ for any $\vec{t} \in \D$. Moreover, $|J| = \sum_{\vec{t} \in \D} J\left(\vec{t}\right)$.

\paragraph{A Strawperson Idea.} Let us first consider a flawed strawperson, which turns out to violate DP:
\begin{itemize}[leftmargin=*]
    \item Compute $J = \Join_{i\in[m]} R_i$ \badih{Need to formally define the $\Join$ notation somewhere?} and then release a synthetic dataset for $J$ as $\widetilde{J}_1$ using a single-table algorithm. However, this is not enough since the single-table algorithm releases exactly $|J| = \countsize(\I)$ records, which will reveal the information of input database. 
    \item We then draw a random noise from $\textsf{STGeom}_{\epsilon, \delta, 1}(x)$ and add it to $\Delta$ as $\widetilde{\Delta}$. Then, we draw a random noise from $\textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}(x)$ as $\lambda$, and choose $\lambda$ records randomly from $\mathbb{D}_1 \times \mathbb{D}_2$ denoted as $\widetilde{J_2}$. %\badih{This should be $\widetilde{J}_2?$} resolved
    \item At last, we release the union of these two datasets $\F = \widetilde{J}_1 \cup \widetilde{J}_2$.
\end{itemize}
The challenge is that invoking the single-table algorithm on $J$ does not satisfy DP, as the initial uniform data distribution parameterized by $|J|$ can lead to the leakage of input database. 


\begin{algorithm}[t]
\caption{{\sc JoinTwoTable}$(\I = \{R_1, R_2\})$}
\label{alg:two-table}

$J = R_1 \Join R_2$\;
$\Delta \gets LS_\countsize(\I)$\;
$\widetilde{\Delta} \gets \Delta + \textsf{STGeom}_{\epsilon, \delta, 1}(x)$\;
$\widehat{n} = |J| + \textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}(x)$\; 
$\F_0 \gets \widehat{n}$ times uniform distribution over $\D$: $\F_0(x) = \frac{\widehat{n}}{|\D|}$\;

\ForEach{$i = 1, 2, \cdots, T$}{
    Sample a query $q_i \in \Q$ using the EM parameterized with $\frac{\epsilon}{2T\cdot \widetilde{\Delta}}$ and score function $s_i(J,q) = |q(\F_{i-1}) - q(J)|$\;
    $m_i \gets q_i(J) + \textsf{STGeom}_{\frac{\epsilon}{2T}, \delta, \widetilde{\Delta}}(x)$\;
    Update for each $x \in \D$: $\F_i(x) \propto \F_{i-1}(x) \times \exp\left(q_i(x) \cdot \left(m_i - q_i(\F_{i-1})\right) \cdot \frac{1}{2\widehat{n}}\right)$\;
}
\Return $\textsf{Avg} \left(\sum_{i=1}^T \F_i\right)$\;
\end{algorithm}

\paragraph{Modified Algorithm.} As shown in Algorithm~\ref{alg:two-table}, we need to change the order of two steps in the strawperson version. After computing function $J$, we add $\textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}(x)$ random noise to $|J|$ as $\widehat{n}$, and then invoke the single-table algorithm on $J$ starting with a uniform distribution parameterized by $\widehat{n}$. As $\widehat{n}$ is released under DP, and the single-table algorithm~\cite{hardt2012simple} also releases a synthetic dataset for $J$ under DP, Algorithm~\ref{alg:two-table} also satisfies DP, as stated in Lemma~\ref{lem:two-table-DP}.

\begin{lemma}
\label{lem:two-table-DP}
    Algorithm~\ref{alg:two-table} preserves $(3\epsilon, 3\delta)$-DP.
\end{lemma}


\paragraph{Error Analysis.} As shown in Appendix~\ref{appendix:single-table}, with probability at least $1 - \frac{1}{\textsf{poly}(\Q)}$, Algorithm~\ref{alg:two-table} produces $\F = \textsf{Avg} \sum_{i=1}^T \F_i$ such that every linear query can be answered within error:
\[\alpha = O_f\left(\sqrt{|J|} \cdot \sqrt{\Delta + \lambda} + \Delta + \lambda \right).\]

\begin{theorem}
\label{the:up-2table}
     For any two-tables instance $\I$, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that preserves $(\epsilon, \delta)$-DP, and with probability at least $1- \frac{1}{\textsf{poly}(|\Q|)}$ produces $\F$ on which all queries in $\Q$ can be answered within error:
    \[\alpha = O_f\left(\sqrt{|J|} \cdot \sqrt{LS_\countsize(\I) + \lambda} + LS_\countsize(\I) + \lambda \right).\]
\end{theorem}



==> backup-laplace/two-table-lb-backup.tex <==
\subsection{Lower Bound on Two-Table Query}

%\begin{lemma}[Helper Lemma]
%\label{lem:max}
%    \rev{For any two-table instance $\I$, any algorithm for answering the counting query over $\I$ within error $\alpha$, must have
%    $\big||J| - \countsize(\I)\big| \le \alpha$,
%    where $|J|$ is the join size of $\I$.}
%%\end{lemma}

%\pasin{By selecting queries here, the lemma only holds for some set of queries. Would be good to specified this in the lemma statement itself.} 


\new{
\begin{theorem}
\label{the:lb-two-table-1}
     %\pasin{This should be ``some''? As Badih mentioned the other day, for a particular $\I$, there is a DP algorithm which just outputs the answer for $\I$ always. In the proof here, we do need the algorithm to be accurate on $\I'$ as well. Maybe we need some sort of neighborhood optimality/utility here?} 
     Any $(\epsilon, \delta)$-DP algorithm that takes as input any two-table instance $\I$ and outputs an approximate answer to the counting query within error $\alpha$, requires that
     $\displaystyle{\alpha \ge \Omega \left(LS_\countsize(\I)\right)}$, with probability at least $\exp(-\epsilon) \cdot (1-\delta)$. \badih{The order of quantifiers here is unclear. Did we mean to say that there is an input under which the algorithm will have large error with high probability?}
\end{theorem}
}

\begin{proof}
    Consider an $(\epsilon, \delta)$-DP algorithm $\mathcal{A}$, and a pair of neighboring instances $\I,\I'$. Let $\countsize(\I), \countsize(\I')$ be the join size of $\I, \I'$ respectively. 
    Let $\widetilde{\countsize}(\I), \widetilde{\countsize}(\I')$ be the results released for $\I, \I'$ respectively. From the error guarantee, $\big|\countsize(\I) - \widetilde{\countsize}(\I)\big| \le \alpha$ and $\big|\countsize(\I') - \widetilde{\countsize}(\I')\big| \le \alpha$.
    As $\mathcal{A}$ preserves $(\epsilon, \delta)$-DP, there must be
    \begin{align*}
        1 &= \Pr\left(\widetilde{\countsize}(\I) \in [\countsize(\I)-\alpha, \countsize(\I) + \alpha] \right) \\
        &\le e^\epsilon \cdot \Pr\left(\widetilde{\countsize}(\I') \in [\countsize(\I)-\alpha, \countsize(\I) + \alpha]\right) + \delta 
    \end{align*}
    i.e., $\Pr\left(\widetilde{\countsize}(\I') \in [\countsize(\I)-\alpha, \countsize(\I) + \alpha]\right) \ge e^{-\epsilon}(1-\delta)$. Moreover, $\big|\countsize(\I') - \countsize(\I)\big| \le 2 LS_\countsize(\I)$. If $\alpha < LS_\countsize(\I)$, we observe that $\countsize(\I') + \alpha < \countsize(\I) - \alpha$, or $\countsize(\I') - \alpha > \countsize(\I) + \alpha$, i.e., $\widetilde{\countsize}(\I') \notin [\countsize(\I)-\alpha, \countsize(\I) + \alpha]$. Thus $\alpha > \Omega(LS_\countsize(\I))$ holds with probability at least $\exp(-\epsilon) \cdot (1-\delta)$.
\end{proof}

We note that this theorem can be extended to general joins. 

\begin{theorem}
\label{the:lb-two-table-2}
    Given arbitrary parameters $\OUT>0$ and $\Delta > 0$ for $\Delta \le \OUT$, let $\mathbb{I}(\OUT, \Delta)$ be the class of instances that have join size $\OUT$ and local sensitivity $\Delta$. There exists a family of queries $\Q$ such that any $(\epsilon, \delta)$-DP algorithm that takes as input a database $\I \in \mathbb{I}(\OUT, \Delta)$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ requires that
    \[\alpha \ge \Omega\left(\sqrt{|\OUT|} \cdot \sqrt{\Delta} \cdot (\frac{\log^{1/2} \D \cdot \log |\Q|}{\epsilon})^{1/2}\right).\]
\end{theorem}

\begin{proof}
Set $n= \frac{\OUT}{\Delta}$ and $\D = (\{0,1\}^d)^n$. From Theorem~\ref{the:lb-single-table}, let $\Q_\textsf{one}$ be the set of queries on which any $(\epsilon, \delta)$-DP algorithm that takes as input a single-table database $T \in \D$ and outputs an approximate answer to each query in $\Q_\textsf{one}$ within error $\alpha$ requires that $\alpha \ge \widetilde{\Omega}\left(\sqrt{n} \cdot (\frac{\sqrt{d} \log |\Q_\textsf{one}|}{\epsilon})^{\frac{1}{2}}\right)$. %\pasin{Add citation \& make this more formal?}
For an arbitrary single-table database $T \in \D$, we construct
a two-table instance $\I$ of input size $m$, join size $\OUT$, and local sensitivity $\Delta$ as follows\footnote{Actually, we can construct a two-table instance of input size $m$ for any $m \ge \frac{\OUT}{\Delta}$, which is the minimum requirement under the join size and local sensitivity constraint. For $m > \frac{\OUT}{\Delta}$, we can simply pad $m- \frac{\OUT}{\Delta}$ dummy tuples to $R_1, R_2$ arbitrary, as long as which do not contribute to any join result.}.
\begin{itemize}[leftmargin=*]
    \item Set $\dom(A) = \D$, $\dom(B) = \mathbb{Z}$ and $\dom(C) = \mathbb{Z}$;
    \item Set $\D_1 = \dom(A) \times \dom(B)$ and $\D_2 = \dom(B) \times \dom(C)$;
    \item Tuples in $R_1$ form a Cartesian product of size $\min\left\{\Delta, \frac{\OUT}{\Delta}\right\} \times \max\left\{1, \frac{\OUT}{\Delta^2}\right\}$ over $\dom(A) \times \dom(B)$;
    \item Tuples in $R_2$ form a Cartesian product of sizes $\max\left\{1, \frac{\OUT}{\Delta^2}\right\} \times \min\left\{\Delta, \frac{\OUT}{\Delta}\right\}$ over $\dom(B) \times \dom(C)$;
    \item For each of the $n$ records in $T$, say $x$, we exclusively choose one tuple $t \in R_1$ and set $\pi_A t = x$. %\pasin{We might have to be a bit more careful about this b/c we have to make sure that the ``chosen'' tuples do not cause ``cascading effect'' and blow up the distance in the new instance.}
\end{itemize}
It can be easily checked that $\I \in \mathbb{I}(\OUT,\Delta)$. 
From $\Q_\textsf{one}$, we construct a set of queries over $\I$ as $\Q_\textsf{two}$. For each query $q \in \Q_\textsf{one}$, we construct another query $q'=(q_1,q_2)$ as follows:
\begin{itemize}[leftmargin=*]
    \item $q_1: \D_1 \to [0,1]$ such that $q_1(t) = q(x)$ if and only if $\pi_A t =x$;
    \item $q_2: \D_2 \to \{+1\}$ over $\D_2$.
\end{itemize}
We also add the counting query $q' = (q_1,q_2)$ with $q_1: \D_1 \to \{+1\}$ and $q_2: \D_2 \to \{+1\}$ to $\Q_\textsf{two}$. An example is illustrated in Figure~\ref{fig:lb-two-table}. 


Our lower bound argument is that if there is an $(\epsilon, \delta)$-DP algorithm that takes any two-table instance in $\mathbb{I}(\OUT, \Delta)$ and outputs an approximate answer to each query in $\Q_\textsf{two}$ within error $\alpha$, then there is a $(\epsilon, \delta)$-DP algorithm that takes any single-table instance $T \in \D$ and outputs an approximate answer to each query in $\Q_\textsf{one}$ within error $\frac{\alpha}{\Delta}$. Let $\mathcal{A}$ be such an arbitrary algorithm that takes any two-table instance in $\mathbb{I}(\OUT, \Delta)$ and outputs an approximate answer to each query in $\Q_\textsf{two}$ within error $\alpha$. Let $\widetilde{q}(\I)$ be the approximate answer for query $q \in \Q_\textsf{two}$. For each query $q \in \Q_\textsf{one}$, the corresponding query $q'\in \Q_\textsf{two}$. Let $\displaystyle{\Lambda = \max_{q'\in \Q_\textsf{two}} |\widetilde{q'}(\I)|}$. For each query $q \in \Q_\textsf{one}$, we just return an approximate answer $\displaystyle{\widetilde{q}(T) = \frac{\widetilde{q'}(\I) \cdot n}{\Lambda}}$, where $q' \in \Q_\textsf{two}$ is the counterpart of $q$ in our construction.

We first note that this algorithm for answering queries in $\Q_\textsf{one}$ preserves $(\epsilon, \delta)$-DP. This is not hard to show, since $\mathcal{A}$ preserves $(\epsilon, \delta)$-DP, and the post-processing is deterministic,  independent of the input instance. We next bound the error of approximate answers for queries in $\Q_\textsf{one}$. For any $q \in \Q_\textsf{one}$ and its counterpart $q' \in \Q_\textsf{two}$, we first point out that $\displaystyle{q'(\I) = q(T) \cdot \Delta}$.
%
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.67]{img/lb-two-table.pdf}
    \caption{Lower bound instance with $n=9$, $\Delta = 3$, $\OUT = 27$. }
    \label{fig:lb-two-table}
\end{figure} 
%
Implied by the error of answering queries in $\Q_\textsf{two}$, we know that
$\displaystyle{\big|q'(\I) - \widetilde{q'}(\I)\big| \le \alpha}$ holds for every query $q' \in \Q_\textsf{two}$.
From the error guarantee on the counting query, $|\Lambda - n \Delta| \le \alpha$.
For any query $q \in \Q_\textsf{one}$, we observe:
    \begin{align*}
       \big|q(T) - \widetilde{q}(T)\big| &= \big|\frac{q'(\I)}{\Delta} - \frac{\widetilde{q'}(\I)}{\Lambda} \cdot n \big| \\
        &= \big|\frac{1}{\Delta} \cdot \left(q'(\I) - \widetilde{q'}(\I) \right)\big| + \big|\left(\frac{1}{\Delta} - \frac{n}{\Lambda}\right) \cdot \widetilde{q'}(\I)\big|\\
        &\le \frac{1}{\Delta} \cdot \alpha + \big|\left(\frac{1}{\Delta} - \frac{n}{\Lambda}\right) \cdot \Lambda \big|  \le \frac{2\alpha}{\Delta}
    \end{align*}
    where the last inequality follows $\big|\left(\frac{1}{\Delta} - \frac{n}{\Lambda}\right) \cdot \Lambda \big| = \frac{1}{\Delta} \cdot \big|\Lambda - n \Delta \big|\le \frac{\alpha}{\Delta}$.
    If $\alpha = o\left(\sqrt{\OUT} \cdot \sqrt{\Delta}\right)$, then there is an $(\epsilon,\delta)$-differentially private algorithm that takes as input any single-table database $T \in \D$ and outputs approximate answers to each query in $\Q_\textsf{one}$ within error $o(\sqrt{n})$, coming to a contradiction of Theorem~\ref{the:lb-single-table}.
\end{proof}

\new{
\begin{theorem}
\label{the:lb-two-table}
    Given arbitrary parameters $\OUT>0$ and $\Delta > 0$ for $\Delta \le \OUT$, let $\mathbb{I}(\OUT, \Delta)$ be the class of instances that have join size $\OUT$ and local sensitivity $\Delta$. There exists a family of queries $\Q$ such that any $(\epsilon, \delta)$-DP algorithm that takes as input a database $\I \in \mathbb{I}(\OUT, \Delta)$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ requires that \[\alpha \ge \Omega\left(\sqrt{\OUT} \cdot \sqrt{\Delta} \cdot (\frac{\log^{1/2} \D \cdot \log |\Q|}{\epsilon})^{1/2}  + \Delta\right).\]
    with probability $\exp(-\epsilon) \cdot (1-\delta)$.
\end{theorem}
}

%\pasin{Following paragraph seems out of place and should be moved somewhere else?}


==> backup-laplace/two-table-lb.tex <==
\subsection{Lower Bounds for Two-Table Query}

%\begin{lemma}[Helper Lemma]
%\label{lem:max}
%    \rev{For any two-table instance $\I$, any algorithm for answering the counting query over $\I$ within error $\alpha$, must have
%    $\big||J| - \countsize(\I)\big| \le \alpha$,
%    where $|J|$ is the join size of $\I$.}
%%\end{lemma}

%\pasin{By selecting queries here, the lemma only holds for some set of queries. Would be good to specified this in the lemma statement itself.} 

The first lower bound is based on the local sensitivity, which can be shown via standard techniques.

\begin{theorem}
\label{the:lb-two-table-1}
     %Given arbitrary parameters $\Delta > 0$, %let $\mathbb{I}(\Delta)$ be the class of instances that have local sensitivity at most $\Delta$.
     For any $\Delta > 0$,
     if there exists a family of queries $\Q$ such that any $(\epsilon, \delta)$-DP algorithm that takes as input a database %$\I \in \mathbb{I}(\Delta)$
     $\I$ with local sensitivity at most $\Delta$
      and outputs an approximate answer to each query in $\Q$ to within error $\alpha$, then $\alpha \ge \Omega\left(\Delta\right)$.
\end{theorem}

%We note that this theorem can be extended to general joins. 
Our second lower bound is via a reduction to the single-table case: we create a two-table instance where $R_1$ encodes the single-table and $R_2$ ``amplifies'' both the sensitivity and the join size by a factor of $\Delta$. This eventually results in the following lower bound.

\begin{theorem}
\label{the:lb-two-table-2}
    %Given arbitrary parameters $\OUT>0$ and $\Delta > 0$ for $\Delta \le \OUT$, let $\mathbb{I}(\OUT, \Delta)$ be the class of instances that have join size $\OUT$ and local sensitivity $\Delta$. There exists a family of queries $\Q$ such that any $(\epsilon, \delta)$-DP algorithm that takes as input a database $\I \in \mathbb{I}(\OUT, \Delta)$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ requires that
    %\[\alpha \ge \tOmega\left(\sqrt{\OUT} \cdot \sqrt{\Delta} \cdot \flo\right).\]
    %For arbitrary parameters $\OUT \geq \Delta > 0$, 
    For any $\OUT \geq \Delta > 0$,
    any sufficiently small $\eps, \alpha>0$, $n_D \ge (1/\alpha)^{\Omega(1)}$ and $n_Q \leq (1/\alpha)^{O(1)}$, if there exists a family $\Q$ of queries of size $n_Q$ on domain $\D$ of size $n_D$ such that any $(\epsilon, o(1/n))$-DP algorithm that takes as input a two-table database of join size $\OUT$ and local sensitivity $\Delta$ and outputs an approximate answer to each query in $\Q$ to within error $\alpha$, then  $\displaystyle{\alpha \ge \tOmega\left(\sqrt{\OUT} \cdot \sqrt{\Delta} \cdot \flo\right)}$.
\end{theorem}

\begin{proof}
Let $n= \frac{\OUT}{\Delta}$. From Theorem~\ref{the:lb-single-table}, there exists a set $\Q_\textsf{one}$ of queries on domain $\D$ for which any $(\epsilon, \delta)$-DP algorithm that takes as input a single-table database $T \in \D$ and outputs an approximate answer to each query in $\Q_\textsf{one}$ within error $\alpha$ requires that $\alpha \ge \tilde{\Omega}\left(\sqrt{n} \cdot \flo(\mathbb{D}, \Q_\textsf{one}, \epsilon)\right)$.
For an arbitrary single-table database $T: \D \to \Z^+$, we construct
a two-table instance $\I$ of join size $\OUT$, and local sensitivity $\Delta$ as follows:%\footnote{Actually, we can construct a two-table instance of input size $m$ for any $m \ge \frac{\OUT}{\Delta}$, which is the minimum requirement under the join size and local sensitivity constraint. For $m > \frac{\OUT}{\Delta}$, we can simply pad $m- \frac{\OUT}{\Delta}$ dummy tuples to $R_1, R_2$ arbitrary, as long as which do not contribute to any join result.}.
\begin{itemize}[leftmargin=*]
    \item Set $\dom(A) = \D$, $\dom(B) = \D \times [n]$ and $\dom(C) = [\Delta]$.
    \item Let $R_1(a, (b_1, b_2)) = \ind[a = b_1 \wedge b_2 \leq T(a)]$ for all $a \in A$ and $(b_1, b_2) \in B$.
    \item Let $R_2(b, c) = 1$ for all $b \in B$ and $c \in C$.
\end{itemize}
%
%\begin{itemize}[leftmargin=*]
%    \item Set $\dom(A) = \D$, $\dom(B) = \mathbb{Z}$ and $\dom(C) = \mathbb{Z}$;
%    \item Set $\D_1 = \dom(A) \times \dom(B)$ and $\D_2 = \dom(B) \times \dom(C)$;
%    \item Tuples in $R_1$ form a Cartesian product of size $\min\left\{\Delta, \frac{\OUT}{\Delta}\right\} \times \max\left\{1, \frac{\OUT}{\Delta^2}\right\}$ over $\dom(A) \times \dom(B)$;
%    \item Tuples in $R_2$ form a Cartesian product of sizes $\max\left\{1, \frac{\OUT}{\Delta^2}\right\} \times \min\left\{\Delta, \frac{\OUT}{\Delta}\right\}$ over $\dom(B) \times \dom(C)$;
%    \item For each of the $n$ records in $T$, say $x$, we exclusively choose one tuple $t \in R_1$ and set $\pi_A t = x$. %\pasin{We might have to be a bit more careful about this b/c we have to make sure that the ``chosen'' tuples do not cause ``cascading effect'' and blow up the distance in the new instance.}
%\end{itemize}
It can be easily checked that $\I$ has join size at most $\OUT$ and local sensitivity $\Delta$, and that two neighboring datasets $T, T'$ result in neighboring $\I, \I'$.
%From $\Q_1$, we construct a set of queries over $\I$ as $\Q_2$. For each query $q \in \Q_\textsf{one}$, we construct another query $q'=(q_1,q_2)$ as follows:
%\begin{itemize}[leftmargin=*]
%    \item $q_1: \D_1 \to [0,1]$ such that $q_1(t) = q(x)$ if and only if $\pi_A t =x$;
%    \item $q_2: \D_2 \to \{+1\}$ over $\D_2$.
%\end{itemize}
%We also add the counting query $q' = (q_1,q_2)$ with $q_1: \D_1 \to \{+1\}$ and $q_2: \D_2 \to \{+1\}$ to $\Q_2$.
% \pasin{I don't think the above is needed since anyway we are defining $Q = Q_1 \times Q_2$ in our problem setting.}
Finally, let $\Q_1$ contain queries from $\Q_\textsf{one}$ applied on its first attribute (i.e., $\Q_1 := \{q \circ \pi_A \mid q \in \Q_\textsf{one}\}$), and let $\Q_2$ contain only a single query $q_\textsf{all-one}: \D_2 \to \{+1\}$.
%
An example is illustrated in 
Figure~\ref{fig:lb-two-table}. 


Our lower bound argument is a reduction to the single-table case. 
%is that if there is an $(\epsilon, \delta)$-DP algorithm that takes any two-table instance in $\mathbf{I}(\OUT, \Delta)$ and outputs an approximate answer to each query in $\Q = \Q_1 \times \Q_2$ within error $\alpha'$, then there is an $(\epsilon, \delta)$-DP algorithm that takes any single-table instance $T \in \D$ and outputs an approximate answer to each query in $\Q_\textsf{one}$ within error $\frac{\alpha'}{\Delta}$. 
Let $\mathcal{A}$ be an algorithm that takes any two-table instance in $\mathbf{I}(\OUT, \Delta)$ and outputs an approximate answer to each query in $\Q$ within error $\alpha'$.  For each query $q \in \Q_\textsf{one}$, let $q' = (q \circ \pi_A, q_\textsf{all-one})$ be its corresponding query in $\Q$. Let $\tq'(\I)$ be the approximate answer for query $\tq'$. We then return $\displaystyle{\tq(T) = \tq'(\I) / \Delta}$ as an approximate answer of $q(T)$.

We first note that this algorithm for answering queries in $\Q_\textsf{one}$ is $(\epsilon, \delta)$-DP due to the post-processing property of DP.  The error guarantee follows immediately from the observation that $q'(\I) = \Delta \cdot q(T)$.
%We next bound the error of approximate answers for queries in $\Q_\textsf{one}$. For any $q \in \Q_\textsf{one}$ and its counterpart $q' \in \Q_\textsf{two}$, we first point out that $\displaystyle{q'(\I) = q(T) \cdot \Delta}$.
%
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.67]{img/lb-two-table.pdf}
    \caption{Lower bound instance with $n=9$, $\Delta = 3$, $\OUT = 27$. }
    \label{fig:lb-two-table}
\end{figure} 
%
%Implied by the error of answering queries in $\Q_\textsf{two}$, we know that
%$\displaystyle{\big|q'(\I) - \widetilde{q'}(\I)\big| \le \alpha}$ holds for every query $q' \in \Q_\textsf{two}$.
%From the error guarantee on the counting query, $|\Lambda - n \Delta| \le \alpha$.
%For any query $q \in \Q_\textsf{one}$, we observe:
%    \begin{align*}
%       \big|q(T) - \widetilde{q}(T)\big| &= \bigg|\frac{q'(\I)}{\Delta} - \frac{\widetilde{q'}(\I)}{\Lambda} \cdot n \bigg| \\
%        &= \bigg|\frac{1}{\Delta} \cdot \left(q'(\I) - \widetilde{q'}(\I) \right)\bigg| + \bigg|\left(\frac{1}{\Delta} - \frac{n}{\Lambda}\right) \cdot \widetilde{q'}(\I)\bigg|\\
%        &\le \frac{1}{\Delta} \cdot \alpha + \bigg|\left(\frac{1}{\Delta} - \frac{n}{\Lambda}\right) \cdot \Lambda \bigg|  \le \frac{2\alpha}{\Delta}
%    \end{align*}
%    where the last inequality follows $\big|\left(\frac{1}{\Delta} - \frac{n}{\Lambda}\right) \cdot \Lambda \big| = \frac{1}{\Delta} \cdot \big|\Lambda - n \Delta \big|\le \frac{\alpha}{\Delta}$.
Therefore, from Theorem~\ref{the:lb-single-table}, we can conclude that $\alpha' \geq \Delta \cdot \tOmega(\sqrt{n} \cdot \flo(\mathbb{D}, \Q_\textsf{one}, \epsilon)) \geq \tOmega\left(\sqrt{\OUT} \cdot \sqrt{\Delta} \cdot \flo\right)$.
\end{proof}

%\new{
%\begin{theorem}
%\label{the:lb-two-table}
%    Given arbitrary parameters $\OUT>0$ and $\Delta > 0$ for $\Delta \le \OUT$, let $\mathbb{I}(\OUT, \Delta)$ be the class of instances that have join size $\OUT$ and local sensitivity $\Delta$. There exists a family of queries $\Q$ such that any $(\epsilon, \delta)$-DP algorithm that takes as input a database $\I \in \mathbb{I}(\OUT, \Delta)$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ requires that \[\alpha \ge \Omega\left(\sqrt{\OUT} \cdot \sqrt{\Delta} \cdot \flo  + \Delta\right).\]
%    with probability $\exp(-\epsilon) \cdot (1-\delta)$.
%\end{theorem}
%}

%Note that, while we prove our lower bounds for the two-table case, it can be trivially extend to the multi-table case. Thereby combining the above two theorems yield \Cref{the:lb-multi-table}.

%\pasin{Following paragraph seems out of place and should be moved somewhere else?}


==> backup-laplace/two-table.tex <==
\subsection{Algorithms for Two-Table Query}
We start with the simplest two-table query. Assume $\mathcal{H}$ is defined on $\x = \{A,B,C\}$, $\x_1 = \{A,B\}$, and $\x_2 = \{B,C\}$. Let us define some parameters first. For $i \in [2]$, we define the \emph{degree} of join value $b \in \dom(B)$ %\pasin{What is $B$? Is this the set of all attributes?}in $R_i$ is denoted as $\degg_i(B,b)$, the frequencies of data records displaying join value $b$ in $R_i$, i.e., resolved
to be $\displaystyle{\degg_i(B, b) = \sum_{t \in \D_i:\pi_B t=b} R_i(t)}$. The \emph{maximum degree} of any join value in $R_i$ is denoted as 
$\displaystyle{\Delta_i = \max_{b \in \dom(B)} \degg_i(B, b)}$. Define $\Delta = \max\{\Delta_1, \Delta_2\}$.
We note that $\Delta = LS_\countsize(\I)$. %\badih{Has $LS_\countsize(\I)$ been defined anywhere? Also, is the last sentence a fact or a definition?}

\paragraph{A Natural (but Flawed) Idea.} Let us first consider a natural approach, which turns out to violate DP:
\begin{itemize}[leftmargin=*]
    \item Compute $J = \Join_{i\in[m]} R_i$ and release a synthetic dataset for $J$ as $\tilde{J}_1$ by invoking the single-table PMW algorithm;
    \item As the PMW algorithm releases a set of records with their total frequencies as $|J|$, which will reveal information of the input instance, we add $\textsf{STGeom}_{\epsilon/2, \delta/2, 1}$ noise to $\Delta$ to obtain $\tDelta$. 
    \item We draw a random noise $\rho$ from $\textsf{STGeom}_{\epsilon/2, \delta/2, \tDelta}$ and choose $\rho$ records randomly from $\mathbb{D}_1 \times \mathbb{D}_2$, denoted as $\tilde{J_2}$. %\badih{This should be $\widetilde{J}_2?$} resolved
    \item We release the union of these two datasets $\F = \tilde{J}_1 \cup \tilde{J}_2$.
\end{itemize}
The challenge is that invoking the single-table algorithm on $J$ does not preserve DP, as the initial data distribution parameterized by $|J|$ can lead to leaking of information about the input database. 

\begin{algorithm}[h!]
\caption{{\sc JoinTwoTable}$(\I = \{R_1, R_2\})$}
\label{alg:two-table}
$\tDelta \gets LS_\countsize(\I) + \textsf{STGeom}_{\epsilon/2, \delta/2, 1}(x)$\;
\Return $\textsc{PMW}_{\eps/2,\delta/2,\tDelta}(\I)$ \hfill $\blacktriangleright$ See \Cref{alg:pmw} \;
\end{algorithm}

\begin{algorithm}[h!]
\caption{{\sc PMW}$_{\eps, \delta, \tDelta}(\I = \{R_1,R_2, \dots, R_m\})$}
\label{alg:pmw}
$\widehat{n} = \max\{1, \countsize(\I) + \textsf{Geom}_{\exp(0.5\epsilon/\tDelta)}\}$\; 
$\F_0 \gets \widehat{n}$ times uniform distribution over $\D$: $\F_0(x) = \frac{\widehat{n}}{|\D|}$\;
$\eps' \leftarrow \frac{\eps}{16 \sqrt{T \cdot \log(1/\delta)}}$\;
\ForEach{$i = 1, 2, \dots, T$}{
    Sample a query $q_i \in \Q$ using the $\eps'$-DP EM with score function $s_i(\I,q) = \frac{1}{\tDelta} \cdot |q(\F_{i-1}) - q(\I)|$\;
    $m_i \gets q_i(\I) + \textsf{Geom}_{\eps', \tDelta}$\;
    Update for each $x \in \D$: $\F_i(x) \propto \F_{i-1}(x) \times \exp\left(q_i(x) \cdot \left(m_i - q_i(\F_{i-1})\right) \cdot \frac{1}{2 \widehat{n}}\right)$\;
}
\Return $\textsf{Avg} \left(\sum_{i=1}^T \F_i\right)$\;
\end{algorithm}

\paragraph{Modified Algorithm.} The main insight is to change the order of two steps in the flawed version. We add $\textsf{Geom}_{\exp(0.5\epsilon/\tDelta)}(x)$ random noise to $\countsize(\I)$ as $\widehat{n}$, and then invoke the single-table algorithm on $J$ starting with a uniform distribution parameterized by $\widehat{n}$. As $\widehat{n}$ is released under DP, and the single-table algorithm~\cite{hardt2012simple} also releases a synthetic dataset for $J$ under DP, Algorithm~\ref{alg:two-table} also satisfies DP, as stated in Lemma~\ref{lem:two-table-DP}.

\begin{lemma}
\label{lem:two-table-DP}
    Algorithm~\ref{alg:two-table} is $(\epsilon, \delta)$-DP.
\end{lemma}


\paragraph{Error Analysis.} As shown in Appendix~\ref{appendix:single-table}, with probability at least $1 - 1/\textsf{poly}(\Q)$, Algorithm~\ref{alg:two-table} produces $\F = \textsf{Avg} \sum_{i=1}^T \F_i$ such that every linear query can be answered within error (omitting $\fup$):
$O\left(\sqrt{|J|} \cdot \sqrt{\Delta + \lambda} + \Delta + \lambda \right)$. Then, we come to the following result:

\begin{theorem}
\label{the:up-2table}
     For any two-table instance $\I$, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that is $(\epsilon, \delta)$-DP, and with probability at least $1- 1/\textsf{poly}(|\Q|)$ produces $\F$ such that all queries in $\Q$ can be answered within error:
    \[\alpha = O\left(( \sqrt{\OUT \cdot (\Delta + \lambda)} + \Delta + \lambda) \cdot \fup\right).\]
    where $\lambda = \frac{1}{\eps} \log \frac{1}{\delta}$, $\OUT = \countsize(\I)$ is the join size of $\I$, and $\Delta = LS_\countsize(\I)$ is the local sensitivity of $\countsize(\cdot)$ on $\I$.
\end{theorem}


==> backup-laplace/uniformize.tex <==
\section{Uniformize Sensitivity} 
\label{sec:uniformization}

So far, we have showed a parameterized algorithm for answering linear queries, whose utility is in terms of the join size and the residual sensitivity. A natural question arises: Can we achieve a more fine-grained parameterized algorithm with better utility? 

\begin{algorithm}[t]
\caption{{\sc Uniformize}$(\I)$}
\label{alg:uniformization-framework}

$\mathbb{I} \gets \textsc{Partition}(\I)$\;
\lForEach{$\I' \in \mathbb{I}$}{
    $\F(\I') \gets \textsc{JoinMultiTable}(\I')$}
\Return $\bigcup_{\I' \in \mathbb{I}}\F(\I')$\;
\end{algorithm}

Let us start with a two-table instance (see Figure~\ref{fig:hard-two-table}), with input size $\Theta(n)$, join size $\OUT = \Theta(n\sqrt{n})$ and local sensitivity $\sqrt{n}$. Algorithm~\ref{alg:two-table} achieves an error of $O(n)$. However, this instance is beyond the scope of Theorem~\ref{the:lb-two-table-2}, as the sensitivity (or degree in this simple scenario) distribution over join values is extremely non-uniform. %It motivates us to seek a tighter upper bound, a tighter lower bound, or both, for this specific instance. 
Revisiting the error complexity in Theorem~\ref{the:up-2table}, we can gain some intuition regarding why Algorithm~\ref{alg:two-table} does not perform well on this instance. The costly term is $O(\sqrt{\OUT} \cdot \sqrt{\Delta})$, where $\Delta$ is the largest degree of join values in the input instance. However, there are many join values whose degree is much smaller than $\Delta$, so a natural idea is to {\em uniformize sensitivities}, i.e., partition the input instance into a set of sub-instances by join values, such that join values with similar sensitivities are put into same sub-instance. After this uniformization, we just invoke our previous join-as-one approach as a primitive on each sub-instance independently, and return the union of synthetic datasets generated for all sub-instances.  The framework of uniformization is illustrated in Algorithm~\ref{alg:uniformization-framework}. (All missing proofs are given in Appendix~\ref{appendix:uniformization}).

\subsection{Uniformize Two-Table}

\xiao{Changed Algorithm 5 as well as the text below. Now $n$ is not explicitly used in the algorithm description, but can be argued that any $i$ with $B^i \neq \emptyset$ must have $i \le \lceil \log (\frac{n}{\lambda}+1) \rceil$. Please check!}

As mentioned, there is quite an intuitive way to uniformize a two-table join.
As described in Algorithm~\ref{alg:partition-2table}, the high-level idea is to bucket join values in $\dom(B)$ by their maximum degree in $R_1$ and $R_2$. To protect the privacy of individual tuples, we add some noise drawn from $\textsf{STGeom}_{\epsilon, \delta, 1}$ to each join value's degree, before determining to 
which bucket it should go. Recall that $\lambda = \frac{1}{\epsilon} \log \frac{1}{\delta}$. Let $\gamma_0 = 0$ and $\gamma_i = 2^i \lambda$ for all $i \in \N$. Conceptually, we divide $[0, n+ \lambda]$ into $\ell = \lceil \log (\frac{n}{\lambda}+1) \rceil$ buckets, where the $i$-th bucket is associated with $(\gamma_{i - 1}, \gamma_i]$ for $i \in [\ell]$. The set of values from $\dom(B)$ whose maximum noisy degree in $R_1$ and $R_2$ falls into the $i$-bucket is denoted as $B^{i}$. For each $i$, we identify tuples in $R_1, R_2$ whose join value falls into $B^{i}$ as $R^{i}_1, R^{i}_2$, which forms the sub-instance $(R^i_1, R^i_2)$. At last, we just return all sub-instances.
Note that $n$ is not explicitly used in Algorithm~\ref{alg:partition-2table} as this is not public, but it is easily to check that there exists no join value with degree more than $n$ under the input size constraint. Hence, it is safe to only consider $i \in [\ell]$ in our analysis.

%\begin{algorithm}[t]
%\caption{{\sc Partition-TwoTable}$(\I=\{R_1, R_2\})$}
%\label{alg:partition-2table}
%
%$\ell \gets \lceil \log (\frac{n}{\lambda}+1) \rceil$\;
%$B^{i} \gets \emptyset$ for each $i \in [\ell]$\;
%\ForEach{$b \in \dom(B)$}{
%\ForEach{$j \in \{1,2\}$}{
%    $\deg_j(B,b) = \degg_j(B,b) + \textsf{STGeom}_{\epsilon, \delta, 1}(x)$\;
%    }
%  
%    $i \gets \max\left\{0, \left\lceil \log \frac{1}{\lambda} \cdot \max\{\deg_1(B, b), \deg_2(B, b)\} \right\rceil\right\}$\;
%    $B^{i} \gets B^{i} \cup \{b\}$\;
%}
%\ForEach{$i \in [\ell]$}{
%    \lForEach{$j\in \{1,2\}$}{
%    $R^{i}_j \gets \{R_j(t): t \in \D_j, \pi_B t \in B^{i}\}$}}
%\Return $\bigcup_{i \in [\ell]} \{(R^i_1, R^i_2)\}$\;
%\end{algorithm}

\begin{algorithm}[t]
\caption{{\sc Partition-TwoTable}$(\I=\{R_1, R_2\})$}
\label{alg:partition-2table}

%$\ell \gets \lceil \log (\frac{n}{\lambda}+1) \rceil$\;
%$B^{i} \gets \emptyset$ for each $i \in [\ell]$\;
\lForEach{$i \in \N$}{$B^i \gets \emptyset$}
\ForEach{$b \in \dom(B)$}{
%\ForEach{$j \in \{1,2\}$}{
%    $\deg_j(B,b) = \degg_j(B,b) + \textsf{STGeom}_{\epsilon, \delta, 1}(x)$\;
%    }
   $\deg(B, b) = \max\{\degg_1(B,b), \degg_2(B,b)\} + \textsf{STGeom}_{\epsilon, \delta, 1}$\;
   
    %$i \gets \max\left\{0, \left\lceil \log \frac{1}{\lambda} \cdot \max\{\deg_1(B, b), \deg_2(B, b)\} \right\rceil\right\}$\;
    $i \gets \max\left\{1, \left\lceil \log \frac{1}{\lambda} \cdot \deg(B, b) \right\rceil\right\}$\;
    %\lIf{$B^i$ does not exist}{$B^{i} \gets \{b\}$}
    %\lElse{$B^{i} \gets B^{i} \cup \{b\}$}
    $B^{i} \gets B^{i} \cup \{b\}$\;
}
\ForEach{$i$ with $B^i \neq \emptyset$}{
    \lForEach{$j\in \{1,2\}$}{
    $R^{i}_j \gets \{R_j(t): t \in \D_j, \pi_B t \in B^{i}\}$}}
\Return $\bigcup_{i: B^i \neq \emptyset} \{(R^i_1, R^i_2)\}$\;
\end{algorithm}

\begin{figure}
    \centering
     \includegraphics[scale=0.7]{img/hard-two-table.pdf}
     \caption{An instance beyond the scope of Theorem~\ref{the:lb-two-table-2}. There are $\sqrt{n}$ join values in attribute $B$, where there is exactly one join value with degree $i$ in both $R_1, R_2$ for every $i\in[\sqrt{n}]$.}
    \label{fig:hard-two-table}
\end{figure}

\begin{lemma}
\label{lem:partition-2table-DP}
    Algorithm~\ref{alg:uniformization-framework} on two-table join is $(\epsilon, \delta)$-DP.
\end{lemma}

The key insight in Lemma~\ref{lem:partition-2table-DP} is that adding or removing one input tuple can increase or decrease the degree of one join value $b \in \dom(B)$ by at most one. Hence, Algorithm~\ref{alg:partition-2table} satisfies $(\epsilon,\delta)$-DP by the parallel composition rule~\cite{mcsherry2009privacy}. Moreover, since each input tuple participates in exactly one sub-instance, and Algorithm~\ref{alg:pmw} preserves $(\epsilon, \delta)$-DP for each sub-instance by Lemma~\ref{lem:two-table-DP}, Algorithm~\ref{alg:uniformization-framework} preserves $(2\epsilon, 2\delta)$-DP by the basic composition~\cite{dwork2006calibrating}.

\paragraph{Error Analysis.} We next analyze the error of Algorithm~\ref{alg:uniformization}. Given an instance $\I$, let $\pi = \{B^1_\pi,\cdots, B^{\ell}_\pi\}$ be the partition of $\dom(B)$ generated by Algorithm~\ref{alg:uniformization}. Correspondingly, $\pi$ derives a partition of input instance $\I = \{(R^i_1, R^i_2): i \in [\ell]\}$, where $(R^i_1, R^i_2)$ is the sub-instance in which tuples have their join values falling into $B^i_\pi$. Moreover, $\pi$ derives a partition of join result $J = \left\{J^1_\pi, J^2_\pi, \cdots, J^{\ell}_\pi\right\}$. Let $\F^i$ be the synthetic dataset generated for $(R^i_1, R^i_2)$ by {\sc JoinMultiTable}. From Theorem~\ref{the:up-2table}, with probability $1-1/\textsf{poly}(|\Q|)$, the error of answering linear queries defined over $\dom(A) \times \dom(B^i_\pi) \times \dom(C)$ that can be achieved with $\F^i$ is $\alpha_i = O\left(\sqrt{|J^{i}_\pi|} \cdot \sqrt{2^i \cdot \lambda} + 2^i \cdot \lambda\right)$. 
By a union bound, with probability $1- 1/\poly(|\Q|)$, the error can be achieved with $\bigcup_i \F^i$ is:
\begin{align*}
    \alpha \le \sum_{i\in [\ell]} \alpha_i \le \sum_{i\in [\ell]} \sqrt{|J^{i}_\pi|} \cdot \sqrt{2^i \cdot \lambda} + (\Delta + \lambda) \cdot \lambda
\end{align*}
where $\sum_{i\in [\ell]} 2^i =  \sum_{i\in [\lceil\log (\Delta+\lambda)\rceil]} 2^i=O\left(\Delta + \lambda\right)$. 

One may observe an overlap between the bucket ranges defined by $\pi$, but $\sum_{i} |J^i_\pi| = |J|$ always holds as $\pi$ induces a partition of $\dom(B)$ as well as $J$. In this way, Algorithm~\ref{alg:uniformization-framework} on two-table query is always better (at least not worse) than Algorithm~\ref{alg:two-table}, since $\sum_{i\in [\ell]} \sqrt{|J^{i}_\pi|} \cdot \sqrt{2^i} \le \sqrt{|J|} \cdot \sqrt{\Delta}$,
which is implied by the Cauchy-Schwarz inequality. Furthermore, we show in Appendix~\ref{appendix:uniformization} that for some input instances the gap between Theorem~\ref{the:up-2table-uniformize} and Theorem~\ref{the:up-2table} can be %logarithmically or even 
polynomially large, in terms of the data size.

Careful inspection reveals that although the partition generated by Algorithm~\ref{alg:partition-2table} is randomized due to the noise, it is not far away from the fixed partition based on true degrees.  As shown in Appendix~\ref{appendix:uniformization}, Algorithm~\ref{alg:partition-2table} always has its error bounded by what can be achieved through the {\em uniform partition} defined as below.

\begin{definition}[Uniform Partition]
    For $n>0, \epsilon >0, \delta >0$, and an input instance $\I = (R_1, R_2)$, the uniform partition of $\dom(B)$ on $\I$ is $\pi^* = \left\{B^1_{\pi^*},\cdots, B^{\lceil \log \frac{n}{\lambda} \rceil}_{\pi^*}\right\}$ such that for any $i \in [\lceil \log \frac{n}{\lambda} \rceil]$, $b \in B^i$ if
    %\begin{itemize}[leftmargin=*]
        %\item $b \in B^i$ if $\max\{\degg_1(B,b), \degg_2(B,b)\} \in (\max\{0,\lambda \cdot 2^{i-1}\}, \lambda \cdot 2^i]$.
    %\end{itemize}
    %$\displaystyle{\max\{\degg_1(B,b), \degg_2(B,b)\} \in (\max\{0,\lambda \cdot 2^{i-1}\}, \lambda \cdot 2^i]}$.
    $\displaystyle{\max\{\degg_1(B,b), \degg_2(B,b)\} \in (\gamma_{i-1}, \gamma_i]}$.
\end{definition}

\begin{theorem}
\label{the:up-2table-uniformize}
    For any two-table instance $\I$, a family of  linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that is $(\epsilon, \delta)$-DP, and with probability at least $1- 1/\textsf{poly}(|\Q|)$ produces $\F$ such that all queries in $\Q$ can be answered within error:%\pasin{Note that $J_i$ here is not the same as $J_i$ above in the analysis (which is defined based on noisy $R^i_1, R^i_2$).}
    %\[\alpha = O\left(\left(\sum_{i\in [\lceil \log \frac{n}{\lambda} \rceil]} \sqrt{\OUT^{i}_{\pi^*} \cdot 2^i \cdot \lambda} + \Delta \cdot \lambda + \lambda^2\right) \cdot \fup \right) \]
    \[\alpha = O\left(\left(\sum_{i\in [\lceil \log \frac{n}{\lambda} \rceil]} \sqrt{\OUT^{i}_{\pi^*} \cdot 2^i \cdot \lambda} + \lambda^2\right) \cdot \fup \right) \]
    where $\lambda = \frac{1}{\epsilon} \log \frac{1}{\delta}$, $\OUT^i_{\pi^*}$ is the number of join results whose join value falls into $B^i_{\pi^*}$ under the uniform partition $\pi^*$. %, and $\Delta = LS_\countsize(\I)$ is the local sensitivity of $\countsize(\cdot)$ on $\I$.
    %pasin: Note that I removed the Delta dependency because it was already dominated by the OUT^i part with largest i.
\end{theorem}

Let $\overrightarrow{\OUT}_{\pi^*} = (\OUT^i_{\pi^*})_{i \in [{\lceil \log \frac{n}{\lambda} \rceil}}$ be a characterization vector of join sizes under the uniform sensitivity partition $\pi^*$. A two-table database $\I=(R_1, R_2)$ {\em conforms} to $\overrightarrow{\OUT}_{\pi^*}$ if \[\sum_{(t_1, t_2) \in \D_1 \times \D_2: \pi_B t_1 = \pi_{B} t_2 \in B^i_{\pi^*}} R_1(t_1) \cdot R_2(t_2) \leq \OUT^i_{\pi^*}\]
holds for each $i \in [\lceil \log \frac{n}{\lambda} \rceil]$. Then, we introduce the following parameterized lower bound in terms of join size distribution, and show that Algorithm~\ref{alg:uniformization} is optimal on two-table query up to poly-logarithmic factors. The proof is given in Appendix~\ref{appendix:uniformization}.

\begin{theorem}
\label{the:lb-instance-optimality-2table}
    Given arbitrary parameters $\overrightarrow{\OUT}_{\pi^*}$ under the uniform partition $\pi^*$,
    for every sufficiently small $\eps, \alpha>0$, $n_D \ge (1/\alpha)^{\Omega(1)}$ and $n_Q \leq (1/\alpha)^{O(1)}$, there exists a family of queries $\Q$ of size $n_Q$ on domain $\D$ of size $n_D$ such that any $(\epsilon, o(1/n))$-differentially private algorithm that takes as input a two-table database of input size at most $n$ while conforming to $\overrightarrow{\OUT}_{\pi^*}$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ must satisfy  
    %\[\alpha \ge \tOmega\left(\sqrt{|\OUT|} \cdot \sqrt{\Delta} \cdot \flo\right).\]
    %Given arbitrary parameters $\overrightarrow{\OUT}$, let $\mathbb{I}(\overrightarrow{\OUT})$ be the set of two-table instances conforming to $\overrightarrow{\OUT}$. There exists a set of queries $\Q$ such that any $(\epsilon, \delta)$-differentially private algorithm that takes as input any instance from $\mathbb{I}(\overrightarrow{\OUT})$ and outputs an approximate answer to each query in $\Q$ within error $\alpha$, must require
    $\displaystyle{\alpha \ge \Omega\left(\max_{i\in [\lceil \log \frac{n}{\lambda} \rceil]} \sqrt{\OUT^i_{\pi^*}} \cdot \sqrt{2^i \cdot \lambda} \cdot \flo\right)}$.
\end{theorem}

%\paragraph{Discussion.} Comparing with Theorem~\ref{the:lb-two-table-2}, a more fine-grained parameterized notion of optimality has been achieved in Theorem~\ref{the:up-2table-uniformize}. A natural question is: Can we push this idea to the extreme, such that each parameterized class only contains a single instance, to obtain {\em instance-optimality}? As observed by \cite{asi2020instance}, this is not possible. We then leave the question of obtaining a neighborhood-optimal algorithm for releasing synthetic dataset as future work. 
\xiao{Pasin: do we need to say something about the hardness of neighborhood-optimality here?}
\pasin{Moved the discussion to the conclusion.}


\input{hierarchical}
%\input{three-table}

==> backup/backup.tex <==
%\begin{figure*}
%    \begin{minipage}{0.18\linewidth}
%        \includegraphics[scale=0.45]{img/attribute-tree.pdf}
%    \label{fig:hierarchical}
%    \end{minipage}
%    \begin{minipage}{0.78\linewidth}
%    \begin{align*}
 %       T_{345} =& \max_{(a,b)\in A\times B} |R_3 \Join R_4 \Join R_5 \ltimes (a,b)| \\
            =& \max_{(a,b) \in A\times B} |R_5 \ltimes (a)| \cdot |(R_3 \Join R_4) \ltimes (a,b)| \\
            \le& \max_{a \in A} |R_5 \ltimes (a)| \cdot \max_{(a,b) \in A\times B} |(R_3 \Join R_4) \ltimes (a,b)| \\
            \le& \max_{a \in A} |R_5 \ltimes (a)| \cdot \max_{(a,b) \in A\times B} |\pi_{ABG} (R_3 \Join R_4)| \cdot \max_{(a,b,g) \in A\times B\times G} |R_3 \ltimes (a,b,g)| 
            \cdot \max_{(a,b,g) \in A\times B\times G} |R_4 \ltimes (a,b,g)| \\
            \le & \max_{a \in A} \degg_{5}(A,a) \cdot \max_{(a,b) \in A\times B} \degg_{34}(AB, ab) \cdot \max_{(a,b,g) \in A\times B\times G} \degg_3(ABG,abg) \cdot \max_{(a,b,g) \in A\times B\times G}\degg_4(ABG,abg) 
    \end{align*}
    \end{minipage}
     \caption{Left upper is the attribute tree for hierarchical join: $R_1(A,B,D) \Join R_2(A,B,F) \Join R_3(A,B,G,K) \Join R_4(A,B,G,L) \Join R_5(A,C)$. Left lower is an example of $H_E$ for $E = \{3,4,5\}$, with boundary attributes $\partial E = \{A,B\}$. After removing $\partial E$, $E$ is decomposed into $\{\{3,4\}, 5\}$. The right is an upper bound derived for $T_E$.}
    \label{fig:hierarchical}
\end{figure*}
\paragraph{Abstract problem on Bipartite Graph} Suppose we are given a bipartite graph $G= (B, C, R)$, where $B$, $C$ are the two vertex sets and $R$ is the set of edges between $B$ and $C$.  There are $n$ edges in total, i.e., $|R| = n$. A $k$-partition of $G$ is defined as: 
\[\{(B_i, C_i, R^i): i \in [k], R^i \subseteq R\}\]
such that 
\begin{itemize}[leftmargin=*]
    \item For any $i \in [k]$, $R^i$ has vertex support as $B_i \subseteq B, C_i \subseteq C$.
    \item $R^i \cap R^j = \emptyset$, for any pair $(i,j) \in [k] \times [k]$ and $i \neq j$.
    \item For any $i \in [k]$, there exists two integers $\ell_1, \ell_2$ such that  for any $b \in B_i$, 
    \[\sum_{t: \pi_B t = b} R^i(t) \in [2^{\ell_1-1}, 2^{\ell_1}]\] 
    and for any $c \in C_i$, 
    \[\sum_{t: \pi_C t = c} R^i(t) \in [2^{\ell_2-1}, 2^{\ell_2}]\] 
    i.e., the degree of vertices in $B_i$ (with respect to $C_i$) are approximately the same (within a constant factor) in $R^i$.
\end{itemize}
The size of such a partition is defined as the maximum number of $R^i$'s each vertex $b \in B$ or $c \in C$ participates in. The question is: Does there always exist a $O(\log^c n)$-sized partition for arbitrary bipartite graph?


We note that a $n$-sized partition is always trivial by putting every single edge into a single $R^i$, but this will not suffice for our algorithm. For a $k$-sized partition, each tuple in $R_1$ or $R_3$ will participate in $k$ sub-instances. If incorporating such a partition into Algorithm~\ref{alg:uniformization-framework}, the privacy budget will blow up by a factor of $k$. If targeting $(\epsilon, \delta)$-DP algorithm, a factor of $\sqrt{k}$ will blow up in the error complexity, which would be too costly.  which will be too costly. 


Consider the hard instance as depicted in Figure~\ref{fig:line-3}. Theorem~\ref{the:}

%The residual sensitivity becomes
%\begin{align*}
%    RS_\countsize(\I^\sigma) &= \max_{k\ge0} e^{-\beta k} \cdot \hat{LS}^{(k)}(\I^{\sigma}) \\
%    &= \max_{k\ge0} e^{-\beta k} \cdot \max\{LS_\countsize(\I^{(\sigma)}), k^2\} \\
%    &\le \max\{LS_\countsize(\I^{\sigma}), \frac{4}{e^2\cdot \beta^2}\}
%\end{align*}


%\begin{lemma}
%    This algorithm preserves $(\epsilon \cdot \log n, \delta \cdot \log n)$-DP.
%\end{lemma}
%
%\begin{proof}
%    Consider two neighboring instances $\I, \I'$. Let $\F, \F'$ be the resulted synthetic datasets generated for $\I,\I'$. It can be easily show that the partition of sub-instances satisfies $(\epsilon, \delta)$-DP. 
%    It can be easily argued that each tuple in $R_1$ or $R_3$ participated in $O(\log n)$ sub-instances. Implied by the group-DP, $\F \sim_{(\epsilon \cdot \log n, \delta \cdot \log n)} \F'$. 
%\end{proof}
%
%$\paragraph{Error analysis.} For each sub-instance $I^\sigma$, the $\ell_\infty$-error can be achieved is 
%\begin{align*}
%    \alpha^\sigma = \sqrt{|J^\sigma|} \cdot \sqrt{SS_\countsize(\I^\sigma)} + SS_\countsize(\I^\sigma)
%\end{align*}
%For any query $q = (q_1, q_2, q_3)$, we have
%\begin{align*}
%    q(R_1, R_2, R_3) - q(\F) & = \sum_{\sigma}  q(R^{\sigma(1)}_1, R_2, R_3) - q(\F^\sigma) \\
%    &\le \sum_{\sigma} \sqrt{|J^\sigma|} \cdot \sqrt{SS_\countsize(\I^\sigma)} + SS_\countsize(\I^\sigma)
%    & 
%  \end{align*}
%
%
%\begin{algorithm}[h]
%\caption{{\sc UniformizeThreeTable}$(R_1, R_2, R_3)$}
%\label{alg:three-table}
%
%$\Delta_1 \gets \max_{b \in \dom(B)} \degg_1(b)$, $\Delta_3 \gets \max_{c \in \dom(C)} \degg_3(c)$\; 
%$\widetilde{\Delta}_1 \gets \Delta_1 + G_{\epsilon, \delta, 1}(x)$, %$\widetilde{\Delta}_3 \gets \Delta_3 + G_{\epsilon, \delta, 1}(x)$\;
%$\ell_1 \gets \lceil \log_2 \widetilde{\Delta}_1 \rceil$, $\ell_3 \gets \lceil \log_2 \widetilde{\Delta}_3 \rceil$\;
%$B^{(i)} \gets \emptyset$ for each $i \in [\ell_1]$, $C^{(j)} \gets \emptyset$ for each $j \in [\ell_3]$\;
%\ForEach{$b \in B$}{
%    $\deg_1(b) = \sum_{t \in \D_1: \pi_B t = b} R_1(t) + G_{\epsilon, \delta, 1}(x)$\;
%    $i \gets \left\lceil \log \deg_1(b) \right\rceil$\;
%    $B^{(i)} \gets B^{(i)} \cup \{b\}$\;
%}
%\ForEach{$c \in C$}{
%    $\deg_3(c) = \sum_{t \in \D_3: \pi_C t = c} R_3(t) + G_{\epsilon, \delta, 1}(x)$\;
%    $j \gets \left\lceil \log \deg_3(c)\right\rceil$\;
%    $C^{(j)} \gets C^{(j)} \cup \{c\}$\;
%}
%\ForEach{$(i,j) \in [\ell_1] \times [\ell_2]$}{
%    $R^{(i)}_1 \gets \left\{R_1(t): t \in \D_1, \pi_{B} t \in B^{(i)}\right\}$\;
%    $R^{(ij)}_2 \gets \left\{R_2(t): t \in \D_2, \pi_{B} t \in B^{(i)}, \pi_{C} t \in C^{(j)}\right\}$\;
%    $R^{(i)}_3 \gets \left\{R_3(t): t \in \D_3, \pi_{C} t \in C^{(j)} \right\}$\;
%    $\F^{(ij)}\gets$ {\sc ThreeTable}$\left(R^{(i)}_1, R^{(ij)}_2, R^{(j)}_3\right)$\;
%}
%\Return $\bigcup_{(i,j) \in [\ell_1] \times [\ell_3]} \F^{(ij)}$\;
%\end{algorithm}
\section{Comparison between different notions of Sensitivity on $\countsize(\cdot)$}


 \medskip
 In the remaining of this paper, if not specified, ``smooth sensitivity'' as short for ``smooth upper bound on local sensitivity'', refers to ``residual sensitivity''.


\iffalse
\begin{proof}[\new{Proof of Lemma~\ref{lem:reduction}}]
We show a reduction from single-table release problem to two-table release problem. Suppose, we are given an arbitrary table $R$ of $n$ records over domain $\mathbb{D}_1$. and be a family of linear queries $\Q = \{q: \mathbb{D}_1 \to [-1,+1]\}$.

We add a common join key to every record in $R$, and construct another table $S$ of $n$ records over $\mathbb{D}_2$ sharing the same join key. Let $q_2: \mathbb{D}_2 \to \{+1\}$ be a query over $S$. Let $\Q_2 = \Q_1 \times \{q_2\}$ be the family of linear queries, where
\begin{align*}
    q(R,S) &= \sum_{(x, y) \in \mathbb{D}_1 \times \mathbb{D}_2} q_1(x) \cdot q_2(y) \cdot R(x) \cdot S(y) \\
           &= \left(\sum_{x \in \mathbb{D}_1} q_1(x) \cdot R(x) \right) \cdot \left(\sum_{y \in \mathbb{D}_2} q_2(y)\cdot  S(y) \right) = q(R) \cdot n
\end{align*}
for $q = (q_1, q_2) \in \Q_1 \times \{q_2\}$. Suppose, we are able to generate a function $Z: \D_1 \times \D_2 \to \mathbb{R}$ for $R, S$ such that the $\ell_\infty$ error is $O(n^{3/2})$, i.e., for any query $q = (q_1, q_2)$,
\begin{align*}
    q(R,S) - q''(\F) =& \ q(R) \cdot n  - \sum_{x\in \D_1} q_1(x) \cdot \sum_{y \in \D_2} \F(x,y) \le n^{3/2}.
\end{align*}
From $\F$, we construct a synthetic dataset for $R$ as follows. Let $\eta = \frac{1}{n} \cdot \sum_{(x,y) \in \D_1 \times \D_2} \F(x,y)$ be the scaling factor. For each $x \in \D_1$, we define $g(x) = \frac{1}{\eta} \cdot \sum_{y \in \D_2} \F(x,y)$. It can be easily checked that 
\[\sum_{x \in \D_1} g(x) = \sum_{x \in \D_1}  \frac{1}{\eta} \cdot \sum_{y \in \D_2} \F(x,y) = \frac{1}{\eta} \cdot \sum_{x \in \D_1}  \sum_{y \in \D_2} \F(x,y) = n.\]
So function $g$ is a valid synthetic dataset for $R$. Moreover, the join size is as large as $n^2$ in this construction. Plugging to Lemma~\ref{lem:max}, we have
\[n^2 - \alpha \le \sum_{(x,y) \in \D_1 \times \D_2} \F(x,y) \le n^2+\alpha,\]
therefore $n - \frac{\alpha}{n} \le \eta \le n+\frac{\alpha}{n}$. 

We next bound the error of answering queries from $\Q_1$ using function $g$. Consider an arbitrary query $q_1 \in \Q_1$. We distinguish the error based on two cases:
\begin{enumerate}
    \item $\eta \ge n$: 
    \begin{align*}
        q(R) - q(\widetilde{R})
        &= \frac{1}{n} \cdot q(R,S) - \frac{1}{\eta} \cdot q''(\F)  \\
        &= \frac{1}{n} \cdot \left(q(R,S) - q''(\F)\right) + \left(\frac{1}{n} - \frac{1}{\eta}\right) \cdot q''(\F) \\
        &\le \frac{\alpha}{n} + \left(\frac{1}{n} - \frac{1}{\eta}\right) \cdot \sum_{(x,y) \in \D_1 \times \D_2} \F(x,y) \\
        &= \frac{\alpha}{n} + \eta - n \le \frac{2\alpha}{n}.
    \end{align*} 
    \item $\eta < n$:
    \begin{align*}
        q(R) - q(\widetilde{R})
        &= \frac{1}{n} \cdot q(R,S) - \frac{1}{\eta} \cdot q''(\F)  \\
        &= \frac{1}{n} \cdot \left(q(R,S) - q''(\F)\right) - \left(\frac{1}{\eta} - \frac{1}{n}\right) \cdot q''(\F) \\
        &\le \frac{\alpha}{n} + \left(\frac{1}{\eta} - \frac{1}{n}\right) \cdot \sum_{(x,y) \in \D_1 \times \D_2} \F(x,y) \\
        &= \frac{\alpha}{n} + n - \eta\le \frac{2\alpha}{n}.
    \end{align*} 
\end{enumerate}
The error for $q(\widetilde{R}) - q(R)$ can be bounded in a similar way.
\end{proof}
\fi

$LS_\countsize(\I) $, in term Define $\Delta$ as the sensitivity of counting join size query (i.e., the maximum sum (of frequency) of tuples in $R_2$ that one tuple in $\D_1$ can be joined with, or the maximum sum (of frequency) of tuples in $R_1$ that one tuple in $\D_2$ can be joined with).  Define $\Delta_1$ as the maximum sum (of frequency) of tuples in $R_1$ that one tuple in $\D_2$ can be joined with. Define $\Delta_2$ as the maximum sum (of frequency) of tuples in $R_2$ that one tuple in $\D_1$ can be joined with. So $\Delta = \max(\Delta_1, \Delta_2)$.


%\begin{enumerate}[leftmargin=*]
%    \item Construct a function $J: \D_1 \times \D_2 \to \mathbb{N}$ over $R_1$ and $R_2$: 
%    \[J = R_1(x) \cdot R_2(y) \cdot \rho(x,y)\]
%    \item We draw a random noise from $G_{\epsilon, \delta, 1}(x)$ and add it to $\Delta$. Let the noisy version of sensitivity as $\widetilde{\Delta}$. Then, we draw a random noise from $G_{\epsilon, \delta, 2\widetilde{\Delta}}(x)$, and choose so many records randomly drawn from $\mathbb{D}_1 \times \mathbb{D}_2$, denoted as $\widetilde{J}$. 
%    \item We combine $J$ and $\widetilde{J}$ as $\widehat{J} = J + \widetilde{J}$, and invoke the single-table algorithm for releasing a synthetic dataset for $\widehat{J}$ as $\F$.  
%\end{enumerate}


%\begin{algorithm}
%%\caption{{\sc TwoTableAnotherVersion}$(R_1, R_2)$}
%\label{alg:two-table-version}
%
%$J(x,y) = R_1(x) \cdot R_2(y) \cdot \rho(x,y)$\;
%$\Delta \gets $ local sensitivity of $|R_1 \Join R_2|$\;
%$\widetilde{\Delta} \gets \Delta + G_{\epsilon, \delta, 1}(x)$\;
%\xiao{$\widehat{n} \gets |J| + G_{\epsilon, \delta, 2\widetilde{\Delta}}(x)$}\;
%$\F_0 \gets \widehat{n}$ times uniform distribution over $\D$: $\F_0(x) = \frac{\widehat{n}}{|\D|}$\;
%\ForEach{$i = 1, 2, \cdots, T$}{
%    Sample a query $q_i \in \Q$ using the EM parameterized with \xiao{$\epsilon/(2T\lambda)$} and score function $s_i(\xiao{J},q) = |q(\F_{i-1}) - q(\xiao{J})|$\;
%    $m_i \gets q_i(\xiao{J}) + \xiao{\textsf{Lap}(2T\lambda/\epsilon)}$\;
%    Update for each $x \in \D$: $\F_i(x) \propto \F_{i-1}(x) \times \exp\left(q_i(x) \cdot \left(m_i - q_i(\F_{i-1})\right) \cdot \frac{1}{2\widehat{n}}\right)$\;
%}
%\Return $\textsf{Avg} \left(\sum_{i=1}^T \F_i\right)$\;
%\end{algorithm}




\xiao{$\F$ doesn't satisfy DP!!! The initial state for two neighboring databases $(R'_1, R'_2)$ and $(R'_1, R'
    _2)$ can reveal the information of input database.}
    


\iffalse
\begin{proof}[\new{Proof of Lemma~\ref{lem:reduction}}]
We show a reduction from single-table release problem to two-table release problem. Suppose, we are given an arbitrary table $R$ of $n$ records over domain $\mathbb{D}_1$, and a family of linear queries $\Q = \{q: \mathbb{D}_1 \to [-1,+1]\}$.

We add a join attribute $B$ to $\D_1$, such that all records in $\D_1$ have the same join value $b$. 
We construct another table $S$ of $n$ records over $\mathbb{D}_2$, such that $\frac{|J|}{n}$ records in $S$ share the same join value $b$, and the remaining $n - \frac{|J|}{n}$ records in $S$ display different join values. Let $q_2: \mathbb{D}_2 \to \{+1\}$ be a query over $S$. Let $\Q_2 = \Q_1 \times \{q_2\}$ be the family of linear queries. For every $q = (q_1, q_2) \in \Q_1 \times \{q_2\}$, we have
\begin{align*}
    q(R,S) & = \sum_{(x,y) \in \D_1 \times \D_2} q_1(x) \cdot R(x) \cdot q_2(y) \cdot S(y) \cdot \rho(x,y) \\
    &= \left(\sum_{x \in \D_1} q_1(x) \cdot R(x) \right) \cdot \left(\sum_{y \in \D_2: \pi_B y = b} S(y) \cdot q_2(y) \right) \\
    &= q(R) \cdot \frac{|J|}{n}
\end{align*}
From $\F$, we construct a synthetic dataset for $R$ as follows. Let $\eta = \frac{1}{n} \cdot \sum_{(x,y) \in \D_1 \times \D_2} \F(x,y)$ be the scaling factor. For each $x \in \D_1$, we define $g(x) = \frac{1}{\eta} \cdot \sum_{y \in \D_2} \F(x,y)$. It can be easily checked that $\sum_{x \in \D_1} g(x) =n$, thus function $g$ is a valid synthetic dataset for $R$. 


We next bound the error of answering queries from $\Q_1$ using function $g$. We first mention the fact that \[\frac{|J|}{n} - \frac{\alpha}{n} \le \eta \le \frac {|J|}{n}+\frac{\alpha}{n},\] implied by Lemma~\ref{lem:max}.
Consider an arbitrary query $q_1 \in \Q_1$. We distinguish the error basde on two cases: 
\begin{enumerate}
    \item $\frac{|J|}{n}<\eta< \frac{|J|}{n} + \frac{\alpha}{n}$: 
    \begin{align*}
        q(R) - q(\widetilde{R}) &= q(R) - \sum_{x \in \D_1} q_1(x) \cdot g(x) \\
        &= \frac{1}{\Delta} \cdot q(R,S) - \frac{1}{\eta} \cdot q''(\F) \\
        &= \frac{1}{\Delta} \cdot \left( q(R,S) - q''(\F) \right) + \left(\frac{1}{\Delta} - \frac{1}{\eta}\right) \cdot q''(\F)\\
        &\le \frac{1}{\Delta} \cdot \alpha + \left(\frac{1}{\Delta} - \frac{1}{\eta}\right) \cdot \sum_{x \in \D_1} \sum_{y \in \D_2} \F(x,y)\\
        &=  \frac{1}{\Delta} \cdot \alpha + \frac{n^2 \cdot \eta}{|J|} - n  \le \frac{2n}{|J|} \cdot \alpha
    \end{align*}
    \item $\frac{|J|}{n} - \frac{\alpha}{n} <\eta \le \frac{|J|}{n} $: 
    \begin{align*}
        q(R) - q(\widetilde{R}) &= q(R) - \sum_{x \in \D_1} q_1(x) \cdot g(x) \\
        &= \frac{1}{\Delta} \cdot q(R,S) - \frac{1}{\eta} \cdot q''(\F) \\
        &= \frac{1}{\Delta} \cdot \left( q(R,S) - q''(\F) \right) + \left(\frac{1}{\Delta} - \frac{1}{\eta}\right) \cdot q''(\F)\\
        &\le \frac{1}{\Delta} \cdot \alpha + \left(\frac{1}{\eta}-\frac{1}{\Delta} \right) \cdot \sum_{x \in \D_1} \sum_{y \in \D_2} \F(x,y)\\
        &=  \frac{1}{\Delta} \cdot \alpha + n- \frac{n^2 \cdot \eta}{|J|}  \le \frac{2n}{|J|} \cdot \alpha
    \end{align*}
\end{enumerate}
The error for $q(\widetilde{R}) - q(R)$ can be bounded in a similar way.
\end{proof}
\fi


%\paragraph{Problem Definition.} Given two input tables $R_1: \mathbb{D}_1 \to \mathbb{N}$ and $R_2: \mathbb{D}_2 \to \mathbb{N}$, each of $n$ records, two families of linear queries $\Q_1, \Q_2$ over $\mathbb{D}_1, \mathbb{D}_2$ separately, a join function $\rho: \mathbb{D}_1 \times \mathbb{D}_2 \to \{0,1\}$ and a family of linear queries $\Q = \Q_1 \times \Q_2$, the question is how to generate a function $\F: \mathbb{D}_1 \times \mathbb{D}_2 \to \mathbb{N}$ such that all queries in $\Q$ can be answered over $\F$ accurately, i.e.,
%\[\min \max_{q \in \Q} |q(R_1, R_2) - q(\F)|\]
%where
%\begin{align*}
%    q(R_1, R_2) &= \sum_{(x,y) \in \D_1 \times \D_2} q_1(x) \cdot R_1(x) \cdot q_2(y) \cdot R_2(y) \cdot \rho(x,y) \\
%    q(\F) &= \sum_{(x,y) \in \D_1 \times \D_2} q_1(x) \cdot q_2(y) \cdot \F(x, y)
%\end{align*}
%while providing $(\epsilon, \delta)$-differential privacy?




\newpage
\paragraph{Release the synthetic data for $R_1, R_2$ using the information from the other table. } 

\begin{algorithm}
\caption{{\sc TwoTableRelease-S}} 

$\D'_2 \gets \{x \in \D_2: |\sigma_{B = \pi_B x} R_1| \ge \tau\}$\;
Let $\widetilde{S}_0$ denote $n \times$ the uniform distribution over $\D_2$\;
\ForEach{$j \in \{1,2,\cdots, T\}$}{
    Sample a query $q_j \in \Q$ using the EM with epsilon value $\epsilon/(2T \cdot \Delta)$ and score function $|q(R, \widetilde{S}_j) - q(R,S)|$ for $q$\;
    $z_j = q_j(R,\widetilde{S}_i)  - q_j(R,S) + \textrm{Lap}(2T \cdot \Delta /\epsilon)$\;
    \lIf{$|z_j| \le 2\alpha$}{
        return $\widetilde{S}_j$
    }
    $\widetilde{S}_{j+1}(y) \gets \widetilde{S}_j(y) \cdot \left(1 -\textrm{sign}(z_j) \cdot \sqrt{\frac{\ln |\D|}{T}} \cdot q_j(y)\right)$\;
}
\Return $\widetilde{S}_{T+1}$\;
\end{algorithm}


\begin{algorithm}
\caption{{\sc TwoTableRelease-R}} 

 
Let $\widetilde{R}_0$ denote $n \times$ the uniform distribution over $\D_1$\;
%$\J = \sum_{(x,y) \in \D_1 \times \D_2: \rho(x,y)=1} R(x)S(y)$\;
\ForEach{$j \in \{1,2,\cdots, T\}$}{
    Sample a query $q_j \in \Q$ using the EM with epsilon value $\epsilon/(2T \cdot \Delta)$ and score function $|q(\widetilde{R}_{j}, S) - q(R,S)|$\;
    $z_j = q_j(\widetilde{R}_j, S)  - q_j(R,S) + \textrm{Lap}(2T \cdot \Delta /\epsilon)$\;
     \lIf{$|z_j| \le 2\alpha$}{
        return $\widetilde{R}_j$
    }
    $\widetilde{R}_{j+1}(x) \gets \widetilde{R}_j(x) \cdot \left(1 -\textrm{sign}(z_j) \cdot \sqrt{\frac{\ln |\D|}{T}} \cdot q_j(x)\right)$\;
}
\Return $\widetilde{R}_{T+1}$\;
\end{algorithm}

We first mention the following fact as a generalization of the single-table case:
\begin{align*}
    & \max_{q \in \Q} \max\left\{|q(R, \widetilde{S}) - q(R,S)|, |q(\widetilde{R},S) -q(R,S)| \right\}  \\
    =& O\left(\sqrt{n} \cdot \sqrt{\Delta} \cdot (\frac{\log |\Q| \cdot \log^{1/2} |\D| \cdot \log \frac{1}{\delta}}{\epsilon})^{1/2}\right)
\end{align*}
Then, our target is to use $(\widetilde{R}, \widetilde{S})$ as a synthetic data for $(R,S)$. For an arbitrary query $q = (q_1, q_2) \in \Q$, the error can be achieved is 
\begin{align*}
    |q(R,S) - q(\widetilde{R}, \widetilde{S})| \le |q(R,S) - q(R, \widetilde{S}) + q(R,\widetilde{S}) - q(\widetilde{R},S) + q(\widetilde{R},S) - q(\widetilde{R}, \widetilde{S})|    
\end{align*}
    


\section{Appendix}

\xiao{Adapted from the single-table paper.}

\begin{proof}[Proof of Lemma~\ref{lem:error}]
The probability that the exponential mechanism with parameter $\frac{\epsilon}{2T \cdot \Delta_2}$ selects a query with quality score at least $r$ less than the optimal is bounded by 
\[\Pr[|q_i(\widetilde{R}_{i-1}) - q_i(\B)| < \ME_i- r] \le |\Q| \times \exp\left(-\frac{\epsilon r}{4T \cdot \Delta_2}\right).\]
If we take $r = (2c + 2) \times 2T \log |\Q| \times \Delta_2/\epsilon$ the probability is at
most $1/|\Q|^{c}$ for each iteration. By the definition of the Laplace distribution,
\[\Pr[|\textrm{Laplace}(\Delta_1 \cdot 2T/\epsilon)| > r] \le \exp\left(-\frac{\epsilon r}{2T \cdot \Delta_1}\right).\]
Taking $r = c \cdot 2T \log |\Q| \cdot \Delta_1/\epsilon$ bounds the probability by at
most $1/|\Q|^{c}$ for each iteration. Taking a union bound over the $2T$ events, we arrive at a
failure probability of at most $2T /|\Q|^{c}$.
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:psi}]
We note that $\widetilde{R}_0(x) = \frac{n}{|D|}$. Then
\begin{align*}
    \Psi_0 =& \sum_{x\in D} \frac{\B(x)}{n} \log \frac{\B(x)}{n} + \sum_{x \in D} \frac{B(x)}{n} \log |D|
    \le  \log |D|
    \end{align*}
    since and $\sum_{x \in D} \frac{\B(x)}{n} = 1$ and $0 \le \frac{\B(x)}{n} \le 1$.
    
We only consider $D' \subseteq D$ such that $\B(x) > 0$ for any $x \in D'$. Since $\ln x \leq x-1$ for all $x > 0$, with equality if and only if $x=1$, we have:
\begin{align*}
    - \frac{1}{n} \cdot \sum_{x \in D'} \B(x) \log \frac{\widetilde{R}_i(x)}{\B(x)} \ge & - \frac{1}{n} \cdot \sum_{x \in D'} \B(x) \left(\frac{\widetilde{R}_i(x)}{\B(x)} -1 \right) \\
    \ge & -\frac{1}{n} \cdot \sum_{x \in D'} \widetilde{R}_i(x) + \frac{1}{n} \cdot \sum_{x \in D'} \B(x) \\
    \ge & - \frac{1}{n} \cdot \sum_{x \in D'} \widetilde{R}_i(x) +1 \ge 0
\end{align*}
\end{proof}

\begin{algorithm}
\label{alg:together}
\caption{{\sc TwoTableRelease}} 

Let $\widetilde{R}_0$ denote $n \times$ the uniform distribution over $\D_1$\;
%$\J = \sum_{(x,y) \in \D_1 \times \D_2: \rho(x,y)=1} \B(x)S(y)$\;
\ForEach{$i \in \{1,2,\cdots, T\}$}{
    Sample a query $q_i \in \Q_1$ using the EM parameterized with epsilon value $\epsilon/(2T \cdot \Delta)$ and the score function 
    \[s_i(\B,S, q) = |q(\widetilde{R}_{i-1}, S) - q(\B,S)|\]
    \\
    $m_i \gets q_i(\B,S) + \textrm{Lap}(2T \cdot \Delta /\epsilon)$\;
    $\eta_i \gets \frac{m_i - q_i(\widetilde{R}_{i-1}, S)}{2n}$\; 
    \ForEach{$x \in \D_1$}{
        $\widetilde{R}_i(x) = \frac{1}{\beta_i} \cdot  \widetilde{R}_{i-1}(x)  \cdot \left( \sum_{y \in \D_2} S(y) \cdot \rho(x,y)\right) \cdot \exp\left(q_{i}(x) \cdot \eta_i \right)$\;
    }
}
\Return $\textrm{avg}_i \widetilde{R}_i$\;
\end{algorithm}

\begin{algorithm}
\label{alg:together}
\caption{{\sc TwoTableRelease}} 

Let $\widetilde{S}_0$ denote $n \times$ the uniform distribution over $\D_2$\;
%$\J = \sum_{(x,y) \in \D_1 \times \D_2: \rho(x,y)=1} \B(x)S(y)$\;
\ForEach{$i \in \{1,2,\cdots, T\}$}{
    Sample a query $q_i \in \Q_2$ using the EM parameterized with epsilon value $\epsilon/(2T \cdot \Delta)$ and the score function 
    \[s_i(\B,S, q) = |q(\B, \widetilde{S}_{i-1}) - q(\B,S)|\]
    \\
    $m_i \gets q_i(\B,S) + \textrm{Lap}(2T \cdot \Delta /\epsilon)$\;
    $\eta_i \gets \frac{m_i - q_i(\B, \widetilde{S}_{i-1})}{2n}$\; 
    \ForEach{$y \in \D_2$}{
        $\widetilde{S}_i(y) = \frac{1}{\beta_i} \cdot  \widetilde{S}_{i-1}(y)  \cdot \left( \sum_{x \in \D_1} \B(x) \cdot \rho(x,y)\right) \cdot \exp\left(q_{i}(y) \cdot \eta_i \right)$;
    }
}
\Return $\textrm{avg}_i \widetilde{S}_i$\;
\end{algorithm}



\subsection{Naive Solution 2}

\paragraph{Algorithm.} Alternatively, we release a synthetic dataset for $R_1, R_2$ separately, denoted as $\widetilde{R}_1, \widetilde{R}_2$. Then, the final function $\F$ is:
\[\F(x,y) = \widetilde{R_1}(x) \cdot \widetilde{R_2}(y) \cdot \rho(x,y)\]
\paragraph{Error Analysis.}  Implied by the single table result, we know
\begin{align*}
    \max_{q_1 \in \Q_1} |q_1(R_1) - q_1(\widetilde{R}_1)| =& O\left(n^{1/2} \cdot f(\mathbb{D}_1, \Q_1, \epsilon, \delta)\right) \\
    \max_{q_2 \in \Q_2} |q_2(R_2) - q_2(\widetilde{R}_2)| =& O\left(n^{1/2} \cdot f(\mathbb{D}_2, \Q_2, \epsilon, \delta)\right)
\end{align*}
Here, we consider the simple natural join for $\rho$, where every data item in $\D_1$ or $\D_2$ has a key, and $\rho(x,y)=1$ if and only if $x,y$ share the same key \badih{How is this different from the more general setting considered above?}. Moreover, we denote the set of data items in $\D_1$ (with respect to $\D_2$) with key $k$ as $\D^{(k)}_1$ (with respect to $\D^{(k)}_2$). In this way, we can rewrite $q(R_1, R_2)$ and $q(\F)$ as follows:
\begin{align*}
    q(R_1, R_2) =& \sum_{k \in \K} \left(\sum_{x \in \D^{(k)}_1} q_1(x) \cdot R_1(x)  \right) \left(\sum_{y \in \D^{(k)}_2}  q_2(y) \cdot R_2(y) \right) \Rightarrow \sum_k \alpha_k \beta_k \\
    q(\F) =& \sum_{k \in \K} \left(\sum_{x \in \D^{(k)}_1} q_1(x) \cdot \widetilde{R}_1(x)  \right) \left(\sum_{y \in \D^{(k)}_2}  q_2(y) \cdot \widetilde{R}_2(y) \right) \Rightarrow \sum_k \widetilde{\alpha}_k \widetilde{\beta}_k 
\end{align*}
We distinguish keys into two categories: 
\begin{align*}
    \K_1 =& \ \left\{k: \sum_{x \in \D^{(k)}_1} R_1(x) = 0 \right\}\\
    \K_2 =& \ \left\{k: \sum_{y \in \D^{(k)}_2} R_2(y) = 0\right\}\\
    \K_3 =& \ \K - \K_1 \cup \K_2
\end{align*}
Observe that $\alpha_k = 0$ for every $k \in \K_1$, and $\beta_k = 0$ for every $k \in \K_2$.
Given the facts that 
\begin{align*}
    q_1(R_1) - q_1(\widetilde{R_1}) = \sum_{k} (\alpha_k -\widetilde{\alpha}_k) \le  \sqrt{n} \cdot f(\mathbb{D}_1, \Q_1, \epsilon, \delta)\\
    q_2(R_2) - q_2(\widetilde{R_2}) = \sum_{k} (\beta_k - \widetilde{\beta}_k) \le \sqrt{n} \cdot f(\mathbb{D}_2, \Q_2, \epsilon, \delta)
\end{align*}\badih{Are we here going from max error bound to sum error bound?} we have
\begin{align*}
     & q(\F) -  q(R_1, R_2) \\
     = & \sum_{k \in \K} \left(\widetilde{\alpha}_k \widetilde{\beta}_k - \alpha_k \beta_k \right) \\
     = & \sum_{k \in \K_1 \cup \K_2} \widetilde{\alpha}_k \widetilde{\beta}_k  +  \sum_{k \in \K_3} \left( (\widetilde{\alpha}_k - \alpha_k) \beta_k + (\widetilde{\beta}_k - \beta_k) \alpha_k + (\widetilde{\alpha}_k - \alpha_k)(\widetilde{\beta}_k - \beta_k) \right)   \\
     \le & \sum_{k \in \K_1 - \K_2} (\widetilde{\alpha}_k - \alpha_k) \widetilde{\beta}_k +
     \sum_{k \in \K_2 - \K_1} \widetilde{\alpha}_k (\widetilde{\beta}_k - \beta_k)  \\
     +&  \Delta_2 \cdot \sum_{k \in \K_3} (\widetilde{\alpha}_k - \alpha_k) + \Delta_1 \cdot  \sum_{k \in \K_3}(\widetilde{\beta}_k - \beta_k) \\
     +&  \sum_{k \in \K_3 \cup (\K_1 \cap \K_2)} (\widetilde{\alpha}_k - \alpha_k)\cdot \sum_{k \in \K_3 \cup (\K_1 \cap \K_2)} (\widetilde{\beta}_k -\beta_k) \\
     \le & \new{\sum_{k \in \K_1 - \K_2} (\widetilde{\alpha}_k - \alpha_k)\beta_k  +
     \sum_{k \in \K_2 - \K_1} \alpha_k  (\widetilde{\beta}_k - \beta_k)}  \\
     +&  \Delta_2 \cdot \sum_{k \in \K_3} (\widetilde{\alpha}_k - \alpha_k) + \Delta_1 \cdot  \sum_{k \in \K_3}(\widetilde{\beta}_k - \beta_k) \\
     +&  \sum_{k \in \K_3 \cup (\K_1 \cap \K_2)} (\widetilde{\alpha}_k - \alpha_k)\cdot \sum_{k \in \K_3 \cup (\K_1 \cap \K_2)} (\widetilde{\beta}_k -\beta_k) \\
     \le & \new{\sqrt{n} \cdot \Delta_2  \cdot f(\mathbb{D}_1, \Q_1, \epsilon, \delta) +  \sqrt{n} \cdot \Delta_1  \cdot f(\mathbb{D}_2, \Q_2, \epsilon, \delta)}  \\
     & \new{+ n \cdot f(\mathbb{D}_1, \Q_1, \epsilon, \delta) \cdot f(\mathbb{D}_2, \Q_2, \epsilon, \delta)}
\end{align*}
where the second last inequality is implied by the facts that $\alpha_k \le \Delta_1$ and $\beta_k \le \Delta_2$ for $k \in \K_3$. By taking $\Delta_1 = \Delta_2 = O(n)$, we can get the worst-case error as 
$O\left(n^{\frac{3}{2}} \cdot f(\mathbb{D}, \Q, \epsilon, \delta) \right)$.

\newcommand{\RNum}[1]{\Fextrm{(\uppercase\expandafter{\romannumeral #1\relax})}}
\subsection{Comparison on I and II}
Both solutions yield the same worst-case error. But we can obtain more fine-grained analysis here (in terms of $n$). We first note that $|J| \le n \cdot \Delta_1$, $|J| \le n \cdot \Delta_2$, and $\max\{\Delta_1,\Delta_2\} \le \Delta \le n$. 

In summary, naive Solution 1 always have better error than Naive Solution 2 on the two-table case. 


\noindent To be discussed: 

2. Naive solution 2 is better on efficiency, since $T$ is proportional to the number of records?

What's the optimal choice of $T$ in the $(\epsilon, \delta)$-DP?

3. What's the tradeoff we want to achieve?
\subsection{Next Steps}

1. Change the initial distribution state

2. How to define the score for the Gaussian Mechanism in the existing framework, that adapts to the synthetic data generated for the first table and join information?

3. Restrictive query families

4. When the join size is small

5. Trade-off when two tables have significantly different sizes

\newpage


\subsection{Small Support}

Given a database $R_1(A,B) \Join R_2(B,C)$, we distinguish two more cases for each join value $b \in B$ with respect to $|\sigma_{B=b} R_1|, |\sigma_{B=b} R_2|$. Let $\mathcal{A}_B$ be the set of active join values over $B$.

\begin{enumerate}
    \item if $|\sigma_{B=b} R_1| + |\sigma_{B=b} R_2| \ge 2$, we definitely include $b$ into $\mathcal{A}_B$.
    \item if $|\sigma_{B=b} R_1| + |\sigma_{B=b} R_2| =1$, we discard it with probability $\delta$\;
\end{enumerate}

In this way, we can shrink our support for naive solution II to $n \times \dom(A)$. 

\paragraph{Fact.} Consider two neighboring databases $R = (R_1, R_2)$ and $R' = (R'_1, R'_2)$. Assume $B = \{b \in \dom(B): |\sigma_{B=b} R_1| + |\sigma_{B=b} R_2| \ge 1\}$ and $B' = \{b \in \dom(B): |\sigma_{B=b} R'_1| + |\sigma_{B=b} R'_2| \ge 1\}$. Let $\mathcal{A}_B, \mathcal{A}'_B$ be the sets of active join values released for $(R_1, R_2)$ and $(R'_1, R'_2)$. Let $b,b'$ be the pair of join values such that $|\sigma_{B=b} R_1| + |\sigma_{B=b} R_2| = |\sigma_{B=b} R'_1| + |\sigma_{B=b} R'_2| + 1$, and $|\sigma_{B=b'} R'_1| + |\sigma_{B=b'} R'_2| = |\sigma_{B=b'} R_1| + |\sigma_{B=b'} R_2| + 1$.

\begin{enumerate}
    \item[(1)] If $deg(R', b) \ge 2$ and $deg(R, b') \ge 2$, then they are the same;
    \item[(2)] If one of them decreases to $1$, say $deg(R', b) = 1$, we distinguish two more cases:
    \begin{enumerate}
        \item [(2.1)] $deg(R, b') \ge 2$, $b' \in \mathcal{A}_B$ for sure and $b \in \mathcal{A}'_B$ happens with prob $1-\delta$;
        \item [(2.2)] $deg(R, b') =1$, then both $b' \in \mathcal{A}'_B$ and $b \in \mathcal{A}_B$ happens with prob $(1-\delta)^2$, and both $b' \notin \mathcal{A}_B$ and $b \notin \mathcal{A}'_B$ happens with prob $\delta^2$;
        \item [(2.3)] $deg(R, b') =0$, $b' \notin \mathcal{A}_B$ for sure and $b \notin \mathcal{A}'_B$ happens with prob $\delta$;
    \end{enumerate}
\end{enumerate}


\subsection{Naive solution II}
We release a synthetic dataset $\widetilde{R}_i$ for $R_i$, where $i=1,2,3$. Then, the final function $\F$ is implied automatically:
\[\F(t_1,t_2,t_3) = \widetilde{R_1}(t_1) \cdot \widetilde{R_2}(t_2) \cdot \widetilde{R_3}(t_3) \cdot \rho(t_1,t_2,t_3)\]
for $(t_1, t_2, t_3) \in \D_1 \times \D_2 \times \D_3$.


\paragraph{Error Analysis.} Implied by the single table result, we know for $i \in \{1,2,3\}$:
\begin{align*}
    \max_{q_i \in \Q_i} |q_i(R_i) - q_i(\widetilde{R}_i)| =& O\left(n^{1/2} \cdot f(\mathbb{D}_i, \Q_i, \epsilon, \delta)\right) 
\end{align*}
Now, for an arbitrary query $q = (q_1, q_2, q_3) \in \Q$, we rewrite 
\begin{align*}
    q(R_1, R_2, R_3) =& \sum_{t_2= (b,c) \in \D_2} R_2(t_2) \cdot \alpha_b \cdot \beta_c \\
    q(\F) =& \sum_{t_2= (b,c) \in \D_2} \widetilde{R}_2(t_2) \cdot \widetilde{\alpha}_b \cdot \widetilde{\beta}_c
\end{align*}
where 
\begin{align*}
    \alpha_b &= \sum_{a: t_1 =(a,b)\in \D_1} q_1(t_1) \cdot R_1(t_1) \\
    \widetilde{\alpha}_b &= \sum_{a: t_1 =(a,b)\in \D_1} q_1(t_1) \cdot \widetilde{R}_1(t_1)\\
    \beta_c  &= \sum_{d: t_3 = (c,d) \in \D_3}  q_3(t_3) \cdot R_3(t_3) \\
    \widetilde{\beta}_c &= \sum_{d: t_1 =(c,d)\in \D_3} q_3(t_3) \cdot \widetilde{R}_3(t_3)
\end{align*}
 Note that $\sum_{b \in \mathbb{B}}(\widetilde{\alpha}_b - \alpha_b) \le \sqrt{n}$ and $\sum_{c \in \mathbb{C}}(\widetilde{\beta}_c - \beta_c) \le \sqrt{n}$ (omitting the logarithmic factors here). We have
\begin{align*}
     & q(\F) -  q(R_1, R_2, R_3) \\
     \le & \sum_{t_2 = (b,c) \in \D_2} \left(R_2(t_2) + \widetilde{R}_2(t_2)\right)  \cdot \left(\widetilde{\alpha}_b \widetilde{\beta}_c - \alpha_b \beta_c \right) \\
     = & \sum_{t_2 =(b,c) \in \D_2} \left(R_2(t_2) + \widetilde{R}_2(t_2)\right)  \cdot \left( (\widetilde{\alpha}_b - \alpha_b) \beta_c + (\widetilde{\beta}_c - \beta_c) \alpha_b + (\widetilde{\alpha}_b - \alpha_b)(\widetilde{\beta}_c - \beta_c) \right) \\
     \le & \sum_{b \in \mathbb{B}} \left( (\widetilde{\alpha}_b - \alpha_b) \cdot \sum_{c: t_2 = (b,c) \in \D_2} \left(R_2(t_2) + \widetilde{R}_2(t_2)\right)  \cdot \beta_{c}\right) \\
     + & \sum_{c \in \mathbb{C}} \left( (\widetilde{\beta}_c - \beta_c) \cdot \sum_{b: t_2 = (b,c) \in \D_2} \left(R_2(t_2) + \widetilde{R}_2(t_2)\right)  \cdot \alpha_{b} \right)\\
     + & \sum_{t_2 = (b,c) \in \D_2}  \left(R_2(t_2) + \widetilde{R}_2(t_2)\right)  \cdot (\widetilde{\alpha}_b - \alpha_b)(\widetilde{\beta}_c - \beta_c)
\end{align*}

\paragraph{Worst-case error analysis.} 
\new{In setting 1,} we have $ q(\F) -  q(R_1, R_2, R_3) \le $
\begin{align*}
    \sqrt{n} \cdot (\Delta_{21} + \sqrt{n}) \cdot \Delta_3 + \sqrt{n} \cdot (\Delta_{22} + \sqrt{n}) \cdot \Delta_1 + n \cdot \sqrt{n} \cdot \sqrt{n} \le n^{5/2}
\end{align*}
In the worst case, it is as large as $n^{5/2}$, matching naive solution I. 
%\new{In setting 2,} we have $ q(\F) -  q(R_1, R_2, R_3) \le $\begin{align*} & \sum_{b \in \mathbb{B}} \left( (\widetilde{\alpha}_b - \alpha_b) \cdot \sum_{c: t_2 = (b,c) \in \D_2}\beta_{c}\right) \cdot \sqrt{n}\\  + & \sum_{c \in \mathbb{C}} \left( (\widetilde{\beta}_c - \beta_c) \cdot \sum_{b: t_2 = (b,c) \in \D_2} \alpha_{b} \right) \cdot \sqrt{n}\\ + & \sum_{b \in \mathbb{B}} (\widetilde{\alpha}_b - \alpha_b) \cdot  \sum_{c \in \mathbb{C}} (\widetilde{\beta}_c - \beta_c) \cdot \sqrt{n}\\  \le & \sqrt{n} \cdot n \cdot \sqrt{n} + \sqrt{n} \cdot n \cdot \sqrt{n} + n \cdot \sqrt{n} = n^{2} \end{align*}

\paragraph{Conjecture.} In setting I, the worst-case error over length-$k$ join is $O(n^{k-\frac{1}{2}})$. %and in setting II, the worst-case error over length-$k$ join is $O(n^{\lceil \frac{k+1}{2} \rceil})$.

%\paragraph{Hybrid Strategy} For simplicity, consider the solution of applying naive solution I to $R_1\Join R_2$, and then applying naive solution II to $(R_1 \Join R_2) \Join R_3$. Let $\widetilde{R}_{12}(A,B,C)$ be the released dataset for $R_1\Join R_2$. Note that $|\widetilde{R}_{12}| = |J_{12}| + \max\{\Delta_{1}, \Delta_{21}\}$ with probability at least $1-\delta$, where $J_{12} = R_1 \Join R_2$. Moreover, for any query $q = (q_1, q_2, q_3)$, we have 
%\begin{align*}
%    \max_{q_{12} = (q_1, q_2) \in \Q_1 \times \Q_2} |q_{12}(\widetilde{R}_{12}) - q_{12}(R_1, R_2)| \le & \sqrt{|J_{12}|} \cdot \sqrt{\max\{\Delta_{1}, \Delta_{21}\}} \\
%    \max_{q_3 \in \Q_3} |q_3(\widetilde{R}_3) - q_3(R_3)| \le & \sqrt{n} 
%\end{align*}
%In total, the error of $q$ is
%\begin{align*}
%    q(R_1, R_2, R_3) - q(\widetilde{R}_{12}, \widetilde{R}_3) \le |\widetilde{R}_{12}| \cdot \sqrt{n}  + \sqrt{|\widetilde{R}_{12}|} \cdot n + \sqrt{|\widetilde{R}_{12}|} \cdot \sqrt{n}  
%%\end{align*}
%which is as large as $n^{5/2}$ in the worst case.
%
%Similarly, the symmetric strategy of applying naive solution I to $R_2 \Join R_3$, and then applying naive solution II to $R_1 \Join (R_2 \Join R_3)$. Let $\widetilde{R}_{23} = |R_2 \Join R_3| + \max\{\Delta_3, \Delta_{22}\}$. The error can be achieved is 
%\begin{align*}
%    q(R_1, R_2, R_3) - q(\widetilde{R}_1, \widetilde{R}_{23}) \le  |\widetilde{R}_{23}| \cdot \sqrt{n}  + \sqrt{|\widetilde{R}_{23}|} \cdot n + \sqrt{|\widetilde{R}_{23}|} \cdot \sqrt{n}  
%\end{align*}
%%
%How about the following data partition? t_1iao{In setting 2,} we partition values in $B$ as heavy and light, depending their degree in $R_1$ or $R_2$ with threshold $\tau$. The total error can be achieved:
%\begin{align*}
%   & n\cdot \tau \cdot \sqrt{n}  +     \sqrt{n\cdot \tau} \cdot n + \frac{n^2}{\tau} \cdot \sqrt{n} + \sqrt{\frac{n^2}{\tau}} \cdot n\\
%    & \le n\cdot \tau \cdot \sqrt{n} + \frac{n^2}{\tau} \cdot \sqrt{n} \le n^2
%\end{align*}  by setting $\tau = \sqrt{n}$.
%t_1iao{Observation 1: In terms of wothe hybrid strategy is better than naive solutions in the first setting, but it is always worse than naive solution 2 in the second setting.}
%
%
%\paragraph{Setting 1 v.s. Stetting 2:} Duplicated tuples with multiplicity v.s. Distinct tuples.
%\begin{center}
%\begin{tabular}{ |c|c|c| } 
% \hline
% & Setting 1 & Setting 2 \\
% \hline
%Naive Solution I & $O(n^{5/2})$ & $O(n^{2})$ \\ 
% \hline
% Naive Solution II & $O(n^{5/2})$ & $O(n^{3/2})$ \\ 
%  \hline
%Hybrid & -- & $O(n^{2})$ \\ 
% \hline
%\end{tabular}
%\end{center}
%
%But naive solution I is always instance-dependent. 
%
%\paragraph{The Net Mechanism.} An $\alpha$-net of query families. A random sample of the underlying database => A random sample of the join result table without materializing the join results. 

\newpage


\section{Space and Error Trade-off}

\subsection{Two-table Join}
\xiao{This is incorrect. For both solutions, the support/space is as large as the domain, although the sum of frequencies can be bounded.}
Naive solution 1: 
\begin{enumerate}
    \item support size $\D$
    \item frequency sum is $S = |J| + \Delta$
    \item error is $O(\sqrt{J} \cdot \sqrt{\Delta} + \Delta)$
\end{enumerate}
Naive solution 2: 
\begin{enumerate}
    \item support size $\D$ \xiao{can we improve this further?})
    \item frequency sum is $S = n$
    \item error is $O(\Delta_1 \cdot \sqrt{n_2} + \Delta_2 \cdot \sqrt{n_1})$.
\end{enumerate}


Since $\Delta_1 \cdot n_2 \ge J$ and $\Delta_2 \cdot n_1 \ge J$, so $\sqrt{J} \cdot \sqrt{\Delta_1} \le \Delta_2 \cdot \sqrt{n_1}$. Note that $\Delta= \max\{\Delta_1, \Delta_2\}$.

\paragraph{Observation.} they have the same error on Cartesian product instance, where $J = n_1 \cdot \Delta_2$ or $J = n_2 \cdot \Delta_1$.

\paragraph{Idea.}
For each possible join key $b \in \mathbb{B}$, let $\deg_1(b), \deg_2(b)$ be the number of tuples in $R_1, R_2$ that have join value $b$, separately.

Fix a threshold $\tau$.
For each possible join key, 
Consider $\widetilde{\deg}_1(b) = \deg_1(b) + \eta$ where $\eta \sim Lap(\frac{1}{\epsilon})$, and $\widetilde{\deg}_2(b) = \deg_2(b) + \eta'$ where $\eta' \sim Lap(\frac{1}{\epsilon})$. If $\widetilde{\deg}_1(b) \ge \tau$ and $\widetilde{\deg}_2(b) \ge \tau$, we identify this join value $b$ as heavy. There are two possible choices here: (1) invoke naive solution 2 to each heavy key separately, with error $O(\sum_b \sqrt{J_b} \cdot \sqrt{\Delta_b} = \sum_b \sqrt{n_b} \cdot \Delta_b)$; (2) invoke naive solution 2 to all heavy keys as whole, with error $O(\max_b \Delta_b \cdot \sqrt{\sum_b n_b})$. As these two solution are incomparable, we will always choose the smaller one achieving the error as:
\[\min\left\{\sum_b \sqrt{n_b} \cdot \Delta_b, \max_b \Delta_b \cdot \sqrt{\sum_b n_b}\right\} \le \min \left\{ \sqrt{J \cdot \frac{n}{\tau}} \cdot \sqrt{\Delta}, \sqrt{n} \cdot \Delta\right\}\]
Choosing which solution depends on whether $\frac{J}{\Delta} > \tau$ or not. 




For remaining $b$'s, where  $\widetilde{\deg}_1(b) <\tau$ or  $\widetilde{\deg}_2(b) <\tau$, we invoke naive solution 1 to all related tuples. 

\xiao{This analysis is incorrect about space usage.}
\begin{enumerate}
    \item Heavy: 
    \begin{enumerate}
        \item[] Space: almost to $O(n)$.
        \item[] Error: $\min \left\{ \sqrt{J \cdot \frac{n}{\tau}} \cdot \sqrt{\Delta}, \sqrt{n} \cdot \Delta\right\}$.
    \end{enumerate}
    \item Light:
    \begin{enumerate}
        \item[] Space: almost to $O(n \cdot \tau)$.
        \item[] Error: $\sqrt{J} \cdot \sqrt{\Delta}$.
    \end{enumerate}
\end{enumerate} 

\noindent Together, we use $O(n \cdot \tau)$ space and achieved $O\left(\min \left\{ \sqrt{J \cdot \frac{n}{\tau}} \cdot \sqrt{\Delta}, \sqrt{n} \cdot \Delta\right\} + \Delta \right)$ error for two-table case. 
\fi

\newpage

\section{Self-Join over Graph}

For counting subgraph size:\\
1. Computational hardness on SS: NP-hard for 2-triangles and cycles of length 4~\cite{karwa2011private} \\
2. Ladder function~\cite{zhang2015private}


%\subsection{Length-3 Path}
%
%Consider the length-3 path join case. 
%
%
%\paragraph{Strategy 1.} We release synthetic data for $R_1 \Join R_2$ and $R_3$ separately. We define $\widetilde{J}_{12} = J_{12} + \Delta(b, R_1) + \Delta(b,R_2)$.
%\\
%
%Space: $J_{12} + \Delta(b, R_1) + %\Delta(b,R_2)$. \\
%
%\begin{align*}
%    \alpha \le& \Delta(c,R_3) \cdot \sqrt{\widetilde{J}_{12}} + \Delta(c, R_1\Join R_2)\cdot \sqrt{n} \\
%    \le& \Delta(c,R_3) \cdot \sqrt{J_{12}} +\Delta(c,R_3) \cdot \sqrt{\Delta(b, R_1)} + \Delta(c,R_3) \cdot \sqrt{\Delta(b, R_2)} \\
%    +& \Delta(c, R_1\Join R_2) \cdot \sqrt{n}\\
%\end{align*}
%
%\paragraph{Strategy 2.} We release synthetic data for $R_1$ and $R_2 \Join R_3$ separately. We define $\widetilde{J}_{23} = J_{23} + \Delta(c,R_2) + \Delta(c,R_3)$. \\
%
%Space: $J_{23} + \Delta(c,R_2) + \Delta(c,R_3)$. %\\
%
%\begin{align*}
%    \alpha & \le \Delta(b,R_1) \cdot \sqrt{\widetilde{J}_{23}} + \Delta(b,R_2 \Join R_3)  \cdot \sqrt{n} \\
%    & \le \Delta(b,R_1) \cdot \sqrt{J_{23}} + \Delta(b,R_1) \cdot \sqrt{\Delta(c,R_2)} + \Delta(b,R_1) \cdot \sqrt{\Delta(c,R_3)} \\
%    & + \Delta(b, R_2 \Join R_3) \cdot \sqrt{n} 
%\end{align*}
%
%
%Given space usage $\tau$, what's the best error that can be achieved?
%Now, let's take a more careful inspection of $LS_\countsize(\I)$. For any neighboring instance $\I'$ of $\I$, there are three possible changes between $\I,\I'$, i.e., one tuple has its frequency +1/-1 in $\D_1$, or $\D_2$, or $\D_3$. For an change in $\D_1$, the maximum change in $\countsize(\I)$ is 
%\[ \max_{b\in \mathbb{B}} \sum_{x_2 \in \D_2: \pi_{B} x_2 = b}R_2(x_2) \cdot \sum_{x_3 \in \D_3: \pi_C x_3 = \pi_C x_2} R_3(x_3) \]
%The case for an change in $\D_3$ is symmetric. For an change in $\D_2$, the maximum change in $\countsize(\I)$ is
%\[\max_{b \in \mathbb{B},c \in \mathbb{C}} \left(\sum_{x_2 \in \D_2: \pi_{B} x_2 = b} R_2(x_2)\right) \cdot \left(\sum_{x_3 \in \D_3: \pi_C x_3 = c} R_3(x_3)\right) \le \Delta_1 \cdot \Delta_3\]
%Corresponding to these three different cases, we now derive the exact form of the local sensitivity: 
%\begin{enumerate}[leftmargin=*]
%    \item[] \new{Setting 1: } $ LS_\countsize(\I) 
%    \le \max\{\Delta_{21} \cdot \Delta_3, \Delta_{22} \cdot \Delta_1, \Delta_1 \cdot \Delta_3\}$.
%    \item[] \new{Setting 2: } $ LS_\countsize(\I) \le \max\{n, \Delta_1 \cdot \Delta_3\}$.
%\end{enumerate}
%
%\paragraph{Worst-case error.} 
%\new{In setting 1,} $J(\I) = O(n^3)$ and $LS_\countsize(\I) = n^2$, so the error that can be achieved is as large as 
%\[O\left(n^{5/2} \cdot f(\D, \Q, \epsilon, \delta) + n^2 \cdot \frac{1}{\epsilon} \log \frac{1}{\delta} \right)\]
%which is better than random guessing since for any query $q \in \Q$, $q(\I) \in [-n^3, n^3]$. %\new{In setting 2,} $J(\I) = O(n^2)$ and $LS_\countsize(\I) = n^2$, so the error that can be achieved is as large as \[O\left(n^2 \cdot f(\D, \Q, \epsilon, \delta) \right)\] Note that $q(\I) \in [-n^2, n^2]$ for any query $q \in \Q$.


%Let $\mathbb{A}, \mathbb{B}, \mathbb{C}, \mathbb{D}$ be the domain of attribute $A, B,C,D$ separately. Define $\D_1 = \mathbb{A} \times \mathbb{B}$, $\D_2 = \mathbb{B} \times \mathbb{C}$ and $\D_3 = \mathbb{C} \times \mathbb{D}$. We consider three families of linear queries: $\Q_i = \{q_i: \D_i \to [-1,+1]\}$ for $i =1,2,3$. Then, for each query $q_i \in \Q_i$, we define $q_i(R_i) = \sum_{x_i \in \D_i} R_i(x_i) \cdot q_i(x_i)$ for $i =1,2,3$. Let $\Q = \Q_1 \times \Q_2 \times \Q_3$. We consider the simple natural join function $\rho: \D_1 \times \D_2 \times \D_3 \to \{0,1\}$ such that $\rho(x_1, x_2, x_3)=1$ for $(x_1, x_2, x_3) \in \D_1 \times \D_2 \times \D_3$ if and only if $\pi_B x_1 = \pi_B x_2$ and $\pi_{C} x_2 = \pi_C x_3$. 
%
%\new{Setting 1:} Define $R_i: \D_i \to \mathbb{Z}$ for $[3]$. 
%
%\new{Setting 2:} 
%Define $R_i: \D_i \to \{0,1\}$ for $i = 1,2,3$.
%
%\medskip
%For each query $q = (q_1, q_2, q_3) \in \Q$,  $q(R_1, R_2, R_3) = $
%\[\sum_{(t_1,t_2,t_3) \in \D_1 \times \D_2 \times \D_3} \rho(t_1,t_2,t_3) %\cdot  \prod_{i\in [3]} q_i(t_i) \cdot R_i(t_i)\]
%

\paragraph{Hard Instance Construction in Lower Bound.} For arbitrary parameters $\OUT>0$ and $\Delta >0$ with $\OUT > \Delta$, it suffices to show a path-3 instance $\I$ of join size $\OUT$ and local sensitivity $\Delta$, such that if there exists any $(\epsilon, \delta)$-DP algorithm answering linear queries over $\I$ with $\ell_\infty$ error as: $\alpha = O\left(\sqrt{\OUT} \cdot \sqrt{\Delta} \right)$, then there is an algorithm for solving linear queries over any single table of input size  $n = \frac{\OUT}{\Delta}$ with $\ell_\infty$ error as: $\alpha'= O\left(\sqrt{n}\right)$. 

Suppose we are given a single table $R$ of size $n$ over domain $\D$. We first construct $3$ domains $\{\D_1, \D_2, \D_3\}$ such that $|\D_i| = 2|\D|$ and $\D \subseteq \D_1$. All records in $\D_1$ have the distinct join value in $B$. There are $n$ records in $R_2$ as a one-to-one mapping from $B$ to $C$. There are $\Delta$ records in $R_3$ sharing the same join value in $C$.  It can be easily checked that join size is $n \cdot \Delta = \OUT$, and local sensitivity is $\Delta$.  

\xiao{\paragraph{How large is the gap between $LS_\countsize(\I)$ and $SS_\countsize(\I)$ on path-3 join?}} We note that
\begin{align*}
    RS_\countsize(\I) &= \max_{E \subsetneq [m]} T_{E}(\I) \\
    LS_\countsize(\I) &= \max_{E = [m] - \{i\}: i \in [m]} T_{E}(\I)
\end{align*}
Observe that $T_{E}(\I) = 1$ for any $E \subseteq [m]$ with $|E| \ge 2$. Then, we have $RS_\countsize(\I) = LS_\countsize(\I)$ on path-3 join.

\xiao{\paragraph{Extension to path-$m$ join.}} The gap can be as large as $(n-1)^{\lceil \frac{m-2}{2}\rceil}$ on path-$m$ join query of input size $n$, similar to the star case. 



\begin{definition}[Admissible Noise Distribution]
A probability distribution on $\mathbb{R}$, given by a density function $h$, is $(\alpha, \beta)$-admissible, if for $\alpha = \alpha(\epsilon, \delta)$ and $\beta = \beta(\epsilon, \delta)$, the following two conditions holds for all $\Delta \le \alpha$ and $\lambda \le \beta$, and for all measurable subsets $S \subseteq \mathbb{R}$:
\begin{enumerate}
    \item $\Pr[Z \in S] \le e^{\frac{\epsilon}{2}} \cdot Pr[Z \in S + \Delta] + \frac{\delta}{2}$\;
    \item $\Pr[Z \in S] \le e^{\frac{\epsilon}{2}} \cdot e^\lambda \cdot Pr[Z \in e^\lambda \cdot S] + \frac{\delta}{2}$\;
\end{enumerate}
\end{definition}


\paragraph{Shifted and truncated Laplacian Distribution.} Define $\textsf{Lap}_b(x) = e^{-\frac{|x|}{b}}$. Let $n_0$ be the smallest integer such that 
\[\Pr\left[\left|\textsf{Lap}_{\frac{\Delta}{\epsilon}}(x)\right| > n_0\right] \le \delta\]
where $n_0 = \frac{\Delta}{\epsilon} \ln \frac{1}{\delta}$. 
\begin{lemma}
    For any two integers $u,v$ with $|u-v| \le \Delta$, we have 
    \[ u + \textsf{STLap}_{\epsilon, \delta, \Delta}(x) \sim_{(\epsilon, \delta)} v + \textsf{STLap}_{\epsilon, \delta, \Delta}(x)\]
\end{lemma}


Let $n_0 = \ln \frac{1}{\delta}$. The shifted and truncated laplacian distribution $\textsf{STLap}_{\epsilon, \delta, 1}(x)$ has support in $[0, 2 n_0]$, and is defined as 
\[\min\left\{ \max \left\{0, n_0 + \textsf{Lap}_1 (x) \right\}, 2n_0 \right\}\]




\begin{lemma}
    Let $h$ be an $(\alpha, \beta)$-admissible noise probability density function, and let $Z$ be a fresh random variable sampled according to $h$. For a function $f$, let $S$ be a $\beta$-smooth upper bound on the local sensitivity of $f$. Then the algorithm $\mathcal{A}(x) = f(x) + \frac{S(x)}{\alpha} \cdot Z$ is $(\epsilon, \delta)$-differentially private.
\end{lemma}

\begin{lemma}
    \textsf{STLap}$(\epsilon, \delta,1)$ is $(\frac{\epsilon}{2}, \frac{\epsilon}{2 \ln \frac{2}{\delta}})$-admissible.
\end{lemma}

\begin{proof}
    For any $-\frac{\epsilon}{2} \le t \le \frac{\epsilon}{2}$, we need to first show the following inequality holds for any $y \in \mathbb{R}$:
    \begin{align*}
        \Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y) \le e^{\frac{\epsilon}{2}} \cdot \Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y + t) + \frac{\delta}{2}  \ \ \ (*)
    \end{align*}
    Let $n_0 = \ln \frac{2}{\delta}$. We distinguish the following three cases.
    \begin{enumerate}[leftmargin=*]
        \item[(1)] $y < 0$ or $y > 2n_0$. $(*)$ holds since $\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y) = 0$.
        \item[(2)] $y = 2n_0$ or $y = 0$. $(*)$ holds since $\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y) = \frac{\delta}{2}$ and $\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y + t) \ge 0$.
        \item[(3)] $0 < y < 2n_0$. We further distinguish three more cases: 
        \begin{enumerate}
            \item[(3.1)] $0 < y + t < 2n_0$. $(*)$ always holds since 
            \begin{align*}
                \frac{\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y)}{\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y + t)} &=  \frac{\Pr(\textsf{Lap}_{1}(x) = y -n_0)}{\Pr(\textsf{Lap}_{1}(x) = y + t - n_0)} \\
                &= \exp(t) \le \exp(\frac{\epsilon}{2}) 
            \end{align*}
            \item[(3.2)] $y + t = 0$ or $y+t = 2n_0$. We first have $\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y + t) = \frac{\delta}{2}$. If $y + t = 0$, as $y>0$, $\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y) \le \Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = \frac{\epsilon}{2}) = \Pr(\textsf{Lap}_{1}(x) = \frac{\epsilon}{2} - n_0) = \exp(-|\frac{\epsilon}{2} - n_0|) =  \exp(-\frac{\epsilon}{2} + n_0) =  \frac{\delta}{2} \cdot \exp(-\frac{\epsilon}{2})$. $(*)$ always holds since
            \[\frac{\delta}{2} \cdot \exp(-\frac{\epsilon}{2}) \le \frac{\delta}{2} \cdot \exp(\frac{\epsilon}{2}) + \frac{\delta}{2}\]
            The case with $y+t = 2n_0$ is similar. 
        \end{enumerate}
    \end{enumerate}
    
    For any $-\frac{\epsilon}{2 \ln \frac{2}{\delta}} \le\lambda \le \frac{\epsilon}{2 \ln \frac{2}{\delta}}$, we need to show the following inequality holds for any $y \in \mathbb{R}$:
    \[\Pr[\textsf{STLap}_{\epsilon, \delta, 1}(x) = y] \le e^{\frac{\epsilon}{2}} \cdot \Pr[\textsf{STLap}_{\epsilon, \delta, 1}(x) = e^\lambda \cdot y ] + \frac{\delta}{2}\]
    
    Let $n_0 = \ln \frac{1}{\delta}$. We distinguish the following three cases.
    \begin{enumerate}[leftmargin=*]
        \item[(1)] $y < 0$ or $y > 2n_0$. $(*)$ holds since $\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y) = 0$.
        \item[(2)] $y = 2n_0$ or $y = 0$. $(*)$ holds since $\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y) = \frac{\delta}{2}$ and $\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = e^\lambda \cdot y) \ge 0$.
        \item[(3)] $0 < y < 2n_0$ and $\lambda > 0$. Here, $0 < e^\lambda \cdot y$ also holds. We further distinguish three more cases: 
        \begin{enumerate}
            \item[(3.1)] $0 < y \le n_0/e^\lambda$. Here, $0< e^\lambda \cdot y \le n_0$. 
            \begin{align*}
                \frac{\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y)}{e^\lambda \cdot \Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = e^\lambda \cdot y)} &=  \frac{\Pr(\textsf{Lap}_{1}(x) = y-n_0)}{e^\lambda \cdot \Pr(\textsf{Lap}_{1}(x) = e^\lambda \cdot y - n_0)} \\
                &\le \frac{1}{e^\lambda}  \le 1 \le e^{\frac{\epsilon}{2}}
            \end{align*}
            \item[(3.2)] $n_0/e^\lambda < y <n_0$. Here, $n_0 < e^\lambda \cdot y \le 2n_0$. 
            \begin{align*}
                \frac{\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y)}{e^\lambda \cdot \Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = e^\lambda \cdot y)} &=  \frac{\Pr(\textsf{Lap}_{1}(x) = y-n_0)}{e^\lambda \cdot \Pr(\textsf{Lap}_{1}(x) = e^\lambda \cdot y - n_0)} \\
                 &= \frac{1}{e^\lambda} \cdot \frac{\exp(y-n_0)}{\exp(-e^\lambda \cdot y+n_0)} \\
                &= \frac{4}{e^\lambda \cdot \delta^2} \cdot \exp(y(1-e^\lambda))\\ 
                &\le \frac{4}{e^\lambda \cdot \delta^2} \cdot \exp(\frac{n_0}{e^\lambda}(1-e^\lambda)) \\
                &\le \frac{4}{e^\lambda \cdot \delta^2} \cdot \delta^{\frac{1-e^\lambda}{e^\lambda}}
            \end{align*}
            \item[(3.3)] $n_0 < y \le 2n_0/e^\lambda$. Here, $n_0 < e^\lambda \cdot y \le 2n_0$. $(*)$ holds since 
            \begin{align*}
                \frac{\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y)}{e^\lambda \cdot \Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = e^\lambda \cdot y)} &=  \frac{\Pr(\textsf{Lap}_{1}(x) = y - n_0)}{e^\lambda \cdot \Pr(\textsf{Lap}_{1}(x) = e^\lambda \cdot y - n_0)} \\
                &= \frac{1}{e^\lambda} \cdot \frac{\exp(-y+n_0)}{\exp(-e^\lambda \cdot y+n_0)} \\
                &= \frac{1}{e^\lambda} \cdot \exp(-y(1-e^\lambda) \\ 
            \end{align*}
            \item[(3.4)] $y > 2n_0/e^\lambda$. In this case, $e^\lambda \cdot y > 2n_0$, thus $\Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = e^\lambda \cdot y) = 0$ and 
            \begin{align*}
                \Pr(\textsf{STLap}_{\epsilon, \delta, 1}(x) = y) &= \Pr(\textsf{Lap}_{1}(x) = y - n_0) \\
                =& \exp(-y+n_0) \le \exp(-\frac{2n_0}{e^\lambda} + n_0) \\
                =& \left(\frac{\delta}{2}\right)^{\frac{2}{e^\lambda} -1} \le \frac{\delta}{2}
            \end{align*}
            since $e^\lambda > 1$.
        \end{enumerate}
    \end{enumerate}
    
\end{proof}
%\begin{definition}
%    Let $h$ be an $(\alpha, \beta)$-admissible noise probability density function, and let $Z$ be a fresh random variable sampled according to $h$. For a function $f$, let $S$ be a $\beta$-smooth upper bound on the local sensitivity of $f$. Then algorithm $\mathcal{A}(x) = f(x) + \frac{S(x)}{\alpha} \cdot Z$ satisfies $(\epsilon, \delta)$-DP.
%\end{definition}
%Consider a pair of neighboring instances $\I,\I'$. Let %$J,J'$ be the join results over $\I,\I'$ respectively.
%Let $\Delta,\Delta'$ be the two noises added to two neighboring instance $\I,\I'$.
%\begin{proof}
%\begin{align*}
%     \frac{\Pr\left(|J|+ \frac{SS_\countsize(\I)}{\epsilon} \textsf{Lap}(1) = z\right)}{\Pr\left(|J'| + \frac{SS_\countsize(\I')}{\epsilon} \textsf{Lap}(1)=z\right)} &= \frac{\Pr\left(\textsf{Lap}(1) = \epsilon \cdot \frac{z-|J|}{SS_\countsize(\I)} \right)}{\Pr\left(\textsf{Lap}(1) = \epsilon \cdot \frac{z-|J'|}{SS_\countsize(\I')} \right)} \\
%     &= \exp\left(\big|\epsilon \cdot \frac{z-|J|}{SS_\countsize(\I)}\big| - \big|\epsilon \cdot \frac{z-|J'|}{SS_\countsize(\I')}\big|\right) \\
%     &= \exp\left(\epsilon \cdot \big|\frac{z-|J|}{SS_\countsize(\I')} - \frac{z-|J'|}{SS_\countsize(\I')}\big|  \right)
%\end{align*}
%\end{proof}
%Since $\textsf{Var}[\eta] =2$, the noise level is $\frac{2\sqrt{2}}{\epsilon} SS_\countsize(\I)$.

\begin{lemma}
    Algorithm~\ref{alg:multi-table} preserves $(3\epsilon, 3 \delta)$-DP.
\end{lemma}


%Several different notions of sensitivity have been proposed for achieving the best tradeoff between the utility (the sensitivity should be as small as possible, as
%the noise level is proportional. Adding noise with a magnitude greater than the actual query answer would completely
%destroy its utility) and the efficiency (the sensitivity should be computed efficiently). Below, we review some representative results, and all of them can be computed in poly-nominal time in terms of the data size.

 %\paragraph{Remark.} $LS_\countsize(\I) \le SS_\countsize(\I) \le RS_\countsize(\I) \le GS_\countsize(\I)$. Moreover, $RS_\countsize(\I)$ is a constant-approximation of $SS_\countsize(\I)$. But the gap between $LS_\countsize(\I)$ and $SS_\countsize(\I)$ can be as large as polynomial in terms of data size; and the same observation applies for $RS_\countsize(\I)$ and $GS_\countsize(\I)$.
 %
 %\medskip
 %All these works focus on answering counting join size query in a differentially private way, and answering multiple queries has not been investigated yet. 
 
 
 %\xiao{\paragraph{Sensitivity of $\widehat{J}$.}} Now we consider the sensitivity of the scoring function in the exponential mechanism. For two neighboring databases $(R_1, R_2), (R'_1, R'_2)$, let $\widehat{J}, \widehat{J'}$ as the datasets generated by Algorithm~\ref{alg:two-table} in line 1-5, respectively. \begin{align*}
%%    \lambda = &\max_q \max_i \big|s_i(\widehat{J}, q) - s_i(\widehat{J'}, q) \big| \\
%    = &\max_q \max_i \big| |q(\F_{i-1}) - q(\widehat{J})| - |q(\F_{i-1}) - q(\widehat{J'})| \big| \\
%    \le & \max_q \big| q(\widehat{J}) - q(\widehat{J'}) \big| \\
%    \le  & \max_q \big|q(J) + q(\widetilde{J}) - q(J') - q(\widetilde{J'}) \big| \\
%    \le & \max_q |q(J) - q(J')| + |\widetilde{J}| + |\widetilde{J'}| \\
%    \le & \Delta + \Delta + \frac{2}{\epsilon} \log \frac{1}{\delta} + O(1) + \Delta + 1 + \frac{2}{\epsilon} \log \frac{1}{\delta} + O(1) \\
%    = & O\left(\Delta + \frac{1}{\epsilon} \log \frac{1}{\delta}\right)
%\end{align*}
%We next consider the sensitivity used by the Laplace mechanism. Similarly, for two neighboring databases $(R_1, R_2), (R'_1, R'_2)$, let $\widehat{J}, \widehat{J'}$ as the datasets generated by Algorithm~\ref{alg:two-table} in line 1-5, respectively.
%\begin{align*}
%    \lambda = & \max_q |q(J) -q(J')| \\ %\le \Delta
%    \le & \max_q |q(J) + q(\widetilde{J}) - q(J') - q(\widetilde{J'})| =  %O\left(\Delta + \frac{1}{\epsilon} \log \frac{1}{\delta}\right)
%\end{align*}
%following the same argument as the analysis above.

%Moreover, the following fact holds for every query $q \in \Q$: \[|q(R_1, R_2) - q(\widehat{J})| = |q(R_1, R_2) - q(J) - q(\widetilde{J})| = |q(\widetilde{J})| \le |\widetilde{J}|\] Together, we can show every query $q \in \Q$: \begin{align*} \xiao{|q(R_1, R_2) - q(\F)| \le} & \xiao{|q(\widehat{J}) - q(\F)| + |q(R_1, R_2) - q(\widehat{J})|} \\ =& O\left( |\widehat{J}|^{1/2} \cdot \lambda^{1/2} + |\widetilde{J}| \right)\end{align*}
%Note that $|\widetilde{J}| = O\left(\frac{\widetilde{\Delta}}{\epsilon} \log \frac{1}{\delta}\right) = O\left((\Delta + \frac{1}{\epsilon} \log \frac{1}{\delta}) \cdot \frac{1}{\epsilon} \log \frac{1}{\delta}\right)$ and $\lambda = O\left(\Delta + \frac{1}{\epsilon} \log \frac{1}{\delta}\right)$. We have 
%\[|\widehat{J}| = |J + \widetilde{J}| = |J| + |\widetilde{J}| = O\left(|J| + (\Delta + \frac{1}{\epsilon} \log \frac{1}{\delta}) \cdot \frac{1}{\epsilon} \log \frac{1}{\delta} \right) \]
%\xiao{Putting every together, the error achieved is  (omitting the factors of $f(\mathbb{D}, \Q, \epsilon, \delta)$ and $\frac{1}{\epsilon} \log \frac{1}{\delta}$):}
%\begin{align*}   \xiao{O\left( \sqrt{|J| + \Delta} \cdot \sqrt{\Delta} + \Delta \right) =  O\left( \sqrt{|J|} \cdot \sqrt{\Delta} + \Delta  \right) } \end{align*}


%We first introduce some terminologies. For each $i \in [m]$, a subset $\y \subseteq \x_i$ is a {\em prefix} of $\x_i$, if the following property holds: for any pair of attributes $x, x'$, if $x \in \y$ and $E_x \subseteq E_{x'}$, there must be $x' \in \y$. Intuitively, $\y$ is a sub-path of the root-to-node path corresponding to $\x_i$, starting from the root. Let $\sigma: [m] \times 2^{[\x]} \to \mathbb{Z} \cup \{\perp\}$ be a characterization of input instance, such that $\sigma(i, \y) \neq \perp$ if and only if $\sigma(i,\y)$ if $\y$ is a prefix of $\x_i$. For each $i \in [m]$, we define the degree function $\degg_i: 2^{\x_i} \times \{\dom(\y): \y \subseteq \x_i\} \to \mathbb{Z}$, such that 
%\[\degg_i(\y, \Vec{y}) = \sum_{t \in \D_i: \pi_{\y} t = \Vec{y}} R_i(t)\]
%i.e., the degree of vector $\Vec{y}$ over attributes $\y$ in relation $R_i$. 

%\begin{displaymath}
%T_E = \max \left\{ \begin{array}{ll}\displaystyle{\max_{b \in \dom(B)} \degg_1(B, b) \cdot \max_{c \in \dom(C)} \degg_3(C, c)} &\\\displaystyle{\max_{b \in \dom(B)}} \sum_{c \in \dom(C)} R_2(b,c) \cdot \degg_3(C, c) & \\\displaystyle{\max_{c \in \dom(C)}} \sum_{b \in \dom(B)} R_2(b,c) \cdot \degg_1(B,b) & \end{array} \right. 
%\end{displaymath}

==> backup/range.tex <==
\section{Range Counting Queries}

Given a set of points $P \subseteq \mathcal{U}$, where $\mathcal{U}$ is the universe, the goal is to release a differentially private data structure of $P$, so that for any query $Q \subseteq \mathcal{U}$ from a certain query family $\mathcal{Q}$, we can find the count $|P \cap Q|$ as accurate as possible. 

We are interested in query families in constant-dimensional Euclidean space. More precisely, the dataset $P$ consists of $n$ points from $\mathcal{U} = [u]^d$, while $\mathcal{Q}$ consists of geometric ranges of a certain type, e.g.,(axis-parallel) rectangles. 

For $d =1$, the only interesting range space is the set of intervals. For this case, Dwork et al. \cite{} present an $(\epsilon, 0)$-DP algorithm with error $O(\frac{1}{\epsilon} \log^{1.5} u)$, as well as a lower bound of $\Omega(\frac{1}{\epsilon} \cdot \log u)$. For $d \ge 2$, the axis-parallel rectangle queries with error $O(\frac{1}{\epsilon} \cdot \log^{1.5d} u)$, which is later improved to $O(\frac{1}{\epsilon} (\log u + \log^{1.5d} n))$.

\subsection{Two-table Join}

Consider two relations $R_1(A,B) \Join R_2(B,C)$, where $\D_A = \D_B = \D_C = [u]$, and $\mathcal{Q} = \mathcal{Q}_1 \times \mathcal{Q}_2$ for $\Q_1, \Q_2$ being the family of intervals over $\D_A, \D_C$ separately.

Let $\Delta$ be the maximum degree of join values in attribute $B$. 

\paragraph{Naive Solution I:} 
We first materialize the join results as $J(A,B,C)$, and invoke the two-dimensional algorithm for answering axis-parallel rectangle queries over $A,C$. Note that inserting or deleting a tuple will affect $\Delta$ records in $J(A,B,C)$, so each partial sum will be added with noise randomly sampled from $\textsf{Lap}\left(\Delta \cdot \frac{\log^2 u}{\epsilon}\right)$. Moreover, each query answers can be represented as $O(\log^2 u)$ partial-sums. Implied by the previous result, the overall error can be achieved is 
\[O\left(\Delta \cdot \frac{\log^2 u}{\epsilon} \cdot \sqrt{\log^2 u} \cdot \log \frac{1}{\delta}\right) =O\left(\Delta \cdot \frac{\log^3 u}{\epsilon} \cdot \log \frac{1}{\delta}\right) \]
with probability at least $1- \delta$. In the worst case, this error could be as large as $O\left(n \cdot \frac{\log^3 u}{\epsilon} \cdot \log \frac{1}{\delta}\right)$.

\paragraph{Naive Solution II:} For each join value $b$ with $\sigma_{B = b} R_1 \neq \emptyset$ or $\sigma_{B = b} R_2 \neq \emptyset$, we build 1D data structure over attributes $A,C$ separately. The error overall is 
\[O\left(\min\{u,n\} \cdot \frac{1}{\epsilon} \cdot \log^3 u \cdot \log \frac{1}{\delta}\right)\]
which is always worse than naive solution I. 

For each join value $b \in B$, if $|\sigma_{B =b} R_1| \ge \tau$ or $|\sigma_{B =b} R_2| \ge \tau$, we invoke the following strategy: build 1d index for tuples in $\sigma_{B =b} R_1$ and $\sigma_{B =b} R_2$ separately. The error achieved is 
\begin{align*}
    & \sum_{b \textrm{is heavy}}\Tilde{q}_1(\sigma_{B =b} R_1) \cdot \Tilde{q}_2(\sigma_{B =b} R_2) - q_1(\sigma_{B =b} R_1) \cdot q_2(\sigma_{B =b} R_2)\\
    &\le n \cdot \frac{1}{\epsilon} \cdot \log^{1.5} u \cdot \log \frac{1}{\delta} + \frac{n}{\tau} \cdot \frac{1}{\epsilon} \cdot \log^3 u \cdot \log \frac{1}{\delta}
\end{align*}

For light join values, we materialize their join results as $J(A,B,C)$ and invoke the naive solution I, whose error is bounded by  
\begin{align*}
    O\left(\tau \cdot \frac{1}{\epsilon} \cdot \log^3 u \cdot \log \frac{1}{\delta} \right)
\end{align*}


\section{summary}

1. Naive solution I is optimal for error, with respect to $|J|$ and $LS_\count$;

2. Space tradeoff: how to improve naive solution II with small support?




==> backup/star.tex <==
\newpage
\newpage
\subsection{Star}

\paragraph{Problem definition.} Consider an arbitrary integer $i \in [m]$. A table $R_i$ defined over domain $\D_i$ can be represented as a function $R_i: \D_i \to \mathbb{Z}$, where $R_i(x)$ indicates the frequency of data item $x \in \D_i$ in $R_i$. We consider $k$ families of linear queries: $\Q_i = \{q_i: \D_i \to [-1,+1]\}$. Then, for each query $q_i \in \Q_i$, we define $q_i(R_i) = \sum_{x \in \D_i} R_i(x) \cdot q_i(x)$. Then, we define a family of linear queries $\Q = \Q_1 \times \Q_2 \times \cdots \times \Q_k$, such that for each query $q = (q_1, q_2, \cdots, q_k) \in \Q$, 
\[q(R_1, \cdots, R_k) = \sum_{(x_1, \cdots, x_m) \in \D_1 \times \cdots \times \D_m} \rho(x_1,\cdots, x_m) \prod_{i=1}^k  q_i(x) \cdot R_i(x) \]
where $\rho: \D_1 \times \cdots \times \D_m \to \{0,1\}$ is the join function indicating $(x_1, \cdots, x_m) \in \D_1 \times \cdots \times \D_m$ can be joined if $\rho(x_1, \cdots, x_m) = 1$ and can not be joined otherwise. The question is how to release a function $\F: \D_1 \times \cdots \times \D_m \to \mathbb{N}$ such that all queries in $\Q$ can be answered over $\F$ accurately, i.e.,
\[\min \max_{q \in \Q} |q(R_1, \cdots, R_k) - q(\F)| \]
where for any query $q = (q_1, q_2, \cdots, q_k) \in \Q$,
\[q(\F) = \sum_{(x_1, \cdots, x_m) \in \D_1 \times \cdots \times \D_m}  \F(x_1, \cdots, x_m) \cdot \prod_{i=1}^k q_i(x_i)\]
while providing $(\epsilon, \delta)$-differential privacy?


\paragraph{Hard Instance Construction in Lower Bound.} For arbitrary parameters $\OUT>0$ and $\Delta >0$ with $\OUT > \Delta$, it suffices to show a hard star instance $\I$ of join size $|J| = \OUT$ and local sensitivity $LS_\countsize(\I) = \Delta$, any $(\epsilon, \delta)$-DP algorithm solve it with $\ell_\infty$ error as $O\left(\sqrt{\OUT} \cdot \sqrt{\Delta} \right)$, then there is an algorithm for solving the single-table case of input size $n = \frac{\OUT}{\Delta}$ with $\ell_\infty$ error as $O\left(\sqrt{n}\right)$. 

Suppose we are given a single table $R$ of size $n$ over domain $\D$. We fix a parameter $\ell \ge \max\left\{\frac{\OUT}{\Delta}, \Delta^{1/m-1}\right\}$, whose value does not affect the proof below. We construct a star instance $\I = \{R_1, R_2, \cdots, R_m\}$ with input size $O(\ell)$, join size $\OUT$, and local sensitivity $\Delta$. We first construct $m$ domains $\{\D_1, \D_2, \cdots, \D_m\}$ such that $|\D_i| = 2|\D|$ and $\D \subseteq \D_1$. Then, we distinguish two more cases:
\begin{enumerate}
    \item[(1)] $\Delta \le \OUT \le \Delta^{m/m-1}$. All records in $\D_1$ have the same join value $b$. In addition, up to $\Delta^{1/m-1}$ records in $\D_i$ have the same join value $b$, which are included by $R_i$. The remaining records in $\D_1 - \D$ as well as $\D_i$ have distinct join values, different from $b$. It can be easily checked that the join size is $\OUT$ and local sensitivity is $\Delta$ since $n = \frac{\OUT}{\Delta} \le \Delta^{1/m-1}$. 
    \item[(2)] $\Delta^{m/m-1} \le \OUT$.  We divide records in $R$ into $\frac{\OUT}{\Delta^{m/m-1}}$ groups, each group consisting of $\Delta^{1/m-1}$ records and sharing the same join value. Similarly, each of them can be joined with $\Delta$ records in $R_i$ for $i \in [2,m]$. There are $n = \frac{\OUT}{\Delta}$ records falling into this construction, and the remaining $\ell-n$ records have distinct join values, different from $b$. It can be easily checked that the join size is $\OUT$ and local sensitivity is $\Delta$.
\end{enumerate} 

\xiao{\paragraph{Question: How large is the gap between $LS_\countsize(\I)$ and $SS_\countsize(\I)$ for star join?} For simplicity, we consider relation $R_i$ has attribute set $\x_i = \{A_i, B\}$ for $i \in [m]$. For each join value $b$, let $\Delta_i(b)$ be the sum of frequencies of tuples in $R_i$ with join value $b$.  We start with rewriting the boundary query $q_E(\I)$ for the star join:
\begin{align*}
    T_E(\I) &= \max_{b \in \dom(B)} |\Join_{j \in E} R_j \ltimes \{b\}| \\
    &= \max_{b \in \dom(B)} \big|\times_{j \in E} \left(R_j \ltimes \{b\}\right)\big| \\
    &= \max_{b \in \dom(B)} \prod_{j \in E} \big|\left(R_j \ltimes \{b\}\right)\big| \\
    & = \max_{b\in \dom(B)} \prod_{j \in E} \Delta_j(b)
\end{align*}
Putting $T_{[m]-\{i\}}(\I)$ into $LS_\countsize(\I)$, we have:
 \begin{align*}
     LS_\countsize(\I) =  \max_{i \in [m]} T_{[m]-\{i\}}(\I) = \max_{i \in [m]} \max_{b\in \dom(B)} \prod_{j \in [m]-\{i\}} \Delta_j(b) 
 \end{align*}
%Then, we define $\bfS^k$ as the set of difference vectors at distance $k$:
%\[\bfS^k = \left\{\s = (\s_1, \s_2, \cdots, \s_m): \sum_{i=1}^m \s_i = k, \s_i \in %\mathbb{Z}, \forall i \in [m]\right\}.\]
%Putting $T_{[m]-\{i\}-E'}(\I)$ into $\hat{LS}^{(k)}_\countsize(\I)$, we have:
%\begin{align*}
%    \hat{LS}^{(k)}_\countsize(\I)
%     = & \max_{\I': d(\I,\I') = k} \max_{i \in [m]} \sum_{E' \subseteq [n] -\{i\} }\left(T_{[m]-\{i\}-E'}(\I) \cdot \prod_{j \in E'} d_j(\I, \I')\right)  \\
%     = & \max_{\s \in \bfS^k} \max_{i \in [m]} \sum_{E' \subseteq [n] -\{i\} }\left(T_{[m]-\{i\}-E'}(\I) \cdot \prod_{j \in E'} \s_j\right) \\
%     \le & 2^n \cdot \max_{\s \in \bfS^k} \max_{i \in [m]} \max_{E' \subseteq [n] -\{i\} }\max_{b\in \dom(B)} \prod_{j \in [m]-\{i\}- E'} \Delta_j(b) \cdot \prod_{j \in E'} \s_j \\
%     =& 2^n \cdot \max_{b\in \dom(B)} \max_{\s \in \bfS^k} \max_{i \in [m]} \max_{E' \subseteq [n] -\{i\}} \prod_{j \in [m]-\{i\}- E'} \Delta_j(b) \cdot \prod_{j \in E'} \s_j
% \end{align*}
 Putting $T_{[m]-\{i\}-E'}(\I)$ into $\hat{LS}^{(k)}_\countsize(\I)$, we have:
 \begin{align*}
     RS_\countsize(\I) = \max_{E \subsetneq [n]} T_E(\I) = \max_{E \subsetneq [n]} \max_{b\in \dom(B)} \prod_{j \in E} \Delta_j(b)
 \end{align*}
 
 The gap could be as large as $\textsf{poly}(n)$ on the following instance $\I$: given $b_1$ such that $\Delta_i(b_1) = 1$ and $b_2$ such that $\Delta_1(b_2) = \Delta_2(b_2) = 0$ while  $\Delta_i(b_2) = n-1$ for every $i \ge 3$. In this case, we have $LS_\countsize(\I) = 1$ and $RS_\countsize(\I) = (n-1)^{(m-2)}$.
 }


\paragraph{Uniformization} The uniformization over star join is similar to the two-table case. Define $\degg_1$

Let $\widetilde{\Delta} =\Delta + G_{\epsilon, \delta, 1}$. We partition$(0,\widetilde{\Delta}]$ into $\ell= \lceil \log_2 \widetilde{\Delta} \rceil$ disjoint intervals, where the $i$-th interval is defined as $(2^{i-1}, 2^i]$ for $i \in [\ell]$. Then, the join values whose degree falls into the $i$-interval is denoted as $B_i$, i.e., \[B^{(i)} = \{b \in B: \max\{\deg_1(b), \deg_2(b)\} \in (2^{i-1}, 2^i]\}.\]
From each $j\in [\ell]$, we identify tuples in $R_1, R_2$ whose join value falls into $B^{(i)}$ as $R^{(i)}_1, R^{(i)}_2$ respectively. For each $i \in [\ell]$, we invoke Algorithm~\ref{alg:two-table} on $(R^{(i)}_1, R^{(i)}_2)$, and obtain the synthetic function $\F^{(i)}$. At last, we return $\F = \bigcup_{i \in [\ell]} \F^{(i)}$. 






==> intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

 Synthetic data release is a very useful objective in private data analysis. Differential privacy \cite{dwork2006calibrating,dwork2006our} has emerged as a compelling model that enables us to formally study the tradeoff between utility of released information and the privacy of individuals. In the literature, there has been a large body of work that studies synthetic data release over a single table, for example, the private multiplicative weight algorithm~\cite{hardt2012simple}, the histogram-based algorithm~\cite{vadhan2017complexity}, the matrix mechanism~\cite{li2010optimizing}, the Bayesian network algorithm\cite{zhang2017privbayes}; and some specialized works for geometric range queries~\cite{li2011efficient, li2012adaptive, dwork2010differential, bun2015differentially, chan2011private, dwork2015pure, cormode2012differentially, huang2021approximate}, and datacubes~\cite{ding2011differentially}. 

Data analysis over multiple private tables connected via join operators has been the subject of significant interest within the area of modern database systems. In particular, the challenging question of releasing the counting join size over a set of private tables has been studied in several recent works including the sensitivity-based framework~\cite{johnson2018towards, dong2021residual,dong2021nearly} and truncation-based mechanism~\cite{kotsogiannis2019privatesql, dong2022r2t, tao2020computing}; and some specialized works for one-to-one join~\cite{mcsherry2009privacy,proserpio2014calibrating}, and graph database~\cite{blocki2013differentially, chen2013recursive}. In practice, multiple queries instead of a single query are typically issued for data analysis, for example, a large class of linear queries on top of join results with different weights on input tuples, as a variant of counting join size query. One might consider answering each query independently but the utility would be very bad due to the limited privacy budget \badih{Do we want to somehow mention here that this would be applying DP composition?}. Hence, how can we release synthetic data for answering such a large class of linear queries over a set of multiple tables in a differentially private way? In this paper, we take the first step in answering this question with theoretical guarantees.

\badih{Do we need to cite previous work on DP SQL queries? Actually, looks like we already added two such citations: the Johnson et al. paper and the Privatesql paper.}

\subsection{Problem Definition}

 \paragraph{Multi-way Join and Linear Queries.} A (natural) join query can be represented as a hypergraph $\mathcal{H} = (\x, \{\x_1, \x_2, \cdots, \x_m\})$~\cite{abiteboul1995foundations}, where $\x$ is the set of vertices or attributes and each $\x_i \subseteq \x$ is a hyperedge or relation. Let $\dom(x)$ be the domain of attribute $x$. Define $\displaystyle{\D = \dom(\x) = \prod_{x \in \x} \dom(x)}$, and $\displaystyle{\D_i = \dom(\x_i) = \prod_{x \in \x_i} \dom(x)}$ for any $i \in [m]$. Given an input instance $\I = \left(R^\I_1, R^\I_2, \cdots, R^\I_m\right)$, each table $R^\I_i: \D_i \to \mathbb{Z}^+$ %\pasin{Is it standard for the range to be $0, 1$? Or do we people generally consider the range to be $\Z$ as well?} Resolved.
 is defined as a function from domain $\D_i$ to a non-negative integer, indicating the frequency of each tuple. This is more general than the setting that each tuple appears at most once in each relation, since it can capture annotated relations with non-negative values. The input size of $\I$ is defined as the sum of frequencies of data records, i.e., $\displaystyle{n = \sum_{i \in [m]} \sum_{t \in \D_i} R^\I_i(t)}$. When the context is clear, we just drop the script $\I$ from $R^\I_j$, and often use $R_j = \{t\in \D_j: R_j(t) >0\}$ to denote the set of tuples with non-zero frequency.\pasin{This notion $R_j$ is pretty confusing to me. Do we really need it?}
 
 For each $i \in [m]$, we have a family of linear queries $\Q_i$ defined over $\D_i$ such that for $q \in \Q_i$, $q: \D_i \to [-1,+1]$. The family of linear queries defined over $\I$ is $\Q  = \times_{i \in [m]}\Q_i$. For each linear query $q = (q_1, q_2, \cdots, q_m) \in \Q$, the result is defined as
 \[ q(\I) = \sum_{\vec{t}= (t_1, t_2, \cdots, t_m) \in \times_{i \in [m]}\D_i} \rho\left(\vec{t}\right) \prod_{i \in [m]} q_i(t_i) \cdot R_i(t_i) \]
 where $\rho: \times_{i \in [m]}\D_i \to \{0,1\}$ is the natural join function, such that for each combination $\vec{t} \in \times_{i \in [m]}\D_i$,  $\rho(\vec{t}) = 1$ if and only if $\pi_{\x_i \cap \x_j} t_i = \pi_{\x_i \cap \x_j} t_j$ for each pair of $i,j \in [m]$, where $\pi$ is the standard projection operator, such that $\pi_x t$ indicates the value(s) that tuple $t$ displays on attribute(s) $x$.
 
 Our target is to release a function $\F: \times_{i \in [m]}\D_i \to \mathbb{N}$ such that all queries in $\Q$ can be answered over $\F$ as accurately as possible, i.e., minimizing the $\ell_\infty$-error $\displaystyle{\alpha = \max_{q \in \Q} |q(\I) - q(\F)|}$, where  
 \begin{align*}
    q(\F) &= \sum_{(t_1, t_2, \cdots, t_m) \in \times_{i \in [m]}\D_i}  \F(t_1, t_2, \cdots, t_m) \prod_{i\in [m]} q_i(t_i). 
 \end{align*}
 % \pasin{I intentionally removed the following paragraph because it is far from clear that the error has to depend e.g. on $n(\I)$. For example, in the single-table case, the error when we take $n \to \infty$, depends only on the query set (and privacy parameters of course).}
 %We study the data complexity~\cite{vardi1982complexity} of this problem, i.e., assume that the query size, namely $m$, is a constant. Hence, the error only depends on the input-dependent quantities, such as input size $n(\I)$.
 
 \paragraph{DP Settings.} Two DP models \badih{Need to specify which of these two models we study in the paper? E.g., in Definition~\ref{def:neighboring} below?} have been studied in the relational model, depending on whether foreign key constraints are
 considered. One considering foreign key constrains assumes the existence of a single primary private table, and deleting a tuple in the primary private relations will delete all other tuples referencing to it; see~\cite{kotsogiannis2019privatesql, tao2020computing, dong2022r2t}. \xiao{We adopt the other one not considering foreign key constrains, which is the same as \cite{johnson2018towards, kifer2011no, narayan2012djoin, proserpio2014calibrating}, that defines the neighboring instances if they can be converted into each other by updating one tuple.} \badih{Cite some papers, in particuarl, some that don't consider foreign key constraints.} As all instances have the same input size, we simply assume that $n$ is public.
 
 \begin{definition}\label{def:neighboring}
     A pair of instances $\I = (R_1, \cdots, R_m)$ and $\I' = (R'_1, \cdots, R'_m)$ are {\em neighboring} if there exists some $i \in [m]$ such that:
    \begin{itemize}[leftmargin=*]
        \item for any $j \in [m] - \{i\}$, $R_j(t) = R'_j(t)$ for every $t \in \D_j$;
        \item there exists $t_1,t_2 \in \D_i$ such that $R_i(t) = R'_i(t)$ for every $t \in \D_i - \{t_1,t_2\}$ with $R_i(t_1) - R'_i(t_1) = 1$ and $R_i(t_2) - R'_i(t_2) = -1$.
    \end{itemize}
 \end{definition}

\begin{definition}[\cite{dwork2006calibrating,dwork2006our}]
    For $\epsilon,\delta>0$, $\mathcal{A}$ is $(\epsilon, \delta)$-differentially private if for any pair of neighboring instances $\I$, $\I'$ and any subset of outputs $\mathcal{S}$,
   $\Pr(\mathcal{A}(\I) \in \mathcal{S}) \le e^\epsilon \cdot \Pr(\mathcal{A}(\I') \in \mathcal{S}) + \delta$,
    which is also denoted by $\mathcal{A}(\I) \sim_{(\epsilon, \delta)} \mathcal{A}(\I')$.
\end{definition}

\subsection{Previous Results on Answering Multiple Queries over a Single Table}

We first review the problem of releasing synthetic data for a single table, and mention two important results in the literature. 
\begin{theorem}[\cite{hardt2012simple}]
\label{the:single-table}
    For a single table $R$ of $n$ records, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that preserves $(\epsilon, \delta)$-DP, and with probability at least $1- 1/\textsf{poly}(|Q|)$ produces $\F$ such that all queries in $\Q$ can be answered within error $\displaystyle{\alpha =O\left(n^{\frac{1}{2}} \cdot \left(\frac{1}{\epsilon} \cdot \log |\Q| \cdot \log \frac{1}{\delta} \cdot \log^{\frac{1}{2}} |\D|\right)^\frac{1}{2}\right)}$.
\end{theorem}

We next generalize it to the settings that neighboring instances have distances as $\Delta$ for $\Delta > 1$. The corollary below follows Theorem~\ref{the:single-table}, whose proof is deferred to Appendix~\ref{appendix:single-table}.

\begin{corollary}
\label{cor:single-table-sensitivity}
    For a single table $R$ of $n$ records with sensitivity $\Delta$, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that preserves $(\epsilon, \delta)$-DP, and with probability at least $1- 1/\textsf{poly}(|Q|)$ produces $\F$ such that all queries in $\Q$ can be answered within error $\displaystyle{\alpha =O\left(\left(n \cdot \Delta\right)^{\frac{1}{2}} \cdot \left(\frac{1}{\epsilon} \cdot \log |\Q| \cdot \log \frac{1}{\delta} \cdot \log^{\frac{1}{2}} |\D|\right)^\frac{1}{2}\right)}$.
\end{corollary}

We define $f(\mathbb{D}, \Q, \epsilon, \delta) = \left(\frac{1}{\epsilon} \cdot \log |\Q| \cdot \log \frac{1}{\delta} \cdot \log^{\frac{1}{2}} |\D|\right)^\frac{1}{2}$. In the remaining of this paper, we usually hide this factor within the notation\pasin{I'm not sure I understand this notion $O_f(\cdot)$. In the TCS convention, this would mean that we fix $f$ to be a constant but clearly this cannot be true because e.g. if we fix $f$ to be constant then $n$ is bounded and all the other terms are already $O_f(1)$. Maybe I'm not understanding the usage here correctly?} $O_f(\cdot)$, since both $\log |\Q|$ and $\log^{\frac{1}{2}} |\D|$ are enlarged by a factor of $m$, the number of tables, which is considered as a constant. 
%\badih{What's the smallest error that can be achieved for single-table synthetic data generation?} Resolved.

\begin{theorem}[\cite{bun2018fingerprinting}]
\label{the:lb-single-table}
    For every sufficiently small $\alpha>0$, $d \ge \log \frac{1}{\alpha}$, there exists a family of queries $\Q$ of size at least $\frac{d}{\alpha^2}$ such that any $(\epsilon, \delta)$-differentially private algorithm that takes as input a database $D \in (\{0,1\}^d)^n$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ requires that 
    $\displaystyle{n \ge \widetilde{\Omega}\left(\frac{\sqrt{d} \log |\Q|}{\epsilon \cdot (\frac{\alpha}{n})^2}\right)}$.\pasin{Note: this needs to be some sort of probabilistic statement?}
\end{theorem}

\subsection{Previous Results on Answering Single Counting Query over Multiple Tables}

Another related problem that has been widely studied by database community is how to release the answer of counting join size query under DP, denoted as $\countsize(\cdot)$:
\[\countsize(\I) =  \sum_{\vec{t} = (t_1, t_2, \cdots, t_m) \in \times_{i \in [m]}\D_i} \rho\left(\vec{t}\right) \prod_{i \in [m]} R_i(t_i),\]
which can be captured by a special linear query $q = (q_1, q_2, \cdots, q_m)$ such that $q_i: \D_i \to \{+1\}$ for $i \in [m]$. 

A popular approach is
the sensitivity framework, which computes $\countsize(\I)$, computes some notions of sensitivity of the query (measuring the difference between the query answers on
neighboring database instances), and then releases a noise-masked query answer, where the noise is
drawn from some %zero-mean 
distribution calibrated appropriately according to the sensitivity. Although this framework can be carried over to answering any single linear query, the computation of sensitivity becomes much more complicated, as a weighted version of $\countsize(\cdot)$. However, we are not interested in answering each linear query individually, since the privacy budget blows up with the number of queries to be answered, which would be too costly when the query space is very large. Our algorithm of releasing a synthetic dataset for answering multiple queries uses the existing results on sensitivity derived for $\countsize(\cdot)$. 
%
%
It is known that the local sensitivity $LS_\countsize(\cdot)$ cannot be directly used for calibrating noise, as $LS_\countsize(\I), LS_\countsize(\I')$ for a pair of neighboring databases can lead to distinguishability of $\I,\I'$ \badih{Not sure if we want to add a citation for this fact?}. Global sensitivity~\cite{} could be used, but the utility is not ideal in many instances. Instead, people have considered smooth upper bounds on local sensitivity~\cite{nissim2007smooth}, for example the {\em smooth sensitivity}, which is the smallest smooth upper bound, and the {\em residual sensitivity}~\cite{dong2021residual}, which is a constant-approximation of smooth sensitivity.
%
Although smooth sensitivity enjoys the best utility, we adopt residual sensitivity in this paper for two reasons: it is much more computationally efficient than smooth sensitivity; and more importantly, it is only built on the statistics of input databases itself while smooth sensitivity built on its all neighboring instances, which is critical in building our optimization algorithm in Section~\ref{sec:hierarchical}. 

\subsection{Our Results}

\badih{Based on discussion with Xiao, we might need to add more interpretation of the results in this section?}

We first present the basic join-as-one approach for releasing a synthetic dataset for multi-table queries, with error a function of the output size of join results and the residual sensitivity. Let $\lambda = \frac{1}{\epsilon} \log \frac{1}{\delta}$, which is a commonly-used parameter in this paper.

\begin{theorem}
\label{the:ub-multi-table}
     For any join query $\mathcal{H}$, an instance $\I$, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that preserves $(\epsilon, \delta)$-DP, and with probability at least $1- \frac{1}{\textsf{poly}(|\Q|)}$ produces $\F$ that all queries in $\Q$ can be answered within error:
    \[\alpha = O_f\left(\sqrt{\OUT} \cdot \sqrt{SS^\beta_\countsize(\I) \cdot \lambda} + SS^\beta_\countsize(\I) \cdot \lambda \right) \]
    where $\OUT$ is the join size of $\I$ and $SS^\beta_\countsize(\I)$ is the $\beta$-residual sensitivity of counting join size $\countsize(\cdot)$ on $\I$ for $\beta = \frac{\epsilon}{2\ln 2/\delta}$.
\end{theorem}

We next show the parameterized optimality with respect to the output size and local sensitivity. It should be noted that taking the choice of  $\epsilon = O(1)$ and $\delta = O\left(\frac{1}{n^c}\right)$ for some constant $c$, we have $\lambda = O\left(\log^c n\right)$ for some query-dependent constant $c$.  The gap between the upper bound in Theorem~\ref{the:ub-multi-table} and the lower bound in Theorem~\ref{the:lb-multi-table} boils down to the inherent gap between local sensitivity and smooth sensitivity, which also exists in answering the single counting join size query. Moreover, this gap is \badih{tight?} up to logarithmic factors \badih{factors?} on the simplest two-table join query.

\begin{theorem}
\label{the:lb-multi-table}
     For any join query $\mathcal{H}$, for any parameters $\OUT >0$ and $\Delta > 0$ for $\OUT \ge \Delta$, let $\mathbb{I}(\OUT,\Delta)$ be the class of instances over $\mathcal{H}$ that have join size $\OUT$ and local sensitivity $\Delta$. There exists a set of queries $\Q$ such that any $(\epsilon,
     \delta)$-DP algorithm that takes as input an instance $\I \in \mathbb{I}(\OUT,\Delta)$ and outputs an approximate answer to each query in $\Q$ within error $\alpha$ must require $\displaystyle{\alpha \ge \Omega\left(\sqrt{\OUT} \cdot \sqrt{\Delta} + \Delta\right)}$, with probability at least $\exp(-\epsilon) \cdot (1-\delta)$. \badih{In this theorem, $\delta$ is being used to denote both the DP parameter and the failure probability?}\xiao{the probability is inherited from Theorem~\ref{the:lb-two-table-1}.}
\end{theorem}

\pasin{Our upper bound above is in terms of smooth sensitivity but lower bound is in terms of local sensitivity. Do we need to state a connection between the two?}
From the error complexity in terms of residual sensitivity, we exploit the technique of {\em uniformizing degrees}\footnote{\xiao{Similar idea have been used in query processing~\cite{joglekar2015s}, but we use it in a more complicated scenario.}} \badih{Per discussion with Xiao, since the previous work used ``uniformization'' to refer to a much simpler technique, we might want to consider using a different term to avoid confusion?} to further improve Theorem~\ref{the:ub-multi-table} and Theorem~\ref{the:lb-multi-table}. For the class of hierarchical queries, which has been widely studied in various contexts of database problems~\cite{dalvi2007efficient, fink2016dichotomies, berkholz2017answering, hu2022temporal}\badih{Should we add a citation to indicate that this class of queries is well-studied in database theory research?}, we obtain a more fine-grained parameterized upper and lower bound in Theorem~\ref{the:ub-hierarhical-uniformize} and Theorem~\ref{the:lb-hierarhical-uniformize}, which are deferred to Section~\ref{sec:uniformization}. 




==> multi-table-backup.tex <==
\subsection{Multi-table Query}

We next extend the join-as-one approach to multi-table query. The general framework shares the common spirit as Algorithm~\ref{alg:two-table}, but involves a non-trivial usage of residual sensitivity. Before diving into the algorithm, we formally define the residual sensitivity. For a join query $\mathcal{H} = (\x, \{\x_1,\x_2,\cdots,\x_m\})$, the residual query on a subset $E \subseteq [m]$ of relations is $H_E = \Join_{i\in E} R_i$. Its boundary, denoted as $\partial_{E}$, is the set of attributes that belong to relations both in and out of $E$, i.e.,
$\partial E = \{x|x \in \textbf{x}_i \cap \textbf{x}_j, i \in E, j \notin E\}$. For a residual query $H_E$ on instance $\I$, the query result is\footnote{The semi-join result of $R \ltimes t$ is defined as $\left\{t' \in R: R(t')>0, \pi_{\x_i} t' = \pi_{\x_i} t\right\}$.}:
\begin{equation}
\label{eq:TE}
    T_E(\I) = \max_{t \in \dom(\partial E)} |H_E(\I) \ltimes t|
\end{equation}
 which is a join-aggregate queries over attributes in $\partial E$. Now, we can use residual query to define the residual sensitivity.
 
 \begin{definition}[Residual Sensitivity for Counting Query~\cite{dong2021residual, dong2021nearly}] Given $\beta > 0$, the $\beta$-residual sensitivity of counting the output size of multi-way join $\mathcal{H}$ over instance $\I$ is defined as $SS^\beta_\countsize(\I) = \max_{k\ge 0} e^{-\beta k} \min\left\{\hat{LS}^{(k)}_\countsize(\I), GS_\countsize\right\}$, where
    \begin{equation}
    \label{eq:residual}
        \hat{LS}^{(k)}_\countsize(\I) =  \max_{\s \in \mathcal{S}^k} \max_{i \in [m]} \sum_{E' \subseteq [m] -\{i\} }T_{[m]-\{i\}-E'}(\I) \cdot \prod_{j \in E'} \s_j 
     \end{equation}
     \begin{equation*}
         GS_\countsize = \max_{i \in [m]} n^{\rho(\x-\x_i, \{\x_1 -\x_i, \x_2 - \x_i, \cdots, \x_m -\x_i\})} \quad \quad \quad \quad 
     \end{equation*}
    for $\mathcal{S}^k = \left\{\s = (\s_1, \s_2, \cdots, \s_m): \sum_{i=1}^m \s_i = k, \s_i \in \mathbb{Z}, \forall i \in [m]\right\}$, and $\rho(\cdot)$ is the optimal fractional edge covering number\footnote{For a hypergraph $(\x, \{\x_1,\x_2,\cdots,\x_m\})$, a fractional edge covering is a length-$m$ vector $\Vec{x}$ such that $\Vec{x}_i \ge 0$ and $\sum_{i: x \in \x_i} \Vec{x}_i \ge 1$. The number of $\Vec{x}$ is defined as $\sum_{i\in[m]} \Vec{x}_i$. }.
 \end{definition}


Now, we are ready to present our general algorithm using residual sensitivity. As described in Algorithm~\ref{alg:multi-table}, we first compute the join results over $\I$ as $J$, and the $\beta$-residual sensitivity of $\countsize(\cdot)$ over $\I$ as $SS^\beta_\countsize(\I)$. After obtaining $SS^\beta_\countsize(\I)$, adding noise to $|J|$ to
achieve DP is straightforward, for example, the Laplacian or Cauchy mechanism~\cite{nissim2007smooth}.  However, we might end up with a negative value, leading to a invalid initial distribution for single-table algorithm (line 4-5). 
%\pasin{I'm not sure why we're using SS and not LS here. Can you please explain more? Is this because LS can now have large sensitivity?} 
To guarantee the correctness, we derive a strict upper bound on $SS^\beta_\countsize(\I)$, denote as $\widetilde{\Delta}$, which also satisfies $(\epsilon, \delta)$-DP. We use this noisy random variable $\widetilde{\Delta}$ to calibrate the truncated and shifted geometric distribution, draw a random variable from $\textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}$, and add it to the true join size as $\widehat{n}$. Finally, we invoke the single-table algorithm to $J$, with initial distribution parameterized by $\widehat{n}$. This upper bound of $SS^\beta_\countsize(\I)$ is also used in parameterizing the exponential mechanism (line 7), and masking the query answer (line 8). 

\begin{algorithm}[t]
\caption{{\sc JoinMultiTable}$(\I = \{R_1,R_2, \cdots, R_m\})$}
\label{alg:multi-table}

$J = \Join_{i \in [m]} R_i$\;
$\beta \gets \frac{\epsilon}{2\ln 2/\delta}$\;
$\widetilde{\Delta} \gets  \max \left \{SS^\beta_\countsize(\I),  SS^\beta_\countsize(\I) \cdot e^{\frac{\beta}{\epsilon} \cdot \textsf{Lap}_1(x) + \frac{1}{2}} \right\}$\;
$\widehat{n} = |J| + \textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}(x)$\; 
$\F_0 \gets \widehat{n}$ times uniform distribution over $\D$: $\F_0(x) = \frac{\widehat{n}}{|\D|}$\;
\ForEach{$i = 1, 2, \cdots, T$}{
    Sample a query $q_i \in \Q$ using the EM parameterized with $\frac{\epsilon}{2T \cdot \widetilde{\Delta}}$ and score function $s_i(J,q) = |q(\F_{i-1}) - q(J)|$\;
    $m_i \gets q_i(J) + \textsf{STGeom}_{\frac{\epsilon}{2T}, \delta, \widetilde{\Delta}}(x)$\;
    Update for each $x \in \D$: $\F_i(x) \propto \F_{i-1}(x) \times \exp\left(q_i(x) \cdot \left(m_i - q_i(\F_{i-1})\right) \cdot \frac{1}{2 \widehat{n}}\right)$\;
}
\Return $\textsf{Avg} \left(\sum_{i=1}^T \F_i\right)$\;
\end{algorithm}

\begin{lemma}
\label{lem:multi-table-DP}
    Algorithm~\ref{alg:multi-table} preserves $(4\epsilon, 4 \delta)$-DP.
\end{lemma}

%The proof of Lemma~\ref{lem:multi-table-DP} is given in Appendix~\ref{appendix:join-as-one}.

\paragraph{Error analysis} With probability at least $1 - \delta$, $\widetilde{\Delta} = O\left(SS_\countsize(\I)\right)$, and therefore $\widehat{n} = O\left(|J| + SS_\countsize(\I)\cdot \lambda \right)$. Putting everything together, the error that can be achieved is (omitting $\fup$): 
\[O\left(\sqrt{\widehat{n}} \cdot \sqrt{\widetilde{\Delta}} \right) = O\left(\sqrt{|J| \cdot SS_\countsize(\I) \cdot \lambda} + SS_\countsize(\I) \cdot \lambda \right)\]

The upper bound is given in Theorem~\ref{the:ub-multi-table}. Moreover, extending the previous lower bound argument on the two-table query, we can obtain the lower bound on the multi-table query in Theorem~\ref{the:lb-multi-table}. 



==> pasin-scratch.tex <==
\section{Pasin's Scratch Pad}

\subsection{Add-Remove DP}

\pasin{This is not a strong suggestion but I think it is a little bit more convenient to use the add-remove DP which anyway also implies substitution DP.}

It will be more convenient to work with the \emph{add-remove} notion of differential privacy, as defined below.

 \begin{definition}\label{def:neighboring-addremove}
     A pair of instances $\I = (R_1, \cdots, R_m)$ and $\I' = (R'_1, \cdots, R'_m)$ are {\em neighboring} if there exists some $i \in [m]$ such that:
    \begin{itemize}[leftmargin=*]
        \item for any $j \in [m] - \{i\}$, $R_j(t) = R'_j(t)$ for every $t \in \D_j$;
        \item there exists $t^* \in \D_i$ such that $R_i(t) = R'_i(t)$ for every $t \in \D_i - \{t^*\}$ with $|R_i(t^*) - R'_i(t^*)| = 1$.
    \end{itemize}
 \end{definition}

We note that the above notion corresponds to the so-called \emph{add-remove} DP where a record is added / removed from a single database $R_i$. Another possible definition is the \emph{substitution} DP; we remark that add-remove DP implies substitution DP with only a factor of two increase in the privacy parameters; therefore, all of our results here also apply to the substitution DP setting.


\subsection{Additional Preliminaries}

\pasin{We probably need the following in our prelims.}

\paragraph{Exponential Mechanism.}
The exponential mechanism (EM)~\cite{McSherryT07} can select a ``good'' candidate from a set $\cC$ of candidates. The goodness here is defined by a scoring function $s(\I, c)$ for input dataset $\I$ and a candidate $c \in \cC$ which should have sensitivity at most one. Then, the EM algorithm is to sample each candidate $c \in \cC$ with probability proportional to $\exp\left(-0.5\eps \cdot s(\I, c)\right)$. When the scoring function has sensitivity at most one, this algorithm is $\eps$-DP.

\subsection{Private Multiplicative Weight Algorithm}

\pasin{The following is my suggestion on how to rephrase the multiplicative weight algorithm. I think it is not a very good idea to repeat this part several times in different algorithm with unclear guarantee. Having something like the following should allow us to avoid repetition and be clear about what exactly we need.}

For an instance $\I = (R_1, \cdots, R_m)$, we write $\joindat{\I}$ as a shorthand for $R_1 \Join \cdots \Join R_m$. Furthermore, for two sets $S, T$, we write $S \setdiff T$ as a shorthand for the symmetric set difference between $S$ and $T$, i.e. $(S \setminus T) \cup (T \setminus S)$. 

%For $k \in \N$, we say that $\I$ and $\I'$ are $k$-neighbors, denoted by $\I\sim_t \I'$, iff there is a sequence $\I_0 = \I, \dots, \I_k = \I'$ such that $\I_{i - 1}, \I_i$ are neighbors for all $i \in [k]$.

A central parameter for our investigation is the (symmetric set) difference between the Join of $\I$ and that of its neighbor $\I'$, i.e. $(\joindat{\I}) \setdiff (\joindat{\I'})$. Its importance stems from the fact that this quantity upper bounds the local sensitivity of any linear queries:

\begin{observation}
For any linear query $q$, we have $|q(\I) - q(\I')| \leq |(\joindat{\I}) \setdiff (\joindat{\I'})|$. Consequently, $\LS_q(\I) \leq \max_{\I' \sim \I} |(\joindat{\I}) \setdiff (\joindat{\I'})|$.
\end{observation}

\pasin{One advantage of removal notion is that $\max_{\I' \sim \I} |(\joindat{\I}) \setdiff (\joindat{\I'})|$ exactly coincides with the LS of $\countsize$ at $\I$.}

A priori, the quantity $\max_{\I' \sim \I} |(\joindat{\I}) \setdiff (\joindat{\I'})|$ can be arbritrarily large. However, as we will see below, we can often estimate it well. Indeed, if we have an upper bound $\tDelta$ on this quantity, then the private multiplicative weight (PMW) algorithm of~\cite{hardt2012simple} from the single table setting can be easily applied to our setting. The algorithm is described in \Cref{alg:pmw} and its guarantees (which follows almost directly from \cite{hardt2012simple}) are stated in \Cref{thm:pmw}.

%Here it takes an additional parameter $\tDelta$ which represents an ``upper bound on the local sensitivity''. 

\begin{algorithm}[t]
\caption{{\sc PMW}$_{\eps, \delta, \tDelta}(\I = \{R_1,R_2, \cdots, R_m\})$}
\label{alg:pmw}
$\widehat{n} = \max\{1, |\joindat{J}| + \textsf{Geom}_{\exp(0.5\epsilon/\tDelta)}(x)\}$\; 
$\F_0 \gets \widehat{n}$ times uniform distribution over $\D$: $\F_0(x) = \frac{\widehat{n}}{|\D|}$\;
$\eps' \leftarrow \frac{\eps}{16 \sqrt{T \cdot \log(1/\delta)}}$\;
\ForEach{$i = 1, 2, \cdots, T$}{
    Sample a query $q_i \in \Q$ using the $\eps'$-DP EM with score function $s_i(\I,q) = \frac{1}{\tDelta}|q(\F_{i-1}) - q(\I)|$\;
    $m_i \gets q_i(\I) + \textsf{Geom}_{\eps', \tDelta}(x)$\;
    Update for each $x \in \D$: $\F_i(x) \propto \F_{i-1}(x) \times \exp\left(q_i(x) \cdot \left(m_i - q_i(\F_{i-1})\right) \cdot \frac{1}{2 \widehat{n}}\right)$\;
}
\Return $\textsf{Avg} \left(\sum_{i=1}^T \F_i\right)$\;
\end{algorithm}


\begin{theorem} \label{thm:pmw}
Let $\I, \I'$ be such that $|(\joindat{\I}) \setdiff (\joindat{\I'})| \leq \tDelta$. Then, \Cref{alg:pmw} satisfies the following:
\begin{itemize}[leftmargin=*]
\item (Privacy) $\PMW(\I) \sim_{(\eps, \delta)} \PMW(\I')$.
\item (Utility) With probability at least $1 - 1/\poly(|\Q|)$, $\PMW(\I)$ produces a dataset such that all queries in $\Q$ can be answered to within error $\displaystyle{\alpha =O\left(\left(n \cdot \tDelta\right)^{\frac{1}{2}} \cdot \fup\right)}$.
\end{itemize}
\end{theorem}





==> three-table.tex <==


%Note that $2^{i+j}$
%We consider an instance $\I$ for this join query (see Figure~\ref{fig:line-3}). Let $\dom(B) = \{b_1,b_2,\cdots, b_{\sqrt{n}}\}$ and $\dom(C) = \{c_1,c_2,\cdots, c_{\sqrt{n}}\}$. For any $i \in [\sqrt{n}]$, every value $b_i \in \dom(B)$ forms a tuple with $c_j$ for each $j \in \{\sqrt{n}-i+1,\sqrt{n}-i+2, \cdots, \sqrt{n}\}$. On this instance, $T_E$ can be simplified as:
%$\displaystyle{\max\left\{\max_{b \in \dom(B)} \degg_2(B,b), \max_{c \in \dom(C)} \degg_2(C,c)\right\}}$. Uniformizing $\I$ boils down to finding a partition $(R^1_2, R^2_2, \cdots, R^k_2)$ of $R_2$, to minimize the error achieved by Algorithm~\ref{alg:uniformization-framework}. Note that  Algorithm~\ref{alg:multi-table} can achieve an error of $O\left(n^{3/4}\right)$ on this instance. As proved in Appendix~\ref{appendix:uniformization}, every possible partition leads to an error at least $\Omega(n^{3/4})$, thus establishing a gap of uniformization on hierarchical and non-hierarchical join queries.

\newpage


==> two-table-backup.tex <==
\subsection{Upper Bound on Two-Table Query}
We start with the simplest two-table case. For simplicity, assume $\mathcal{H}$ has $\x = \{A,B,C\}$, $\x_1 = \{A,B\}$ and $\x_2 = \{B,C\}$. Let's define some parameters first. For $i \in [2]$, the degree of join value $b \in \dom(B)$ %\pasin{What is $B$? Is this the set of all attributes?}in $R_i$ is denoted as $\degg_i(B,b)$, the frequencies of data records displaying join value $b$ in $R_i$, i.e., resolved
$\displaystyle{\degg_i(B, b) = \sum_{t \in \D_i:\pi_B t=b} R_i(t)}$. The maximum degree of any join value in $R_i$ is denoted as 
$\displaystyle{\Delta_i = \max_{b \in \dom(B)} \degg_i(B, b)}$. Define $\Delta = \max\{\Delta_1, \Delta_2\}$.
We note that $LS_\countsize(\I) = \Delta$. \badih{Has $LS_\countsize(\I)$ been defined anywhere? Also, is the last sentence a fact or a definition?}


\paragraph{Shifted and truncated geometric distribution~\cite{chan2019foundations}.} Let $\textsf{Geom}_\alpha(x) \\= \frac{\alpha-1}{\alpha+1} \cdot \alpha^{-|x|}$. Let $\epsilon > 0$, $\delta \in (0, 1)$ and $\Delta \ge 1$.
Let $n_0$ be the smallest positive integer such that $\displaystyle{\Pr\left[\left|\textsf{Geom}_{\exp(\frac{\epsilon}{\Delta})}(x) \right| \ge n_0\right] \le \delta}$,
where $n_0 \leq \frac{\Delta}{\epsilon} \log \frac{2}{\delta} + 1$. The shifted and truncated geometric distribution $\textsf{STGeom}_{\epsilon, \delta, \Delta}(x)$ has support in $[0, 2\cdot(n_0 + \Delta-1)]$, and is defined as 
$\displaystyle{\min\left\{\max \left\{0, n_0 + \Delta - 1 + \textsf{Geom}_{\exp(\frac{\epsilon}{\Delta})}(x)\right\}, 2(n_0 + \Delta - 1)\right\}}$. It has been proved~\cite{balcer2017differential, chan2019foundations} \badih{Need to add some citation here.} that for any pair of $u,v$ with $|u -v| \le \Delta$,
\[u + \textsf{STGeom}_{\epsilon, \delta, \Delta}(x) \sim_{(\epsilon, \delta)} v + \textsf{STGeom}_{\epsilon, \delta, \Delta}(x).\]

\paragraph{Join result as a function.} As each input relation is a function, we introduce the natural join result function $J = \Join_{i \in [m]} R_i$, such that $J\left(\vec{t}\right) = \prod_{i \in [m]} R_i\left(\pi_{\x_i} \vec{t}\right)$ for any $\vec{t} \in \D$. Moreover, $|J| = \sum_{\vec{t} \in \D} J\left(\vec{t}\right)$.

\paragraph{A Strawperson Idea.} Let us first consider a flawed strawperson, which turns out to violate DP:
\begin{itemize}[leftmargin=*]
    \item Compute $J = \Join_{i\in[m]} R_i$ \badih{Need to formally define the $\Join$ notation somewhere?} and then release a synthetic dataset for $J$ as $\widetilde{J}_1$ using a single-table algorithm. However, this is not enough since the single-table algorithm releases exactly $|J| = \countsize(\I)$ records, which will reveal the information of input database. 
    \item We then draw a random noise from $\textsf{STGeom}_{\epsilon, \delta, 1}(x)$ and add it to $\Delta$ as $\widetilde{\Delta}$. Then, we draw a random noise from $\textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}(x)$ as $\lambda$, and choose $\lambda$ records randomly from $\mathbb{D}_1 \times \mathbb{D}_2$ denoted as $\widetilde{J_2}$. %\badih{This should be $\widetilde{J}_2?$} resolved
    \item At last, we release the union of these two datasets $\F = \widetilde{J}_1 \cup \widetilde{J}_2$.
\end{itemize}
The challenge is that invoking the single-table algorithm on $J$ does not satisfy DP, as the initial uniform data distribution parameterized by $|J|$ can lead to the leakage of input database. 


\begin{algorithm}[t]
\caption{{\sc JoinTwoTable}$(\I = \{R_1, R_2\})$}
\label{alg:two-table}

$J = R_1 \Join R_2$\;
$\Delta \gets LS_\countsize(\I)$\;
$\widetilde{\Delta} \gets \Delta + \textsf{STGeom}_{\epsilon, \delta, 1}(x)$\;
$\widehat{n} = |J| + \textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}(x)$\; 
$\F_0 \gets \widehat{n}$ times uniform distribution over $\D$: $\F_0(x) = \frac{\widehat{n}}{|\D|}$\;

\ForEach{$i = 1, 2, \cdots, T$}{
    Sample a query $q_i \in \Q$ using the EM parameterized with $\frac{\epsilon}{2T\cdot \widetilde{\Delta}}$ and score function $s_i(J,q) = |q(\F_{i-1}) - q(J)|$\;
    $m_i \gets q_i(J) + \textsf{STGeom}_{\frac{\epsilon}{2T}, \delta, \widetilde{\Delta}}(x)$\;
    Update for each $x \in \D$: $\F_i(x) \propto \F_{i-1}(x) \times \exp\left(q_i(x) \cdot \left(m_i - q_i(\F_{i-1})\right) \cdot \frac{1}{2\widehat{n}}\right)$\;
}
\Return $\textsf{Avg} \left(\sum_{i=1}^T \F_i\right)$\;
\end{algorithm}

\paragraph{Modified Algorithm.} As shown in Algorithm~\ref{alg:two-table}, we need to change the order of two steps in the strawperson version. After computing function $J$, we add $\textsf{STGeom}_{\epsilon, \delta, \widetilde{\Delta}}(x)$ random noise to $|J|$ as $\widehat{n}$, and then invoke the single-table algorithm on $J$ starting with a uniform distribution parameterized by $\widehat{n}$. As $\widehat{n}$ is released under DP, and the single-table algorithm~\cite{hardt2012simple} also releases a synthetic dataset for $J$ under DP, Algorithm~\ref{alg:two-table} also satisfies DP, as stated in Lemma~\ref{lem:two-table-DP}.

\begin{lemma}
\label{lem:two-table-DP}
    Algorithm~\ref{alg:two-table} preserves $(3\epsilon, 3\delta)$-DP.
\end{lemma}


\paragraph{Error Analysis.} As shown in Appendix~\ref{appendix:single-table}, with probability at least $1 - \frac{1}{\textsf{poly}(\Q)}$, Algorithm~\ref{alg:two-table} produces $\F = \textsf{Avg} \sum_{i=1}^T \F_i$ such that every linear query can be answered within error:
\[\alpha = O_f\left(\sqrt{|J|} \cdot \sqrt{\Delta + \lambda} + \Delta + \lambda \right).\]

\begin{theorem}
\label{the:up-2table}
     For any two-tables instance $\I$, a family of linear queries $\Q$, and $\epsilon > 0$, $\delta > 0$, there exists an algorithm that preserves $(\epsilon, \delta)$-DP, and with probability at least $1- \frac{1}{\textsf{poly}(|\Q|)}$ produces $\F$ on which all queries in $\Q$ can be answered within error:
    \[\alpha = O_f\left(\sqrt{|J|} \cdot \sqrt{LS_\countsize(\I) + \lambda} + LS_\countsize(\I) + \lambda \right).\]
\end{theorem}



==> two-table-lb-backup.tex <==
\subsection{Lower Bound on Two-Table Query}

%\begin{lemma}[Helper Lemma]
%\label{lem:max}
%    \rev{For any two-table instance $\I$, any algorithm for answering the counting query over $\I$ within error $\alpha$, must have
%    $\big||J| - \countsize(\I)\big| \le \alpha$,
%    where $|J|$ is the join size of $\I$.}
%%\end{lemma}

%\pasin{By selecting queries here, the lemma only holds for some set of queries. Would be good to specified this in the lemma statement itself.} 


\new{
\begin{theorem}
\label{the:lb-two-table-1}
     %\pasin{This should be ``some''? As Badih mentioned the other day, for a particular $\I$, there is a DP algorithm which just outputs the answer for $\I$ always. In the proof here, we do need the algorithm to be accurate on $\I'$ as well. Maybe we need some sort of neighborhood optimality/utility here?} 
     Any $(\epsilon, \delta)$-DP algorithm that takes as input any two-table instance $\I$ and outputs an approximate answer to the counting query within error $\alpha$, requires that
     $\displaystyle{\alpha \ge \Omega \left(LS_\countsize(\I)\right)}$, with probability at least $\exp(-\epsilon) \cdot (1-\delta)$. \badih{The order of quantifiers here is unclear. Did we mean to say that there is an input under which the algorithm will have large error with high probability?}
\end{theorem}
}

\begin{proof}
    Consider an $(\epsilon, \delta)$-DP algorithm $\mathcal{A}$, and a pair of neighboring instances $\I,\I'$. Let $\countsize(\I), \countsize(\I')$ be the join size of $\I, \I'$ respectively. 
    Let $\widetilde{\countsize}(\I), \widetilde{\countsize}(\I')$ be the results released for $\I, \I'$ respectively. From the error guarantee, $\big|\countsize(\I) - \widetilde{\countsize}(\I)\big| \le \alpha$ and $\big|\countsize(\I') - \widetilde{\countsize}(\I')\big| \le \alpha$.
    As $\mathcal{A}$ preserves $(\epsilon, \delta)$-DP, there must be
    \begin{align*}
        1 &= \Pr\left(\widetilde{\countsize}(\I) \in [\countsize(\I)-\alpha, \countsize(\I) + \alpha] \right) \\
        &\le e^\epsilon \cdot \Pr\left(\widetilde{\countsize}(\I') \in [\countsize(\I)-\alpha, \countsize(\I) + \alpha]\right) + \delta 
    \end{align*}
    i.e., $\Pr\left(\widetilde{\countsize}(\I') \in [\countsize(\I)-\alpha, \countsize(\I) + \alpha]\right) \ge e^{-\epsilon}(1-\delta)$. Moreover, $\big|\countsize(\I') - \countsize(\I)\big| \le 2 LS_\countsize(\I)$. If $\alpha < LS_\countsize(\I)$, we observe that $\countsize(\I') + \alpha < \countsize(\I) - \alpha$, or $\countsize(\I') - \alpha > \countsize(\I) + \alpha$, i.e., $\widetilde{\countsize}(\I') \notin [\countsize(\I)-\alpha, \countsize(\I) + \alpha]$. Thus $\alpha > \Omega(LS_\countsize(\I))$ holds with probability at least $\exp(-\epsilon) \cdot (1-\delta)$.
\end{proof}

We note that this theorem can be extended to general joins. 

\begin{theorem}
\label{the:lb-two-table-2}
    Given arbitrary parameters $\OUT>0$ and $\Delta > 0$ for $\Delta \le \OUT$, let $\mathbb{I}(\OUT, \Delta)$ be the class of instances that have join size $\OUT$ and local sensitivity $\Delta$. There exists a family of queries $\Q$ such that any $(\epsilon, \delta)$-DP algorithm that takes as input a database $\I \in \mathbb{I}(\OUT, \Delta)$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ requires that
    \[\alpha \ge \Omega\left(\sqrt{|\OUT|} \cdot \sqrt{\Delta} \cdot (\frac{\log^{1/2} \D \cdot \log |\Q|}{\epsilon})^{1/2}\right).\]
\end{theorem}

\begin{proof}
Set $n= \frac{\OUT}{\Delta}$ and $\D = (\{0,1\}^d)^n$. From Theorem~\ref{the:lb-single-table}, let $\Q_\textsf{one}$ be the set of queries on which any $(\epsilon, \delta)$-DP algorithm that takes as input a single-table database $T \in \D$ and outputs an approximate answer to each query in $\Q_\textsf{one}$ within error $\alpha$ requires that $\alpha \ge \widetilde{\Omega}\left(\sqrt{n} \cdot (\frac{\sqrt{d} \log |\Q_\textsf{one}|}{\epsilon})^{\frac{1}{2}}\right)$. %\pasin{Add citation \& make this more formal?}
For an arbitrary single-table database $T \in \D$, we construct
a two-table instance $\I$ of input size $m$, join size $\OUT$, and local sensitivity $\Delta$ as follows\footnote{Actually, we can construct a two-table instance of input size $m$ for any $m \ge \frac{\OUT}{\Delta}$, which is the minimum requirement under the join size and local sensitivity constraint. For $m > \frac{\OUT}{\Delta}$, we can simply pad $m- \frac{\OUT}{\Delta}$ dummy tuples to $R_1, R_2$ arbitrary, as long as which do not contribute to any join result.}.
\begin{itemize}[leftmargin=*]
    \item Set $\dom(A) = \D$, $\dom(B) = \mathbb{Z}$ and $\dom(C) = \mathbb{Z}$;
    \item Set $\D_1 = \dom(A) \times \dom(B)$ and $\D_2 = \dom(B) \times \dom(C)$;
    \item Tuples in $R_1$ form a Cartesian product of size $\min\left\{\Delta, \frac{\OUT}{\Delta}\right\} \times \max\left\{1, \frac{\OUT}{\Delta^2}\right\}$ over $\dom(A) \times \dom(B)$;
    \item Tuples in $R_2$ form a Cartesian product of sizes $\max\left\{1, \frac{\OUT}{\Delta^2}\right\} \times \min\left\{\Delta, \frac{\OUT}{\Delta}\right\}$ over $\dom(B) \times \dom(C)$;
    \item For each of the $n$ records in $T$, say $x$, we exclusively choose one tuple $t \in R_1$ and set $\pi_A t = x$. %\pasin{We might have to be a bit more careful about this b/c we have to make sure that the ``chosen'' tuples do not cause ``cascading effect'' and blow up the distance in the new instance.}
\end{itemize}
It can be easily checked that $\I \in \mathbb{I}(\OUT,\Delta)$. 
From $\Q_\textsf{one}$, we construct a set of queries over $\I$ as $\Q_\textsf{two}$. For each query $q \in \Q_\textsf{one}$, we construct another query $q'=(q_1,q_2)$ as follows:
\begin{itemize}[leftmargin=*]
    \item $q_1: \D_1 \to [0,1]$ such that $q_1(t) = q(x)$ if and only if $\pi_A t =x$;
    \item $q_2: \D_2 \to \{+1\}$ over $\D_2$.
\end{itemize}
We also add the counting query $q' = (q_1,q_2)$ with $q_1: \D_1 \to \{+1\}$ and $q_2: \D_2 \to \{+1\}$ to $\Q_\textsf{two}$. An example is illustrated in Figure~\ref{fig:lb-two-table}. 


Our lower bound argument is that if there is an $(\epsilon, \delta)$-DP algorithm that takes any two-table instance in $\mathbb{I}(\OUT, \Delta)$ and outputs an approximate answer to each query in $\Q_\textsf{two}$ within error $\alpha$, then there is a $(\epsilon, \delta)$-DP algorithm that takes any single-table instance $T \in \D$ and outputs an approximate answer to each query in $\Q_\textsf{one}$ within error $\frac{\alpha}{\Delta}$. Let $\mathcal{A}$ be such an arbitrary algorithm that takes any two-table instance in $\mathbb{I}(\OUT, \Delta)$ and outputs an approximate answer to each query in $\Q_\textsf{two}$ within error $\alpha$. Let $\widetilde{q}(\I)$ be the approximate answer for query $q \in \Q_\textsf{two}$. For each query $q \in \Q_\textsf{one}$, the corresponding query $q'\in \Q_\textsf{two}$. Let $\displaystyle{\Lambda = \max_{q'\in \Q_\textsf{two}} |\widetilde{q'}(\I)|}$. For each query $q \in \Q_\textsf{one}$, we just return an approximate answer $\displaystyle{\widetilde{q}(T) = \frac{\widetilde{q'}(\I) \cdot n}{\Lambda}}$, where $q' \in \Q_\textsf{two}$ is the counterpart of $q$ in our construction.

We first note that this algorithm for answering queries in $\Q_\textsf{one}$ preserves $(\epsilon, \delta)$-DP. This is not hard to show, since $\mathcal{A}$ preserves $(\epsilon, \delta)$-DP, and the post-processing is deterministic,  independent of the input instance. We next bound the error of approximate answers for queries in $\Q_\textsf{one}$. For any $q \in \Q_\textsf{one}$ and its counterpart $q' \in \Q_\textsf{two}$, we first point out that $\displaystyle{q'(\I) = q(T) \cdot \Delta}$.
%
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.67]{img/lb-two-table.pdf}
    \caption{Lower bound instance with $n=9$, $\Delta = 3$, $\OUT = 27$. }
    \label{fig:lb-two-table}
\end{figure} 
%
Implied by the error of answering queries in $\Q_\textsf{two}$, we know that
$\displaystyle{\big|q'(\I) - \widetilde{q'}(\I)\big| \le \alpha}$ holds for every query $q' \in \Q_\textsf{two}$.
From the error guarantee on the counting query, $|\Lambda - n \Delta| \le \alpha$.
For any query $q \in \Q_\textsf{one}$, we observe:
    \begin{align*}
       \big|q(T) - \widetilde{q}(T)\big| &= \big|\frac{q'(\I)}{\Delta} - \frac{\widetilde{q'}(\I)}{\Lambda} \cdot n \big| \\
        &= \big|\frac{1}{\Delta} \cdot \left(q'(\I) - \widetilde{q'}(\I) \right)\big| + \big|\left(\frac{1}{\Delta} - \frac{n}{\Lambda}\right) \cdot \widetilde{q'}(\I)\big|\\
        &\le \frac{1}{\Delta} \cdot \alpha + \big|\left(\frac{1}{\Delta} - \frac{n}{\Lambda}\right) \cdot \Lambda \big|  \le \frac{2\alpha}{\Delta}
    \end{align*}
    where the last inequality follows $\big|\left(\frac{1}{\Delta} - \frac{n}{\Lambda}\right) \cdot \Lambda \big| = \frac{1}{\Delta} \cdot \big|\Lambda - n \Delta \big|\le \frac{\alpha}{\Delta}$.
    If $\alpha = o\left(\sqrt{\OUT} \cdot \sqrt{\Delta}\right)$, then there is an $(\epsilon,\delta)$-differentially private algorithm that takes as input any single-table database $T \in \D$ and outputs approximate answers to each query in $\Q_\textsf{one}$ within error $o(\sqrt{n})$, coming to a contradiction of Theorem~\ref{the:lb-single-table}.
\end{proof}

\new{
\begin{theorem}
\label{the:lb-two-table}
    Given arbitrary parameters $\OUT>0$ and $\Delta > 0$ for $\Delta \le \OUT$, let $\mathbb{I}(\OUT, \Delta)$ be the class of instances that have join size $\OUT$ and local sensitivity $\Delta$. There exists a family of queries $\Q$ such that any $(\epsilon, \delta)$-DP algorithm that takes as input a database $\I \in \mathbb{I}(\OUT, \Delta)$, and outputs an approximate answer to each query in $\Q$ to within error $\alpha$ requires that \[\alpha \ge \Omega\left(\sqrt{\OUT} \cdot \sqrt{\Delta} \cdot (\frac{\log^{1/2} \D \cdot \log |\Q|}{\epsilon})^{1/2}  + \Delta\right).\]
    with probability $\exp(-\epsilon) \cdot (1-\delta)$.
\end{theorem}
}

%\pasin{Following paragraph seems out of place and should be moved somewhere else?}

